Safe Exploration for Efficient Policy Evaluation and Comparison

High-quality data plays a central role in ensuring the accuracy of policy evaluation. This paper initiates the study of efficient and safe data collection for bandit policy evaluation. We formulate the problem and investigate its several representative variants. For each variant, we analyze its statistical properties, derive the corresponding exploration policy, and design an efficient algorithm for computing it. Both theoretical analysis and experiments support the usefulness of the proposed methods.

==> Archive/8_discussion_points.tex <==
\section{Discussion Points}



% \todob{Restructure the above paragraph to better motivate what we do. In off-policy optimization, we estimate $\widehat{V}(\pi_1; \mD)$ for some known $\pi_1$ and from known $\mD$. This is typically used to test if $V_r(\pi_1) > V_r(\pi_0)$. How $\mD$ arises is never questioned. We study the problem of collecting $\mD$ to decide $V_r(\pi_1) > V_r(\pi_0)$ as efficiently as possible.}
% \todorw{Let's discuss should we discuss more in the introduction and keep this setup section concise?}


\todorw{Let's discuss the space issue as well. Some details/derivations/contents need to be moved to the appendix anyway. ICML format instruction requires name+year citation. }



==> Archive/9_Differentiable_Policy.tex <==
\subsection{Differentiable Policy}

==> Archive/9_Discussions.tex <==
\section{Discussion points to be resolved}
% Note that
% \begin{equation}
%     \begin{split}
%         var_{A_t \sim b}[\frac{\pi(A_t)}{b(A_t)}r(A_t)] 
%         = \sum_a \frac{\pi^2(a) r^2(a)}{b(a)}
%     \end{split}
% \end{equation}
% but this may not hold for \pi_{\Delta}
\begin{itemize}
    % \item The main goal of the discussion above is to motivate why we can ignore the second term in solving an efficient allocation. Alternatively, we can direct start our discussions with an exact design, and then relax to the continuous design case, which might be more natural. Though we need to introduce design instead of policy earlier. 
% Any other suggestions?
% from our observe in estimating $L$ and $U$ from the logged data 
\end{itemize}

% The second term can be dropped when we consider a fixed design where $N_a = \sum_t \I(A_t = a) \propto b(a)$.  \todob{I do not understand why the second term can be dropped. It does not seem to be zero. Specifically, even for a fixed design, when $A_t \sim b$, the term is not zero.}

% Although such a design probably can be obtained exactly, it can be our motivation to consider optimizing $b$ with this first term as the objective (where $b$ is used to compute the allocation proportions), and in implementation we may still need randomized rounding would be needed. 
% % Ignoring the second term for now (as in SafeOD)
% In this case, we consider the value estimator to be IPW with estimated assignment probability, i.e., the plug-in estimator with sample mean $\widehat{V}(\pi) = \sum_{a \in [K]} \frac{\sum_t \I(A_t = a) R_t}{\sum_t \I(A_t = a)}$. 
% \todob{Why do we need this plug-in estimator? I thought that we do inverse propensity scores. A: the main reason is, with a deterministic allocation rule, the standard IPW is not well defined.}


==> Archive/9_MAB_IPW_estiamted_propensity.tex <==
\subsection{Multi-armed bandits  with inverse probability weighting}\label{sec:MAB_IPW_alt}
We start our discussion with estimating the value of a $K$-armed bandit  policy using the popular inverse probability weighting (IPW) estimator \cite{dudik2014doubly}. 
For any dataset $\mD = \{(A_i, R_i)\}$, 
the IPW estimator is defined as 
$\widehat{V}_{IPW}(\pi; \mD) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \frac{\pi(A_i)}{\hat{b}(A_i)}R_i$, where $\hat{b}(a) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \I(A_t = a)$. 
Note that here we use the estimated propensity $\hat{b}(a)$. 
A well-known but perhaps counter-intuitive result \cite{brumback2009note} says that, even if $\mD$ is collected by following $b$ and $b$ is known, $\widehat{V}_{IPW}(\pi; \mD)$ is more efficient than plugging-in $b$. 

We aim to design the optimal way to collect the new dataset of size $T$, which is equivalent to allocating the $T$ budgets to the $K$ arms. 
Let $N_a$ be the number of data points assigned to the $a$th arm, 
set $b(a) = N_a / T, \forall a \in [K]$, 
and denote the resulting dataset by $\mD_b$. 

We first consider the case where there is no logged dataset $\mD_0$. 
Our objective can then be written as
\begin{align*}
            &\argmin_{b \in \Delta_{K - 1}} var\big(\widehat{V}_{IPW}(\pi_1; \mD_{b}) - \widehat{V}_{IPW}(\pi_0; \mD_{b}) \big)\\
        &s.t. \;\; V_{\vr}(b) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K. 
\end{align*}
This problem is particularly challenging due to (i) the dependency of the objective on $b$ is complex, 
and (ii) the safety constraint involves the unknown function $V$ and hence not easy to guarantee. 

% \textbf{Objective function. }
We aim to first transform the objective into a tractable form. 
Let $\pi_{\Delta} = \pi_1 - \pi_0$ and $\sigma^2_a = var(R_t \mid A_t = a), \forall a \in [K]$. 
We have 
\begin{align}
&T \times var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{b}) - \widehat{V}_{IPW}(\pi_0; \mD_{b}) \Big)\nonumber\\
&= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \sigma^2_a 
 \label{eqn:MAB_objective_alt}
\end{align}
Without safety constraints, 
the optimal allocation rule is similar with the Neyman allocation in statistics \cite{neyman1992two}, i.e., $b(a) \propto \sigma_a |\pi_{\Delta}(a)|$. 
Besides, perhaps surprisingly, following similar arguments, we can show that the on-policy strategy (i.e., by setting $b = \pi_1$) is not even optimal in minimizing $var\big(\widehat{V}(\pi_1; \mD_{b}))$, 
when $\sigma_a$'s are different. 

% $\{A_t\}_{t=1}^T \sim \text{Multinomial}(T, b)$, 
%  = T \times b(a)
The first challenge to solving \eqref{eqn:MAB_objective} is that, it is hard to guarantee that $N_a$'s are all integers for the minimizer $b$. 
However, various randomized rounding techniques \hl{[cite]} can be applied to obtain a set of integers $\{N_a\}$ that is close to the continuous solution, and the variance inflation is guaranteed to be negligible when $K$ is small compared with $T$. % enough

% derivations in \eqref{eqn:MAB_objective}  may not hold any longer. That is why I introduced a new IPW
% " " does not make sense any longer
The second challenge is that $\sigma_a$ is typically not known \textit{a priori}. 
Without additional information and given the fact the second moment is typically more difficult to estimate than the first moment, 
we consider an upper bound of the objective, by replacing every $\sigma_a$ with their joint upper bound. 
With this relaxation, our objective reduces to 
\begin{equation*}
    \begin{split}
    \argmin_{b  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)}
    \end{split}
\end{equation*}
Without safety constraints, 
the optimal allocation rule is similar with the proportional allocation in statistics \cite{fuller2011sampling}, i.e., $b(a) \propto |\pi_{\Delta}(a)|$. 
% Again, the exact integer allocations can be solved via randomized rounding. 
% This exactly corresponds to the on-policy strategy. 

% \textbf{Safety constraint. }
With a tractable and appropriate surrogate objective, we are now ready to consider the safety constraint $V_{\vr}(b) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K$. 
The first observation is that, the constraint is equivalent to $b(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]$. 
This is mainly due to that there is no any information on $\vr$ and we need to ensure the safety constraint under the worst case. 
Specifically, 
when there exists at least one arm $a$ such that $b(a) < (1-\epsilon) \pi_0$, we can always construct a instance to violate the constraint, where $r(a) = 1$ and $r(a') = 0, \forall a' \neq a$. 

\textbf{Optimization without side information. }
Therefore, we finally achieve a desired optimization objective, by solving which we can obtain an efficient and safe continuous design for our OPE task: 
\begin{equation}
    \begin{split}
        &\argmin_{b  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\; b(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K] . 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_no_logged_alt}
\end{equation}
This problem is convex and hence can be efficiently solved by many convex optimization algorithms \cite{boyd2004convex}. 
% For general values of $\{\sigma_a\}$, though this solution will not be globally optimal,  we can provide upper bounds instead. 


% \begin{figure}
%     \centering
%     \includegraphics[width = 10cm]{Fig/MAB.png}
%     \caption{MAB: $V(\pi_1)$}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}

\textbf{Utilization of side information. }
\hl{update here.!}
Next, we consider there is side information that allows us to improve on \eqref{eqn:MAB_IPW_no_logged}. 
We assume we have a logged dataset $\mD_0$ generated by a historical behaviour policy $b_0$. 
We assume $b_0$ is known for simplicity, and otherwise it can be estimated via methods standard in the OPE literature. 
We expect the information in $\mD_0$ will have impact on both our objective and safety constraint. 
Specifically, the original problem can be written as 
\begin{equation}
    \begin{split}
        &\argmin_{b \in \Delta_{K - 1}} 
        % (N+T)^{-2}
        var \Big(
        \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{b(A_t)} R_t
        + \sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
        \Big)\\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\; min_{\vr \in \mathcal{C}_\delta(\mD_0)} \vr^T(b - (1-\epsilon) \pi_0) \ge 0. 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_w_logged_raw_alt}
\end{equation}  
Here, $\mathcal{C}_\delta(\mD_0)$ is an $(1-\delta)$-confidence region on $\vr$ obtained from $\mD_0$. 
For instance, we can construct an $(1-\delta / K)$-confidence interval for each arm separately. 
Alternatively, one may consider a Bayesian setup where there is a prior on $\vr$, and $\mathcal{C}_\delta(\mD_0)$ is the credible intervals derived from the corresponding posteriors. 

% [\vL(\delta, \mD_0), \vU(\delta, \mD_0)]


Perhaps surprisingly, thanks to the independence between $\mD_b$ and $\mD_0$, the objective of     \eqref{eqn:MAB_IPW_w_logged_raw} is equal to
$
var \Big(
\sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{b(A_t)} R_t \Big)
+ var\Big(\sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
\Big)$, 
where the second term does not depend on $b$ can hence can be dropped in the objective. 
In other words, the additional dataset $\mD_0$ does not affect the optimization objective. 
The main reason is that in IPW, every data point contributes independently to the estimator. 
This may not be the case for some other OPE estimators, as will be shown later. 

\textbf{Optimization with side information. }
Therefore, by similar arguments with \eqref{eqn:MAB_IPW_no_logged}, we can consider the following optimization problem
\begin{equation}
    \begin{split}
        &\argmin_{b \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\;  \vr^T(b - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \mathcal{C}_\delta(\mD_0). 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_w_logged_alt}
\end{equation}
We note this problem is particularly challenging as the constraint implicitly contains a \textit{infinite} number of constraints. 
With the observation that, for any finite set $\Theta \subset \Delta_{k-1}$, 
$min_{\vr \in \Theta} \vr^T(b - (1-\epsilon) \pi_0) \ge 0$ is a system of linear constraints. 
Therefore, we propose to solve \eqref{eqn:MAB_IPW_w_logged} by combining convex optimization with the cutting-plane method \cite{bertsimas1997introduction}. 
Specifically, the cutting-plane method iteratively refines a finite set of constraints to approximate the infinite set of constraints through adding then one by one, until no constraint in the infinite set is violated. 
We present the algorithm details in Appendix \ref{sec:optimization_MAB}. 

% The underlying principle is to approximate the feasible region of a nonlinear (convex) program by a finite set of closed half spaces and to solve a sequence of approximating linear programs.

\hl{[explain the allocation more clearly]}

% We note that, with IPW as the value estimator, the objective does not change when we also utilize the logged dataset $\mD_0$ in the objective in addition to in the safety constraint. 
% This is because the additive structure of IPW. 
% This may not be the case when we consider other estimators. 
% although it looks like we only utilize the side information (which typically comes from a ) in the safety constraint but not in the objective, 
% and when we only utilize (?) it in the safety constraint




==> Archive/9_Setup.tex <==


% \section{Setup}


% \begin{align*}
%     r(\vx_t, a) &= \vx_t^T \vthe_a, \forall a \in \mathcal{A} \; \text{(disjoint, finite arm)} \\ % including two-arm (A learning?)
%     r(\vx,a) &= \vphi^T_{\vx,a} \vthe \; \text{(transformed feature)}\\ % \Mean(R_t|\vx_t = \vx, A_t = a) = 
%     % , \forall a \in \mathcal{A} \\ % including two-arm (A learning?)
%     r(\mX,a) &= \vx^T_{a,t} \vthe \; \text{(one context per arm)}\\ 
%     r(\vx_t) &=  \vx_t^T \vthe  \;\; \text{(x is just arm; can be a fixed set, or infinite)}     % linear regression 
% \end{align*}

% \textbf{Setup.} 
% \begin{equation}
%     \begin{split}
%     r(\vx,a) &= \vphi^T_{\vx,a} \vthe^*\\ % \Mean(R_t|\vx_t = \vx, A_t = a) = 
%     V(\pi) &= \Mean_{\vx \sim p(\vx), a \sim \pi(a \mid \vx) }  \; r(\vx, a)
%     % V(\pi) &= \ \Mean_{\vx \sim p(\vx)}  \sum_{a \in \mathcal{A}} \pi(a \mid x) r(x, a)\\
%     % , \forall a \in \mathcal{A} \\ % including two-arm (A learning?)
%     \end{split}
% \end{equation}



% \item : i.i.d. sampled following a behaviour policy $b_0$, which could be the same with $\pi_0$
% \item the context distribution $p(\vx)$ or possibly a large context dataset $\mD'_{\vx}$
% \item a function to construct the transformed feature  $\vphi_{\vx, a}$


% Suppose we have access to (some are optional):
% \begin{itemize}
    % or adaptively collected
    % \item an off-policy optimization algorithm $\mathcal{O}$ which maps a dataset to a policy
%     \item budget $T$ and risk tolerance $\epsilon \in (0,1)$ % safety threshold
% \end{itemize}


% \textbf{Goal. }
% % We would like to design a  (or an adaptive one?) to collect a new dataset $\mD = \{(\vx_t, A_t, R_t)\}_{t=1}^T$ where $A_t \sim b(\cdot|\vx_t)$, 
% so that 
% % (i) during the $T$ interactions, we satisfy the safety constraint that $\sum_t\Mean_{\vx_t \sim p(\vx), A_t \sim b(\cdot \mid \vx_t)}R_t \ge (1-\epsilon) \sum_t\Mean_{\vx_t \sim p(\vx), A_t \sim \pi_0(\cdot \mid \vx_t)} R_t$ for any problem instance (or with probability at least $\delta$ evaluated using logged dataset? expectation over x?), 
% % (could be a stage-wise as well) 
% and (ii) after the $T$ interactions, we achieve one of the following goals: 
% % \begin{itemize}
% %     \item \textbf{Evaluation}: we can consider several goals, of (potentially) increasing difficulty
%     \begin{itemize}
%         \item minimize $var(\widehat{V}(\pi_1))$: suppose we have enough data following  $\pi_0$ and hence its value can be well estimated, which is a common starting point. (We also need to assume the linear reward function is correctly specified, and hence the DM estimator is unbiased, and hence we only need to minimize the variance. )
%         \item maximize $\prob( \widehat{V}(\pi_1) - \widehat{V}(\pi_0) \ge 0  \mid V(\pi_1) - V(\pi_0) \ge \delta)$
%         % \item maximize $\prob{(\widehat{V}(\pi_1) - \widehat{V}(\pi_0)) (V(\pi_1) - V(\pi_0)) > 0}$
%         \item maximize $\prob(reject \;\; \{V(\pi_1) - V(\pi_0) \le 0 \} \mid V(\pi_1) - V(\pi_0) \ge \delta)$
%         % \item continuously monitor the test to allow early stop
%     \end{itemize}
    % our new policy $\pi' = \mathcal{O}\Big(\mD \bigcup \mD'\Big)$ yields high value in expectation (or high-probability bound?), i.e., we aim to maximize $\Mean(V(\pi'))$ where the expectation is taken over $\mD'$ and hence $\pi'$.
    % \item \textbf{Optimization}: our new policy $\pi' = \mathcal{O}\Big(\mD \bigcup \mD_0\Big)$ yields high value in expectation (or high-probability bound?), i.e., we aim to maximize $\Mean(V(\pi'))$, where the expectation is taken over $\mD$ and hence $b$.
% \end{itemize}

% There are several moving parts: 
% \begin{enumerate}
%     % \item Objective
%     \item Safety constraint: there are a few ways to define
%     \item Logged dataset: should enter (provide information for) both the objective and the safety constraint
%     \item Value estimator can be different (IPW, DM, DR)
%     \item Bandit problem setup: MAB, nonstochastic linear bandits, 
%     contextual MAB, stochastic contextual linear bandits, etc. 
%     % linear generalization, contextual MAB, etc. 
% \end{enumerate}

% Distributional G-optimal design?
% back to linear regression? so simple?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% functional form of pi and pi_0 matter? [let us start with linear]

% \subsection{Related work and comparison}


==> Archive/9_allocation_rule.tex <==
\subsection{From exploration policy to allocation rule}
In the previous discussion, we aim to solve an efficient exploration policy $b$, which is a (conditional) distribution over arms. 

For tractability, NP-hard.

In this section, we discuss how to utilize $b$ to collect the dataset $\mD_b$ of size $T$. 


\hl{Read more. }

==> Archive/9_derivations_IPW.tex <==
\subsection{Inverse IPW}
\begin{equation}
    \begin{split}
   V_{\pi_1}  &= \Mean  \sum_a Y(a) \pi_1(a \mid \vx) = \Mean \frac{R_t \pi_1(A_t \mid \vx_t)}{b(A_t \mid \vx_t)}\\
   \widehat{V}_{\pi}  &= N^{-1} \sum_t\frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} 
    \end{split}
\end{equation}

Positivity assumption: $\forall (\vx, a)$, if $P(\vx) > 0$ and  $\pi_1(a \mid \vx ) > 0$, then $b(a \mid \vx ) > 0$. 

\begin{equation}
    \begin{split}
\argmin_b \;\;
&var \Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
+ 
var_{\vx_t} \Mean_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
+ 
var_{\vx_t} \Mean_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
% + 
% var_{\vx_t} \Mean_{A_t \sim \pi_1(a \mid \vx_t)}\Big[R_t \mid \vx_t \Big]
+ const\\
&= 
\Mean_{\vx_t} 
\Big\{
\Mean_{A_t \sim b(a \mid \vx_t)}\Big[ var(R_t \mid A_t, \vx_t) \frac{ \pi^2_1(A_t \mid \vx_t) }{b^2(A_t \mid \vx_t)}  \Big]
+
var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{\Mean(R_t \mid A_t, \vx_t)  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \Big]
\Big\}
+ const\\
&= 
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}
+ const
    \end{split}
\end{equation}
Without the safety constraint and ignoring the logged dataset, and suppose we know  $\Mean[R^2_t \mid \vx_t, A_t] $, the optimal design should be the Neyman allocation, i.e., 
\begin{equation}
    \begin{split}
    b(a \mid \vx) \propto \sqrt{var(R_t \mid A_t = a, \vx_t = \vx)} \times  \pi_1(a \mid \vx), \forall \vx
    \end{split}
\end{equation}

There are several issues we need to address:
\begin{enumerate}
    \item $var(R_t \mid A_t = a, \vx_t = \vx)$ is unknown: The unknown variance can be replaced with the plug-in estimator, or we can consider some less optimal ones? 
% Since 
    \item The safety constraint
    \item The existing offline dataset: The existing offline dataset can be accommodated via results from stratified sampling, as in \cite{kallus2021optimal}. 
\end{enumerate}
% adaptively collected
% support deficiency



The safety constraint needs a lower bound for IPW-based value estiamtor (under potential support deficiency?) 
Based on the asymptotic distribution 

\begin{align*}
          \sqrt{n}(\widehat{V}_{b} - V_{b})
    %   \sim  
    &\convergeD
      \mathcal{N}(\vzero, \sigma_1^2), 
      \quad  
      \sigma_1^2 
      = 
    \Mean_{b_0}\Big(\frac{R_t  b(A_t \mid \vx_t)}{b_0(A_t \mid \vx_t)}  - V_{b} \Big)^2, 
    %   \Mean\Big(\frac{(Y_i - V_{\delta})^2}{\prob_{\delta(\vx_t)}} \Big)
\end{align*}
where $b_0$ is the behaviour policy for $\mD_0$. 
A lower bound on $V_b$ is then $\widehat{V}_{b} - z_{\alpha} n^{-1/2} \sigma_1$. 
Hence, we may need to solve the problem above, under a constraint similar with (too conservative?)
$  \widehat{V}_{b} = |\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i)   \ge (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1$. 
% Given any $\vx$, we would like to solve
% \begin{align*}
%     \argmin_{b} \; 
%     \sum_a 
%     \frac{\Mean[R^2_t \mid \vx, a]  \pi^2_1(a \mid \vx)}{b(a \mid \vx)} 
% \end{align*}

% suppose the variance level is the same. 
% stratified sampling

\begin{equation}
    \begin{split}
    &\argmin_b    
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}\\
&s.t. \;
|\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i)   \ge (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1  
    \end{split}
\end{equation}

We can parameterize $b$ as a differentiable policy and solve the Lagrange via stochastic gradient descent-ascent? 
\begin{equation}
    \begin{split}
min_b \max_{\lambda \ge 0}    L(b, \lambda)
    = \Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\} 
+ \lambda 
\Big\{
l_0 - |\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i) 
\Big\}, 
    \end{split}
\end{equation}
where $l_0 = (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1$. 


 
 
Alternatively, we can consider
\begin{equation}
    \begin{split}
&\argmin_b    
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}\\
&s.t. \;  b(a\mid\vx) \ge (1-\epsilon) \pi_0(a\mid\vx), \forall a, \vx, 
    \end{split}
\end{equation}
which can probably be solved via constrained optimization. 
Alternatively, we can consider the policy mixture approach in \cite{zanette2021design}, that is, do \textit{pseudo} online learning with the offline dataset from $t = 0$, and at each time point, we choose the direction that minimize the variance under the constraint, and finally apply a mixture policy. 

% Assuming a linear value function?:
% \begin{align*}
%     \min_{\vthe \in \mathcal{C}_\delta} \quad \Mean_{\vPhi \sim b} \big(\vone^T \vPhi\vthe\big)  
%     \ge (1-\epsilon) \max_{\vthe \in \mathcal{C}_\delta}  \Mean_{\vPhi \sim \pi_0} \big(\vone^T \vPhi\vthe\big)  
% \end{align*}

% Try to further simplify the form. 

% \begin{align*}
%     \argmin_{b} \; &\Mean_{\vx_t \sim p(\vx), A_t \sim b(a \mid \vx_t) }\Big(\frac{R_t  \pi_1(A_t \mid \vx_t)}{b(A_t \mid \vx_t)}  - V_\pi \Big)^2\\
%     % s.t. \quad 
%     s.t. \; &\min_{\vthe \in \mathcal{C}_\delta} \quad \Mean_{\vPhi \sim b} \big(\vone^T \vPhi\vthe\big)  
%     \ge (1-\epsilon) \max_{\vthe \in \mathcal{C}_\delta}  \Mean_{\vPhi \sim \pi_0} \big(\vone^T \vPhi\vthe\big)  
%     % &XX1
% \end{align*}

\subsection{Adaptive exploration policy}
maximize the least confident direction + check the lower bound to make sure no violation

\subsection{Fixed exploration policy}
Achieve that idea in an offline fashion [by simulation] [because of the fixed] [a simulation based procedure]


==> Archive/main_draft.tex <==
% \input{FRONT}
\input{Style}
\title{Safe Exploration for Efficient Off-policy Evaluation}
\date{\today}
\author{}
% Efficient
% Optimization

\begin{document}
\maketitle
\linenumbers
% \pagestyle{fancy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{1_Setup}
\input{1_Intro}

\input{2_Method}

\input{3_Theory}

\input{4_Expt}



\bibliographystyle{aaai2021.bst}
\bibliography{bib}

\appendix
\newpage


\input{9_Appendix_other_settings}


\end{document}


==> Archive/testing.tex <==

\subsection{Connection with hypothesis testing}
% \textbf{Connection with hypothesis testing.} 
In real applications, one important task is to test whether or not the target policy $\pi_1$ is significantly better than $\pi_0$, which impacts the decision-making of deploying $\pi_1$. 
We next present the relationship between the power of such a test and our ultimate optimization objective $var\big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \big)$. 
We focus on the case without side information for simplicity, and it is straightforward to accommodate $\mD_{0}$. 
% extend to the case with
Specifically, we consider the test
\begin{align*}
    H_0: V(\pi_1) \le V(\pi_0) \quad \text{v.s.} \quad H_1: V(\pi_1) > V(\pi_0). 
\end{align*} 
% $\sigma(\pi_e) {=} \sqrt{var\big(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t\big)}$
% $\sigma(\pi_e) {=} \sqrt{var(\pi_e(A_t)^{-1}\pi_{\Delta}(A_t)R_t)}$
Denote our raw objective \eqref{eqn:raw_MAB_obj} by $\sigma(\pi_e)$  and let $\hat{\sigma}(\pi_e)$ be a consistent estimator with $\mD_e$ (typically the plug-in estimator with sample variance). 
By the central-limit theorem and the Slutsky’s lemma, we have 
\scalebox{0.92}{\parbox{\linewidth}{%
\begin{align*}
\frac{\sqrt{T}}{\hat{\sigma}(\pi_e)}
    \Big[
    \big(\widehat{V}(\pi_1; \mD_{e}) 
    {-} \widehat{V}(\pi_0; \mD_{e}) \big)
    {-} \big(V(\pi_1) {-} V(\pi_0)\big)\Big]
    \overset{d}{\to} \normal(0, 1), 
\end{align*}
}}
% \begin{align*}
%     \hat{\sigma}(\pi_e)^{-1} \sqrt{T}
%     &\Big[
%     \big(\widehat{V}(\pi_1; \mD_{e}) 
%     - \widehat{V}(\pi_0; \mD_{e}) \big)\\
%     &\quad- \big(V(\pi_1) - V(\pi_0)\big)\Big]
%     \overset{d}{\to} \normal(0, 1), 
% \end{align*}
% $\hat{\sigma}(\pi_e)^{-1} \sqrt{T}
% \big(\widehat{V}(\pi_1; \mD_{e}) 
% {-} \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}$
when $T$ grows.  %  \to \infty
Therefore, an (asymptotically) $\alpha$-level test is to reject the null when 
\begin{align*}
    \hat{\sigma}(\pi_e)^{-1} \sqrt{T}
\big(\widehat{V}(\pi_1; \mD_{e}) 
{-} \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}, 
\end{align*}
where $z_{1-\alpha}$ is  the upper $\alpha$th quantile of the standard normal distribution. 
For any $\Delta > 0$, the (asymptotic) power under the local alternative $H_1 : V(\pi_1) - V(\pi_0) {=} \Delta / \sqrt{T}$ 
is hence 
$1 - \Phi\big(z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta\big)$, where $\Phi(\cdot)$ is the cumulative distribution function of standard Gaussian. 
Since the other terms are all constant, it is clear that $\sigma(\pi_e)$ determines the power. 
Therefore, with a fixed budget, one can improve the power by designing a better policy $\pi_e$ to reduce $\sigma(\pi_e)$, which corresponds to our objective. 
Such a connection can be built similarly for the other setups considered in this paper (see Appendix \ref{sec:other_testing} for details). 
\todob{Do we want to have something more finite-sample?} 
\todorw{Let's discuss more. Not sure how. In Stats and Econ, the value tests I am aware of are all asymptotic. (besides boostrapping-based)}
\todob{We do not really do policy evaluation. That would be estimate $V(\pi_1)$. We do lift evaluation. This is what $V(\pi_\Delta)$ means. The problems are algebraically equivalent though. We can claim that we can do both. We focus on $V(\pi_\Delta)$ because it is more practical.}
% in similar ways
% \hl{hold for other settings?}
% both $V(\pi_1) - V(\pi_0)$ and $z_{1-\alpha}$


% $\prob\Big(Z \ge z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta \Big)$
% $Z$ is a standard normal random variable. 

==> Fig/illustration.tex <==
\begin{figure*}[!t]
\centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\begin{subfigure}{.3\textwidth}
  \centering
    % \vspace{.2cm}
  \includegraphics[width=\linewidth]{Fig/safeOD_OPE-OPE.pdf}
  \vspace{-0.5cm}
  \caption{
  Standard OPE. 
  }
\end{subfigure}%
% \hspace{.3cm}
\begin{subfigure}{.55\textwidth}
  \vspace{-.2cm}
  \centering
  \includegraphics[width=\linewidth]{Fig/safeOD_OPE-Ours.pdf}
  \vspace{-1.1cm}
  \caption{SEPEC: designing a safe and efficient exploration policy to collect high-quality data for a given OPE task. 
  }
\end{subfigure}%
\vspace{-.3cm}
\caption{Comparisons between the standard OPE setting and our proposal.}\label{fig:illustration}
\vspace{-0.3cm}
% safe design of experiments
\end{figure*}


==> Fig/more_setting_results.tex <==
\renewcommand{\sharedwidthSubFig}{0.9}
\renewcommand{\sharedwidth}{0.52}
\renewcommand{\sharedheight}{3cm}
\renewcommand{\hbetween}{0.1cm}
\renewcommand{\vbetween}{-0.5cm}

\begin{figure}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/MAB.pdf}
    \vspace{\vbetween}
  \caption{
  MAB with IPW. 
  }
\end{subfigure}%

% \hspace{\hbetween}
\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/CMAB.pdf}
    \vspace{\vbetween}
  \caption{CMAB with IPW.}
\end{subfigure}%

\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/LB.pdf}
  \vspace{\vbetween}
  \caption{Linear bandits with DM.}
\end{subfigure}%
\vspace{-0.2cm}
\caption{Experiment results. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
For methods that consider the safety constraint, the losses from safety violation are around zero and hence may overlap.}\label{fig:more_setting_CMAB}
% safe design of experiments
\vspace{-0.5cm}
\end{figure}


==> Fig/real_data_results.tex <==
\begin{figure}[!t]
  \centering
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337CMAB_real.pdf}
  \caption{CMAB with IPW.}\label{fig:real_CMAB}
\end{subfigure}%
\hspace{.5cm}
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337LB_real.pdf}
  \caption{Linear bandits with DM.}\label{fig:real_LB}
\end{subfigure}%
\caption{Experiment results on the MNIST dataset. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
For methods that consider the safety constraint, the losses from safety violation are around zero and hence may overlap.}\label{fig:real}
\end{figure}


==> Fig/simu_res_old.tex <==
% \newcommand{\sharedwidthSubFig}{0.85}
\newcommand{\sharedwidth}{0.5}
\newcommand{\sharedheight}{3cm}
\newcommand{\hbetween}{0.1cm}
\newcommand{\vbetween}{-0.6cm}
\newcommand{\hleft}{-0.3cm}

\begin{figure}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/MAB.pdf}
    \vspace{\vbetween}
  \caption{
  MAB with IPW. 
  }
\end{subfigure}%

% \hspace{\hbetween}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/CMAB.pdf}
    \vspace{\vbetween}
  \caption{CMAB with IPW.}
\end{subfigure}%

\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/LB.pdf}
  \vspace{\vbetween}
  \caption{Linear bandits with DM.}
\end{subfigure}%
\vspace{-0.2cm}
\caption{Experiment results. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
% For methods that consider the safety constraint, 
The losses from safety violation for safe methods are all around zero and hence overlap.}\label{fig:simu}
% safe design of experiments
\vspace{-0.5cm}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/0_Front_ICML.tex <==

\twocolumn[
\icmltitle{
Safe Exploration for Efficient Policy Evaluation and Comparison
}

% It is OKAY to include author information, even for blind
% \icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Runzhe Wan}{to1}
\icmlauthor{Branislav Kveton}{to2}
\icmlauthor{Rui Song}{to1}
\end{icmlauthorlist}

\icmlaffiliation{to1}{Department of Statistics, North Carolina State University}
\icmlaffiliation{to2}{Amazon}
% \icmlaffiliation{to3}{Department of Statistics, North Carolina State University}
% \icmlaffiliation{goo}{Googol ShallowMind, New London, Michigan, USA}
% \icmlaffiliation{ed}{School of Computation, University of Edenborrow, Edenborrow, United Kingdom}

\icmlcorrespondingauthor{Rui Song}{rsong@ncsu.edu}
% \icmlcorrespondingauthor{Eee Pppp}{ep@eden.co.uk}


% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

\printAffiliationsAndNotice{} % otherwise use the standard text.
% icmlEqualContribution


==> Safe Exploration for OPE [Camera-ready]/1_Abstract.tex <==
\begin{abstract}
High-quality data plays a central role in ensuring the accuracy of policy evaluation. 
This paper initiates the study of efficient and safe data collection for bandit policy evaluation. 
We formulate the problem and investigate its several representative variants. 
For each variant, we analyze its statistical properties, derive the corresponding exploration policy, and design an efficient algorithm for computing it. 
Both theoretical analysis and experiments support the usefulness of the proposed methods. 
\end{abstract}

% of the value estimator

==> Safe Exploration for OPE [Camera-ready]/1_Intro.tex <==
\section{Introduction}
% \input{Fig/illustration}
Bandit policies have been widely applied to areas including advertising \citep{bottou2013counterfactual}, search \citep{li2011unbiased} and healthcare \cite{zhou2017residual}. 
% clinical trials \citep{durand2018contextual}. 
% in many applications, 
Before deploying a target policy, it is typically crucial to have an accurate evaluation  of its performance, which can subsequently provide valuable information for deployment decisions or model improvement.  
This is in general achieved by utilizing logged data, known as the \textit{off-policy evaluation (OPE)} problem. 
% a different logging
% collected following other policies

Although OPE has been studied extensively \cite{dudik2014doubly, li2015toward, swaminathan2016off, wang2017optimal, su2020doubly, kallus2021optimal, cai2021deep}, 
the existing works mainly focus on various estimators with a \textit{fixed} dataset. 
However, limited attention has been paid to the dataset itself, which plays a vital role in estimation accuracy. 
For instance, inverse probability weighting \citep[IPW, ][]{li2015toward}, one popular OPE method, has a key requirement that the logging policy has 
\say{full support}. 
% "full support". 
% \todob{Use \say{full support} from dirtytalk for quotes.}
This usually translates into requiring the logging policy to be close enough to the target policy \citep{sachdeva2020off, tran2021combining}. 
For direct method \citep[DM, ][]{dudik2014doubly}, it is also common that some feature directions are less explored in the logged dataset, which impacts the accuracy of this regression-based estimator. 
% Besides, the concern over the potential confounders \cite{sohoney2018handling} is another common reason to challenge OPE with logged data and require collecting some data in a controllable way. 

% motivation to consider  some experiment data, on the basis of which we can then evaluate an policy. 
% class of OPE estimators
% \todob{Too long sentence.}

To improve the accuracy of policy evaluation, a natural idea is to actively collect high-quality data, and ideally, the data collection  rule should be tailored to the given  evaluation task. 
This problem is surprisingly unexplored. 
Moreover, due to the common safety concerns \cite{wu2016conservative, zhu2021safe}, 
it is of great practical importance to make sure the data collection rule is safe. 

% \todob{I noted that you use a lot of "will". Unless talking about future work, they are not necessary. "We focus on" would sound as natural here.} 

%  = \{(\vx_i, A_i, R_i)\}
% collect additional data in an controllable way
% non-adaptive
In this paper, we initiate the study of \textit{Safe Exploration for Policy Evaluation and Comparison (\name{SEPEC})}, the design of an efficient and safe exploration policy that collects a high-quality dataset for the given evaluation task. 
We  focus on non-adaptive policies, as they are simple to implement logistically. 
Indeed, in practice, the challenge of requiring investments (e.g., in infrastructures) for adaptive algorithms has been widely recognized \cite{zanette2021design, zhu2021safe}, especially before the value is proved via OPE. Our proposal is summarized in Figure \ref{fig:illustration}. 
% \todob{I do not understand "personnel training". Drop it. There are no specific jobs for running adaptive policies... although that would be sweet :o)}
% and personnel training
% Besides, it is easy to parallelize \cite{zanette2021design} and to conduct inference with \citep{cai2021doubly}. 
% We focus on non-adaptive policy 
% given the common engineering complexity of building an infrastructure for an adaptive algorithm \cite{zanette2021design, zhu2021safe}, especially before the value of any policy is proved using OPE. 
% \todorw{Brano: would you mind checking this sentence? and adding the safety issue of adaptive algorithm if you think that helps here? Thanks!}
% The goal, at the first glance, may seem to contradict the OPE objective, as one may expect we should be either fully off-policy with only logged data, or we can just run on-policy evaluation (i.e., acting following the target policy). 

Another possible approach to policy evaluation is being on-policy (i.e., following the target policy). 
However, the safety concern typically does not allow a direct deployment. 
% us to directly deploy it; % be fully on-policy
In addition, perhaps surprisingly, the on-policy evaluation is not optimal under some setups (e.g., when the variances of different arms differ) or for some evaluation tasks (e.g., comparing the target policy with a baseline policy). 
See Section \ref{sec:MAB_IPW} for an example. 
Therefore, more careful analysis and design are required. 

% comparison between our proposal and the standard OPE task can be found
% We expect and will also show 
As expected and shown later, our proposed solutions vary across different bandit setups, evaluation tasks, and value estimators. % , and availability of side information. 
To shed light on this novel problem, we study its three representative variants, including multi-armed bandits (MAB) with IPW, contextual MAB (CMAB) with IPW, and linear bandit with DM. 
Our results can be extended to several other setups that are introduced as well. 
% important aspects of this problem, and
% The discussions and ideas developed can be extended to some other problems that will be introduced as well. 
% Following these discussions and similar ideas, a few extensions can be considered and will be introduced as well. 
Finally, although other evaluation problems (e.g., estimating the value of the target policy in Section \ref{sec:PE}) can be addressed similarly to our work, for concreteness, we focus on \textit{policy comparison}, where we estimate the value difference between the target and baseline policies. 
This task is closely related to deployment decision making. 

\input{Fig/illustration_one_graph}


\textbf{Contribution. } Our contributions can be summarized as follows. 
First, motivated by practical needs for improving policy evaluation accuracy and the common safety concerns, we propose and formulate the \name{SEPEC} framework. % safe exploration for policy evaluation % problem
To the best of our knowledge, this is the \textit{first} work studying how to collect data for efficient policy evaluation, with or without  safety constraints. % even without
% The limitations of existing approaches are discussed to provide insights. 
Second, we investigate its three representative variants thoroughly. 
We analyze their statistical properties, design tractable optimization problems, and provide efficient optimization algorithms. 
The situations with or without side information are both considered. 
% provide tractable algorithms for the challenging optimization problems. 
Third, we theoretically prove the efficiency and optimality of our approach. 
% Third, we provide theoretical analysis to support the efficiency of our approach. 
Lastly, we demonstrate the superior performance of \name{SEPEC} through extensive experiments. 
% over popular baselines
% on the estimation error and related hypothesis testing power following our approach. 
% which clearly demonstrates the benefits. 
% and relate our objective to the power of hypothesis testing.


==> Safe Exploration for OPE [Camera-ready]/1_Objective.tex <==
\section{Objective and Existing Approaches}\label{sec:objective_and_baselines}
For concreteness, we first introduce the objective of \name{SEPEC} under MAB, and will extend it to other settings later. 
% to contextual bandits and linear bandits
% We first \textit{informally}  the problem below and will instantiate when we consider different OPE estimators. 
For any positive integer $M$, we denote the set $\{1, \dots, M\}$ by $[M]$. 
Let $\Delta_{K-1}$ be the $K$-dimensional simplex. 
% For any vectors $\mathbf{a}$ and $\mathbf{b}$, we use $\mathbf{a} \ge \mathbf{b}$ to denote that the inequality holds for all entries.
In a $K$-armed bandit, 
we represent a policy by a vector $\pi = (\pi(1), \dots, \pi(K))^T \in \Delta_{K-1}$, where $\pi(a)$ is the probability that arm $a$ is pulled under policy $\pi$. 
% , a distribution over arms. 
After choosing an arm $A_t$, we receive its stochastic reward $R_t$. 
% Following policy $\pi$, at every round $t$, we choose an arm $A_t \in [K]$ with probability $\pi(A_t)$, and then receive a stochastic reward $R_t$. 
Let $r_a = \Mean[R_t | A_t = a]$ be the expected reward of arm $a$ and $\sigma^2_a = \var(R_t | A_t = a)$ be the variance of its rewards. 
Let $\vr = (r_1, \dots, r_K)^T$. 
The value of a policy is $V(\pi) = \sum_{a \in [K]} \pi(a) r_a$. 
Sometimes we write $V_{\vr}(\pi)$ to emphasize the dependency on $\vr$. 
% of $V(\pi)$ on the instance parameter $\vr$. 
We make the standard assumptions that $r_a \in [0,1]$ and $\sigma^2_a \le \sigma^2$ for some $\sigma > 0$. 
A problem instance is specified by $(\vr, \{\sigma_a\})$. 
% Without loss of generality, we assume $\sigma^2_a \le \sigma^2$ for some $\sigma$. 


% which is typically the baseline  policy
We assume that we are given a \emph{target policy} $\pi_1$ and a safe \emph{baseline policy} $\pi_0$. 
We may also have side information, such as an existing dataset $\mD_0$. 
%  of action-reward pairs
% prior distributions or
We focus on estimating the value difference $V(\pi_1) - V(\pi_0)$, although several other estimands (e.g., $V(\pi_1)$) can be addressed similarly. 
% Although a few OPE tasks (e.g., estimating $V(\pi_1)$) can be addressed similarly following our discussions, for concreteness, we focus on , since it is closely related to the deployment decision making. 
In practice, OPE methods are commonly used to estimate this lift and test its significance using existing data, which determines the deployment decision. 
However, the dataset is typically assumed as well explored, and 
little attention has been paid to how it arises. 
We aim to fill this gap. 
% limited attention has been paid to the dataset itself and we aim to fill this gap. 
Specifically, given an \emph{exploration budget $T$}, a \emph{risk tolerance $\epsilon \in (0,1)$}, and a user-specified estimator that maps a dataset $\mD$ to a value estimate of policy $\pi$ as $\widehat{V}(\pi; \mD)$, 
we aim to design an \emph{exploration policy $\pi_e$} to collect a dataset $\mD_e$ of size $T$, while achieving the following two objectives simultaneously: 
% We aim to 

% How $\mD$ arises is never questioned. We study the problem of collecting $\mD$ to decide $V_r(\pi_1) > V_r(\pi_0)$ as efficiently as possible.
% \hl{make it clear that D0 is not always available.}

\begin{itemize}
    \item \textbf{Safety}: Exploration should be safe, in the sense that $V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0)$ holds, either for all problem instances $\vr$ or with a high probability given side information. 
    \item  \textbf{Efficiency}: 
The exploration should be efficient, 
which we define as the minimization of $\var\big(\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)\big)$, i.e., 
the maximization of the evaluation accuracy with the given estimator. 
Specifically, we mainly focus on unbiased value  estimators, and in this case, the variance is closely related to many practical metrics, such as the mean squared error and the statistical power of testing $V(\pi_1) > V(\pi_0)$. 
See Section \ref{sec:testing} for details.
\end{itemize}

% \;\; 1. \textbf{Safety}: Exploration should be safe, in the sense that $V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0)$ holds, either for all problem instances $\vr$ or with a high probability given side information. 




% \;\; 2. \textbf{Efficiency}: 
% The exploration should be efficient, 
% which we define as the minimization of $\var\big(\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)\big)$, i.e., 
% the maximization of the evaluation accuracy with the given estimator. 
% Specifically, we mainly focus on unbiased value  estimators, and in this case, the variance is closely related to many practical metrics, such as the mean squared error and the statistical power of testing $V(\pi_1) > V(\pi_0)$. 
% See Section \ref{sec:testing} for details.

% Following $\pi_e$ to collect $\mathcal{D}_e$,


% of this connection. 

% With the given estimator, 
% the evaluation accuracy is maximized, which we define as the minimization of $\var\big(\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)\big)$. 
% Specifically, we mainly focus on unbiased value  estimators, and in this case, the variance is closely related to many practical metrics, such as the mean squared error and the statistical power of testing $V(\pi_1) > V(\pi_0)$. 
% See Section \ref{sec:testing} for details of this connection. 
% \todob{Let me know if you need help with this. I just made a similar analysis for GLMs. Analyzing the accuracy of the decision is relatively straightforward.}

% \begin{enumerate}
%     % data collection policy
%     \item \textbf{Safety}: the exploration should be safe, in the sense that $V(\pi_e) \ge (1-\epsilon) V(\pi_0)$ holds, either for any problem instances or with high probability given side information. 
%     \item \textbf{Efficiency}: the OPE efficiency is maximized, which we defined as the minimization of $var\big(\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)\big)$. 
%     Specifically, we will mainly focus on the case that the estimator is unbiased, and hence its variance is closely related with many practical metrics, such as the mean squared error and the statistical power of testing $V(\pi_1) > V(\pi_0)$. 
%     % Besides, we focus on $\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)$ instead of $\widehat{V}(\pi_1; \mD_0 \cup \mD_e)$ as a common business objective is to compare $\pi_1$ and $\pi_0$. 
%     % % typically to draw conclusion on if $\pi_1$ is better than $\pi_0$. 
%     % We note that all discussions in this paper can be directly extended to $\widehat{V}(\pi_1; \mD_0 \cup \mD_e)$ as well. 
%     %  $\Mean_{\vx_t \sim p(\vx), A_t \sim \pi_e(\cdot \mid \vx_t)}R_t \ge (1-\epsilon) \sum_t\Mean_{\vx_t \sim p(\vx), A_t \sim \pi_0(\cdot \mid \vx_t)} R_t$ for any problem instance (or with probability at least $\delta$ evaluated using logged dataset? expectation over x?),
% \end{enumerate}
% we would like to find an efficient allocation rule to collect the new dataset $\mD_e$ of size $T$ by following an exploration policy $\pi_e$.  
% The allocation rule is typically derived from an exploration policy $\pi_e$ after certain randomized rounding (will be explained later). 
% An allocation rule selects the $T$ data points jointly. 
% design a \textit{non-adaptive} policy or a \textit{fixed} allocation rule $\pi_e$
% Let $V(\pi)$ be the value of a policy or an allocation rule  $\pi$. 


\textbf{Two existing approaches. }
% collecting data
To satisfy the safety constraint while exploring, the most popular practice \cite{thomas2015high, jiang2016doubly, slivkins2019introduction}, arguably, is to allocate an $\epsilon \in (0, 1)$ 
% \todob{$\in [0, 1]$} 
proportion of the budget to an exploration policy $b'\in \Delta_{K -1}$, 
% \todob{$\in \Delta_{K -1}$} 
and construct a \textit{mixture policy} $\pi_e = \epsilon b' + (1 - \epsilon) \pi_0$. 
The common choice of $b'$ is $\pi_1$ (i.e., on-policy) or the uniform distribution (i.e., random exploration). 
This approach, albeit being safe, could be inefficient. % in many aspects
For example, $\pi_e$ is confined in a small policy class, and as we will show shortly, we can actually obtain a safe policy directly in a larger class via optimization. % from an optimization viewpoint
Besides, even within this policy class, $b'$ needs to be carefully designed and this problem alone is also underexplored. 
% We initiate its study. 
% for a given OPE task, 

% More insights will be provided following our discussions. 
% For example, when the objective is $V(\pi_1) - V(\pi_0)$, we expect more budget to be spent on the arms where $\pi_1$ and $\pi_0$ differ the most. 
% Even when the objective is $V(\pi_1)$, some feature directions (in contextual bandits) may have been well explored in $\mathcal{D}_0$ or will be explored extensively by $\pi_0$, and hence the $\epsilon$ proportion of budget can focus more on the other directions. 
% at least

% where the authors also
Another existing approach is \citet{zhu2021safe}, which also aims to collect high-quality bandit feedback in a safe manner. 
Our approach to handling the safety constraints is partially inspired by this paper. 
However, their targeted application is policy optimization, and hence they propose to maximize $\min_{a \in [K]} \pi_e(a)$, or in other words, they aim to collect data for evaluating \textit{all} policies jointly by reducing uncertainty uniformly. %the worst case and aim
Therefore, their exploration policy is not tailored for evaluation, and will be less efficient without utilizing its specific structure. 
The \name{SEPEC} problem requires a more careful task-oriented analysis and design. 
A concrete example follows below. 

% \todob{It is simply optimization. Minimize variance over ALL policies. We have ONE policy. Because of the latter, we also study the difference of the mean rewards. This is like a dueling bandit, while the prior work is like an MAB.}

% However, their objective is to maximize $\min_{a \in [K]} \pi_e(a)$, or in other words, they consider the worst case and aim to collect data for \textit{any} tasks, with targeted application as policy optimization. 
%  by minimizing the maximum uncertainty over all arms. 


% $K = 3$,
\textbf{Illustrative example.}
We start with analyzing the efficiency in a toy example without safety constraints. 
Consider $\pi_0 = (0.4, 0.1, 0.5)^T$ and $\pi_1 = (0.1, 0.4, 0.5)^T$. 
Then, one immediate observation is that, arm $3$ does not affect the estimate of the value difference $V(\pi_1) - V(\pi_0) = (0.1-0.4)r_1 + (0.4-0.1)r_2 + 0$, and so no budget should be spent on arm $3$ when exploring. 
Therefore, either following $\pi_1$, running A/B experiment (allocating $x\%$ budget to $\pi_1$ and $(100-x)\%$ to $\pi_0$), or using the uniform exploration of \citet{zhu2021safe} is clearly sub-optimal. 
The problem will become even more interesting when we maximize the efficiency with safety constraints, stochastic contexts, and generalization functions.

% side information, 


==> Safe Exploration for OPE [Camera-ready]/2_1_MAB_IPW.tex <==
\subsection{MAB with IPW}\label{sec:MAB_IPW}
% inverse probability weighting
% We start discussing \name{SEPEC} with evaluating an MAB policy using IPW. 
We first apply \name{SEPEC} to evaluating an MAB policy using the IPW estimator, without side information. 
With a dataset $\mD_e = \{(A_t, R_t)\}_{t =1}^T$ collected following $\pi_e$, 
% \todob{Why not just $\pi_e$?}
the IPW estimator is 
\begin{align*}
    \widehat{V}_{IPW}(\pi; \mD_e) = \frac{1}{T}\sum_{t=1}^T \frac{\pi(A_t)}{\pi_e(A_t)}R_t. 
\end{align*} 
% \todob{Why $T^{-1}$ and not $\frac{1}{T}$?}
% logged data $\mD_0$
% where there is no logged dataset $\mD_0$. 
Our objective can be written as
\begin{align*}
            &\argmin_{\pi_e \in \Delta_{K-1}} \var\big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \big)\\
        &s.t. \;\; V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K. 
\end{align*} 
% \todob{[RESOLVED.]This $\argmin$ does not render properly. This is everywhere.}
% Here, we assume the dataset $\mD_e$ is collected by following $A_t \sim \pi_e$. 
% $\{A_t\} \sim Multinomial(T, \pi_e)$
This problem is particularly challenging because (i) the dependency of the objective on $\pi_e$ is complex, 
and (ii) the safety constraint involves the unknown function $V$ and hence is not easy to guarantee. 
% \todob{Say why the above problem is hard to solve. One reason is that $V$ is unknown.}
% and $\widehat{V}_{b,T}(\pi)$ denotes the estimated value of policy $\pi$ after collecting $T$ data points following $\pi_e$. 

\textbf{Objective function.}
We aim to first transform the objective into a tractable form. 
Let $\pi_{\Delta} = \pi_1 - \pi_0$. 
We have 
% \scalebox{0.92}{\parbox{\linewidth}{%
\begin{align}
&T \times \var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)\nonumber\\
&= T \times \var\Big(T^{-1} \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t \Big)\nonumber\\
&= \var_{A_t \sim \pi_e}\Big(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t \Big) \label{eqn:raw_MAB_obj}\\
&= 
\Mean_{A_t \sim \pi_e}\Big[\var(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t | A_t)\Big]\nonumber\\
&\quad+ \var_{A_t \sim \pi_e}\Big[\Mean(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t | A_t)\Big] \nonumber\\
% &= 
% \Mean_{A_t \sim \pi_e}[\frac{\pi^2_{\Delta}(A_t)}{b^2(A_t)}\var(R_t \mid A_t)]
% + \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)] \nonumber\\
&= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \var_{A_t \sim \pi_e}\Big[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r_{A_t}\Big]
 \label{eqn:0_MAB_objective_0}\\
 &= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- c, 
 \label{eqn:0_MAB_objective_1}
\end{align}
% }} 
% \todob{Several comments:
% Line 1: Comment on the extra $T$. It took me a while to understand that you get $1 / T^2$ from the variance and because we only consider one term later, the $T$ cancel out.
% Line 2: Say that this is for any $t \in [T]$.
% % Last line: How is this derived?
% }
where $c = (V(\pi_1) - V(\pi_0))^2$ is independent of $\pi_e$. 
The third equality is due to the law of total variance and the last one is due to $\var(X) = \Mean(X^2) - \Mean^2(X)$. 
We note that \eqref{eqn:0_MAB_objective_1} cannot be optimized directly, 
as $\sigma_a$'s and $r_a$'s are in general unknown. 
In fact, there does not exist a policy $\pi_e$ that achieves global optimum for all instances (see Appendix \ref{sec:Counter-example} for proof). 
% Besides, the fact that the objective involves unknown quantities also highlights the infeasibility of
However, this transformation provides insights into an efficient allocation rule. % for us to design
Without additional information, 
we consider an upper bound of the objective, by replacing $\sigma_a$'s and $r_a$'s with their joint upper bounds. 
% With this relaxation, by design, our policy would be \textit{minimax optimal}, which we formally prove in Section \ref{sec:analysis}. \todob{This sentence breaks the flow. Why do we need it here?}
Our relaxed objective is
\begin{equation}
    \begin{split}
    \argmin_{\pi_e  \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)},
    \end{split}
 \label{eqn:0_MAB_objective_no_constraint}
\end{equation} 
where the feasible set $\Pi_{\Delta} = \{\pi \in \Delta_{K - 1} : \pi(a) > 0 \; \text{if}\; \pi_{\Delta}(a) > 0 \}$ can be easily verified as convex. 
% a convex set. 
% \todob{It the convexity by definition or an additional assumption? We also say this in Sections 3.2 and 3.3.}
This ensures the \textit{positivity assumption} required by IPW \citep{li2015toward}. 
Although commonly assumed, this assumption has been found violated in many OPE applications \citep{sachdeva2020off, tran2021combining}, where IPW methods can fail catastrophically. 
This is particularly severe with contextual bandits or large action space. 
\name{SEPEC} proactively resolves this issue. 
Finally, without safety constraints, 
the solution of \eqref{eqn:0_MAB_objective_no_constraint} is $\pi_e(a) \propto |\pi_{\Delta}(a)|$. 
This result is intuitive: the larger the difference, the more we explore.
% \todob{Should not this be $\pi_e(a) \propto \pi^2_{\Delta}(a)$? Actually what is the optimal policy?}

% The objective of \eqref{eqn:0_MAB_objective_no_constraint} is clearly different with that in \citet{zhu2021safe}, which is $\min_{a \in [K]} \pi_e(a)$. 
% This simple setup provides insights into why a task-specific design is necessary. 
% \todob{I would drop this paragraph. You were right. It breaks the flow and your earlier comparison to SafeOD makes things clear.}

% optimal policy

% allocation rule is $\pi_e(a) \propto |\pi_{\Delta}(a)|$, similar with the \textit{proportional allocation} in statistical survey \cite{fuller2011sampling}. 
% Again, the exact integer allocations can be solved via randomized rounding. 
% This exactly corresponds to the on-policy strategy. 
% and given the fact the second moment is typically more difficult to estimate than the first moment




% \begin{remark}[Positivity assumption]
% For IPW to be valid, a vital requirement is the positivity assumption, which in our case means 
% $\pi_e(a) > 0$ whenever $\pi_{\Delta}(a) > 0$ (otherwise, there is a division by zero). 
% % a denominator in IPW would be zero). 
% % Otherwise, the estimator is not well-defined. 
% Although commonly assumed, this condition has been found violated in many OPE applications \citep{sachdeva2020off, tran2021combining}, where IPW methods can fail catastrophically. 
% This is particularly severe with contextual bandits or large action space. 
% % In contrast, 
% \name{SEPEC} proactively resolves this issue. 
% % our proposal
% \end{remark} 


We make two remarks regarding the raw objective function \eqref{eqn:0_MAB_objective_0}.
% \todob{It seems that the pointer should be to \eqref{eqn:0_MAB_objective_1}.}
First, perhaps surprisingly, by similar arguments, we can show that the on-policy strategy (i.e., $\pi_e = \pi_1$) is not optimal even in minimizing $\var\big(\widehat{V}(\pi_1; \mD_{e}))$ without safety constraints, when $\sigma_a$'s or $r_a$'s vary across arms. 
Instead, $\pi_e(a) \propto \pi_1(a) \times (r_a^2 + \sigma_a^2)$ is the most efficient one. 
% optimal policy $\pi_e$ since the optimization involves . 
% infeasibility

Second, the two terms of \eqref{eqn:0_MAB_objective_0} correspond to the \textit{intrinsic uncertainty} from the reward noise after pulling  arms and the \textit{extrinsic randomness} from sampling arms. 
% our sampling procedure itself, respectively. 
When $T \gg K$, 
it is possible to (approximately) remove the second term by considering a deterministic allocation. 
Specifically, given $\pi_e$, instead of sampling the $T$ data points, 
we can assign $N_a = T \times \pi_e(a)$ 
% \todob{$T_a$ would be more natural than $N_a$. No need to change if this is too much work.} 
data points to the $a$th arm, which is known as the optimal continuous design in statistics \cite{lee1988constrained}.
However, in general, it is hard to guarantee that $N_a$'s are all integers, and one has to resort to randomized rounding to obtain an allocation $\{N_a\}$ that is close to  $\pi_e$. % the continuous design
Although a few such techniques \cite{bouhtou2010submodularity, allen2017near} can yield small variance inflation when $T \gg K$, they are in general hard to generalize to broader setups such as contextual bandits, where the budget for each context is small and also stochastic. 
This is a setting of sharp difference with the standard experimental design literature. 
Therefore, we choose to sample from $\text{Multinomial}(T, \pi_e)$, which is a popular randomized rounding approach recently \cite{azizi2021fixed, zhu2021safe}. 

% See Appendix \ref{sec:MAB_IPW_alt} for more discussions. 

% there is stochasticity in the contexts and

% By sampling from $\pi_e$ instead of rounding it to form a deterministic allocation, our discussion can be easily extended to accommodate stochastic contexts, which is a setting of sharp difference with the standard experiment design literature. 




% obtain a set of integers $\{N_a\}$ , and the variance inflation is negligible when $K$ is small compared with $T$. % enough

% Notably, when $N_a$'s are all integers, it is easy to see from \eqref{eqn:MAB_objective} that the variance under such an allocation is strictly lower than that under the stochastic allocation. 
% Specifically, the second term of \eqref{eqn:MAB_objective} becomes zero, and the first term remains the same. 
% if use the alternative IPW estimator \textbf{cite here} with estimated propensity, i.e., 
% $|\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \frac{\pi(A_i)}{\pi_e(A_i)}R_i$
% \todorw{the reason I introduce this new estimator is that, $A_t \sim \pi_e$ has no meaning when considering the deterministic allocation. The alternative IPW is also popular in statistics, though might introduce confusion here. Let's discuss. }





% $\{A_t\}_{t=1}^T \sim \text{Multinomial}(T, \pi_e)$, 
% Therefore, we focus on the optimization objective
% \begin{equation*}
%     \begin{split}
%     \argmin_{\pi_e  \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma_a^2
%     \end{split}
% \end{equation*}
% Without safety constraints, 
% the optimal allocation rule is similar with the Neyman allocation in statistics \cite{neyman1992two}, i.e., $\pi_e(a) \propto \sigma_a |\pi_{\Delta}(a)|$. 
% We still define the value of such an continuous allocation rule as $V(\pi_e) = \sum_{a \in [K]} \pi_e(a) r_a$. 


% derivations in \eqref{eqn:MAB_objective}  may not hold any longer. That is why I introduced a new IPW
% " " does not make sense any longer



% \textbf{Safety constraint.}
\textbf{Optimization without side information.}
With a tractable and appropriate surrogate objective, we are now ready to consider the safety constraint. 
The first observation is that $V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K$ is equivalent to $\pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]$. 
This is because we need to ensure safety even in the worst case. 
% , with no  information on $\vr$. 
Indeed, if there exists at least one arm $a$ such that $\pi_e(a) < (1-\epsilon) \pi_0$, we can always construct an  instance to violate the constraint, with $r_a = 1$ and $r_{a'} = 0, \forall a' \neq a$. Thus our optimization problem is
% for our OPE task: 
% continuous design
\begin{equation}
    \begin{split}
    % \Delta_{K - 1}
        &\argmin_{\pi_e  \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\%
        % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
        &s.t. \;\; \pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K], 
        % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_no_logged}
\end{equation}
and its solution is a safe policy. 
This problem is convex and hence can be efficiently solved by many  optimization algorithms \cite{boyd2004convex}. % convex
% For general values of $\{\sigma_a\}$, though this solution will not be globally optimal,  we can provide upper bounds instead. 

% \begin{equation}
%     \begin{split}
%     % \Delta_{K - 1}
%         &\argmin_{\pi_e  \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\
%         % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
%         &s.t. \;\; \pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]. 
%         % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
%     \end{split}
%     \label{eqn:MAB_IPW_no_logged}
% \end{equation}


% \begin{figure}
%     \centering
%     \includegraphics[width = 10cm]{Fig/MAB.png}
%     \caption{MAB: $V(\pi_1)$}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}

% 


\textbf{Utilization of side information.}
Next, we study how to improve over  \eqref{eqn:MAB_IPW_no_logged} when there is side information, such as an existing dataset $\mD_0$ generated by a known behavior policy $\pi_b$. 
Typically $\pi_b$ is just $\pi_0$, but could be different. 
% Next, we consider there is side information that allows us to improve over  \eqref{eqn:MAB_IPW_no_logged}. 
% We assume we have a logged dataset $\mD_0$ generated by a known behaviour policy $\pi_b$. 
% $\pi_b$ is assume as known for simplicity, and otherwise it can be estimated via methods standard in OPE. 
% Besides, 
We assume  $\pi_b$ satisfies the positivity assumption; otherwise one can use IPW with a mixed propensity \cite{kallus2021optimal}. 
Specifically, 
we consider IPW with multiple logging policies \cite{kallus2021optimal}, 
and the original problem becomes
% can be written as 
\begin{align*}
    &\argmin_{\pi_e \in \Pi_{\Delta}} 
    % (N+T)^{-2}
    \var \Big(
    \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)} R_t
    + {\sum_{(A_i, R_i) \in \mD_0}} \frac{\pi_{\Delta}(A_i)}{\pi_b(A_i)} R_i
    \Big)\\
    % \label{eqn:MAB_IPW_w_logged_raw}
    % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
    % min_{\vr \in \mathcal{C}_\delta(\mD_0)} 
    &s.t. \;\; V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in \mathcal{C}_\delta(\mD_0). \nonumber
    % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
\end{align*}
Here $\mathcal{C}_\delta(\mD_0)$ is an $(1-\delta)$-confidence region on $\vr$ obtained from $\mD_0$, which can be constructed based on concentration inequalities. 
Alternatively, one can consider a Bayesian viewpoint when there is a prior on $\vr$ that summarizes domain knowledge, and $\mathcal{C}_\delta(\mD_0)$ is the credible region derived from the corresponding posteriors. We assume $\mathcal{C}_\delta(\mD_0)$ is a convex region, which is commonly the case following either approach.
See Appendix \ref{sec:appendix_constraint} for details.
The convexity allows finding the most violated constraint, for any fixed $\pi_e$, efficiently.
% \todob{It is unclear why we require convexity here. Say that this allows finding the most violated constraint, for any fixed $\pi_e$, efficiently.}
As such, the side information helps relax the safety constraint. 
Finally, we notice that for any $\vr$, $V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0)$ is equivalent to  $\vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0$, a linear constraint in $\pi_e$.

In addition, 
the objective      
is equal to
% ${\var \big(
% \sum_{t} R_t \pi_{\Delta}(A_t) / \pi_e(A_t)  \big)
% + \var\big(\sum_{(A_i, R_i) \in \mD_0} R_i \pi_{\Delta}(A_i) /\pi_b(A_i)
% \big)}$, 
\begin{align*}
    \var \Big(
\sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)} R_t \Big)
+ \var\Big(\sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{\pi_b(A_i)} R_i
\Big), 
\end{align*}
thanks to the independence between $\mD_e$ and $\mD_0$. 
The second term does not depend on $\pi_e$ and hence can be dropped in  optimization. 
In other words, perhaps surprisingly, the additional dataset $\mD_0$ does not \textit{directly} enter the objective. 
The main reason is that, every data point contributes independently to the IPW estimator. 
This may not hold for other estimators, as shown for DM in Section \ref{sec:Nonstochastic linear bandits}. 
% be the case

\textbf{Optimization with side information. }
By similar arguments to \eqref{eqn:MAB_IPW_no_logged}, we propose an optimization problem
\begin{equation}
    \begin{split}
        &\argmin_{\pi_e \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\%
        % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
        &s.t. \;\;  \vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \mathcal{C}_\delta(\mD_0). 
        % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_w_logged}
\end{equation}
This problem is particularly challenging as the constraint implicitly contains an \textit{infinite} number of constraints. % linear
We note that, for any finite set $\Theta \subset \Delta_{k-1}$, 
the corresponding constraint $\vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \Theta$ is actually a finite number of linear constraints on $\pi_e$. 
% \todob{This sentence is hard to read and understand. Rephrase.}
Therefore, we propose to solve \eqref{eqn:MAB_IPW_w_logged} by adapting the cutting-plane method \cite{bertsimas1997introduction}. 
Specifically, the cutting-plane method iteratively adds more constraints to a finite set to approximate the convex feasible set, until no constraint in the original problem is violated. 
The convergence analysis is provided in \citet{boyd2007localization}. 
We present the algorithm details in Appendix \ref{sec:optimization_MAB}.

% design subprocedures in an efficient way 
% Euclidean space

% to approximate the infinite set of constraints through adding then one by one
% infinite set

% The underlying principle is to approximate the feasible region of a nonlinear (convex) program by a finite set of closed half spaces and to solve a sequence of approximating linear programs.


% We note that, with IPW as the value estimator, the objective does not change when we also utilize the logged dataset $\mD_0$ in the objective in addition to in the safety constraint. 
% This is because the additive structure of IPW. 
% This may not be the case when we consider other estimators. 
% although it looks like we only utilize the side information (which typically comes from a ) in the safety constraint but not in the objective, 
% and when we only utilize (?) it in the safety constraint




\begin{remark}\label{remark:alternative objective}
Recall that the raw objective \eqref{eqn:0_MAB_objective_1} involves the unknown parameters $\sigma_a$'s and $r_a$'s. 
We relax it using the upper bounds to guarantee the worst-case efficiency. 
% for all instances. % uniformly
When side information is available, 
alternatively, one can try to infer these parameters and consider a different objective function than \eqref{eqn:MAB_IPW_w_logged}, with a Bayesian or high-probability guarantee. 
We discuss this more in Appendix \ref{sec:obj_side_IPW}. 
% We leave this interesting direction for future research. 
\end{remark}
% protect against the worst case. 
% experimental design


==> Safe Exploration for OPE [Camera-ready]/2_2_Contextual_MAB_IPW.tex <==
\subsection{CMAB with IPW}\label{sec:contextual_MAB_IPW}
In this section, we apply \name{SEPEC} to contextual MAB (CMAB). 
% With a bit overload of notations, we introduce the setup as follows. \todob{I do not think that overload much.} 
% We assume there is a finite set of contexts $\mathcal{X}$. % $p$-dimensional 
At every round $t$, we observe a context $\vx_t$ from a finite set of contexts $\mathcal{X}$, choose an arm $A_t \in [K]$, and then receive a stochastic reward $R_t$. 
We similarly define the mean reward ${r(a|\vx)= \Mean[R_t | A_t = a, \vx_t = \vx]}$, the mean reward vector $\vr(\cdot|\vx)\in [0, 1]^K$,  and the policy
$\pi(\cdot|\vx) \in \Delta_{K - 1}$. 
% = (\pi(1|\vx), \dots, \pi(K|\vx))^T 
% vector from concatenating $\vr(\cdot|\vx)$ or $\pi(\cdot|\vx)$ 
We also use $\vr = (\vr(\cdot|\vx))_{\vx\in\mathcal{X}}$ and $\pi = (\pi(\cdot|\vx))_{\vx\in\mathcal{X}}$ to denote the corresponding vector concatenated over $\mathcal{X}$. 
With $\pi_0$ and $\pi_1$ given, we define $\pi_{\Delta}$ as their difference. 
% either the collection or
% \todob{Formally define $\vr$ and $\pi$. $\vr$ is later used as a matrix. So both are matrices?}
% We make the standard assumption that $\vr(\cdot|\vx) \in [0,1]^K, \forall \vx \in \mathcal{X}$. 
For design purpose, we make a common assumption \cite{wu2015algorithms, zhu2021safe} that the context distribution $p(\vx)$ is known, since there is typically a large dataset of contexts. 
% We assume the context distribution $p(\vx)$ is known, which is commonly assumed in the literature \cite{wu2015algorithms, zhu2021safe} as we typically have a large dataset of contexts. 
Let $V_{\vr}(\pi|\vx) = \sum_{a \in [K]} \pi(a|\vx) r(a|\vx)$. 
The policy value is  $V_{\vr}(\pi) = \sum_{\vx\in \mathcal{X}}
p(\vx) V_{\vr}(\pi|\vx)$. 
Define $\Pi_{\Delta} = \{\pi : \pi(a|\vx) > 0 \; \text{if}\; \pi_{\Delta}(a|\vx) > 0, \forall a, \vx\}$. 
%  \in [K], \vx \in \mathcal{X}
% similarly as in the MAB case as the set of policies satisfying the positivity assumption.
% \todob{$\Pi_{\Delta}(\vx)$ is undefined.}
$\Pi_{\Delta}$ is a convex set by definition. 
% \todob{It the convexity by definition or an additional assumption? We also say this in Sections 3.1 and 3.3.}
% , where $\Pi_{\Delta}(\vx) = \{\pi {\in} \Delta_{K - 1} {:} \pi(a|\vx) > 0 \; \text{if}\; \pi_{\Delta}(a|\vx) > 0 \}$

% (\vx_i, A_i, R_i) \in \mD
For any dataset $\mD_e = \{(\vx_t, A_t, R_t)\}_{t=1}^T$ collected following a policy $\pi_e$, 
we consider the IPW estimator 
$\widehat{V}_{IPW}(\pi; \mD_e) = T^{-1}\sum_{t=1}^T \frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t$. 
Without side information, our problem is defined as 
\begin{equation}
    \begin{split}
        &\argmin_{\pi_e\in \Pi_{\Delta}} T \times \var\big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \big)\\
        &s.t. \;\; V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^{K |\mathcal{X}|}. %  \times
        % &\quad\quad 
        % \pi_e(\cdot | \vx) \in \Pi_{\Delta}(\vx), \forall \vx \in \mathcal{X}. 
    \end{split}
    \label{eqn:goal_CMAB}
\end{equation} 
We aim to construct an efficient and safe exploration policy as in the MAB (Section \ref{sec:MAB_IPW}). 
The main additional challenges come from the stochasticity in the contexts and that we need to solve the problem jointly over all contexts. 


% For IPW to be valid, a vital requirement is the positivity assumption, which in our case means 
% $\pi_e(a) > 0$ whenever $\pi_{\Delta}(a) > 0$ (otherwise, there is a division by zero). 
% % a denominator in IPW would be zero). 
% % Otherwise, the estimator is not well-defined. 
% Although commonly assumed, this condition has been found violated in many applications \citep{tran2021combining, sachdeva2020off}, where existing IPW methods can fail catastrophically. 
% This is particularly severe when we consider contextual bandits or when the action space is large. 
% In contrast, our proposal proactively resolves this issue. 

% Besides, the concerns over the potential confounding variables  is another common reason to challenge OPE with logged data and require \textit{actively} collecting some data. 
% % motivation to consider  some experiment data, on the basis of which we can then evaluate an policy. 


\textbf{No side information.}
We begin with studying the case without side information. 
We first note that our objective 
% \begin{align*} can be decomposed as
%     &T \times \var(\widehat{V}_{IPW}(\pi_1; \mD_e) - \widehat{V}_{IPW}(\pi_0; \mD_e))\nonumber\\
%     % &= 
%     % T^{-1} \var \Big(\sum_t \frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\\
%         % &= \var \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\nonumber\\
%         &= 
%         \Mean_{\vx_t \sim p(\vx)}
%         \Big\{
%         \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}\nonumber\\
%         &\quad +
%         \var_{\vx_t \sim p(\vx)}
%         \Big\{ \Mean[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}. 
% \end{align*}
% $T \times \var(\widehat{V}_{IPW}(\pi_1; \mD_e) - \widehat{V}_{IPW}(\pi_0; \mD_e))$ 
in \eqref{eqn:goal_CMAB} can be decomposed as 
% \todob{We sometimes refer to problems as "(x)" and sometimes as "Problem (x)". Choose one and stick to it.}
\begin{align*}
&\Mean_{\vx_t \sim p(\vx)}
\big\{
\var[ \big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \big) | \vx_t]
\big\}\\
&\quad+ 
\var_{\vx_t \sim p(\vx)}
\big\{ \Mean[ \big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \big) | \vx_t]
\big\}. 
\end{align*}
% the sum of 
% $\Mean_{\vx_t \sim p(\vx)}
% \big\{
% \var[ \big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \big) | \vx_t]
% \big\}$
% and 
% $\var_{\vx_t \sim p(\vx)}
% \big\{ \Mean[ \big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \big) | \vx_t]
% \big\}$. 
The second term is equal to
\begin{align*}
    \var_{\vx_t \sim p(\vx)}\big[\sum_{a \in [K]} \pi_{\Delta} (a | \vx_t) r(a|\vx_t)\big], 
\end{align*}
does not depend on $\pi_e$, and hence can be dropped in  optimization. 
The first term can be regarded as the expectation of the MAB objective \eqref{eqn:raw_MAB_obj} over the context distribution. 
% Again, the total variance decomposition allows us to simplify the optimization objective. 
% \todob{It is unclear what this refers to. In particular, I see that you applied the decomposition to $x_t$ above. However, to derive the final result, it also needs to be applied to $A_t$.}

The second observation is that, 
the safety constraint is equivalent to $\pi_e(\cdot| \vx) \ge (1-\epsilon) \pi_0(\cdot| \vx), \forall \vx \in \mathcal{X}$. 
Otherwise, one can always construct a counter-example by setting $\vr(\cdot|\vx) = \vzero$, except for one context $\vx'$ where the constraint is violated. 
Then, we have $V(\pi_e) = p(\vx')V(\pi_e|\vx') < (1-\epsilon) p(\vx')V(\pi_0|\vx')
= (1-\epsilon) V(\pi_0)$, when $p(\vx') > 0$. 

% to ensure the safety constraint is satisfied, we need to impose 

% % \scalebox{0.85}{\parbox{\linewidth}{%
% \begin{align*}
% &\Mean_{\vx_t \sim p(\vx)}
% \Big\{
% \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
% \Big\}\\
% &\quad+
% \var_{\vx_t \sim p(\vx)}
% \Big\{ \Mean[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
% \Big\}. 
% \end{align*}
% % }}
% Here, the second term is equal to $\var_{\vx_t \sim p(\vx)}\big[\sum_{a \in [K]} \pi_{\Delta} (a | \vx_t) r(a|\vx_t)\big]$, does not depend on $\pi_e$, and hence can be dropped in  optimization. 


% Regarding the objective, we first note the relationship
% \begin{align*}
%     &T \times \var(\widehat{V}_{IPW}(\pi_1; \mD_e) - \widehat{V}_{IPW}(\pi_0; \mD_e))\nonumber\\
%     % &= 
%     % T^{-1} \var \Big(\sum_t \frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\\
%         % &= \var \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\nonumber\\
%         &= 
%         \Mean_{\vx_t \sim p(\vx)}
%         \Big\{
%         \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}\nonumber\\
%         &\quad +
%         \var_{\vx_t \sim p(\vx)}
%         \Big\{ \Mean[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}. 
% \end{align*}
% _{\vx \sim p(\vx)}
% we can focus on the first term of \eqref{eqn:CMAB_IPW_raw}, and 
% the equivalent form of the constraint and on

        % \label{eqn:CMAB_IPW_raw}
        % &= const + 
        % \Mean_{\vx_t \sim p(\vx)} 
        % \Big\{
        % \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
        % \Big\}
    % &= \var(\frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t)\\
    % &= 
    % \Mean_{\vx_t \sim p(\vx)} \Big[ \var(\frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t) | \vx_t \Big]
    % + \var_{\vx_t \sim p(\vx)}\Big[ \Mean(\frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t | \vx_t) \Big]\\
    % &=  \sum_{\vx \in \mathcal{X}}  p(\vx) \Big[ \var(\frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t) \Big] + \var_{\vx_t \sim p(\vx)}\Big[ \Mean(\frac{\pi(A_t|\vx_t)}{\pi_e(A_t|\vx_t)}R_t | \vx_t) \Big], 





% \scalebox{0.85}{\parbox{\linewidth}{%
% \begin{align*}
%     T {\times} \var(\widehat{V}(\pi_1; \mD_e) - \widehat{V}(\pi_0; \mD_e))
%          &= \Mean_{\vx_t \sim p(\vx)}
%         \Big\{
%         \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}\nonumber\\
%          &+
%         \var_{\vx_t \sim p(\vx)}
%         \Big\{ \Mean[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
%         \Big\}. 
% \end{align*}
% }}
% Besides, 
% at first glance, it could challenging to additionally account for  and it is complicated to 
% when we use IPW, since there is no generalization across contexts, 
% using similar arguments, 
% $T \times \var(\widehat{V}_{IPW}(\pi_1; \mD_e) - \widehat{V}_{IPW}(\pi_0; \mD_e))
% % &= 
% % T^{-1} \var \Big(\sum_t \frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\\
% % &= \var \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big)\nonumber\\
% = 
% \Mean_{\vx_t \sim p(\vx)}
% \Big\{
% \var[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
% \Big\}
% {+}
% \var_{\vx_t \sim p(\vx)}
% \Big\{ \Mean[ \Big(\frac{\pi_{\Delta} (A_t | \vx_t) }{\pi_e(A_t | \vx_t)}R_t \Big) | \vx_t]
% \Big\}.$
% Specifically, we note that 

Therefore, by similar arguments as in Section \ref{sec:MAB_IPW} on deriving the surrogate objective, we propose the following tractable optimization problem
\begin{equation*}
    \begin{split}
        &\argmin_{\pi_e\in \Pi_{\Delta}} \sum_{\vx \in \mathcal{X}} \sum_{a \in [K]} p(\vx) \frac{\pi^2_{\Delta}(a| \vx)}{\pi_e(a| \vx)} \\
        &s.t. \;\; \pi_e(\cdot| \vx) \ge (1-\epsilon) \pi_0(\cdot| \vx), \forall \vx \in \mathcal{X},
        % \\
        % &\quad\quad 
        % \pi_e(\cdot | \vx) \in \Pi_{\Delta}(\vx), \forall \vx \in \mathcal{X}, 
        % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
\end{equation*}
which can be solved by optimizing 
\begin{equation}
    \begin{split}
        &\argmin_{\pi_e(\cdot | \vx) \in \Pi_{\Delta}(\vx)} \sum_a \frac{\pi^2_{\Delta}(a| \vx)}{\pi_e(a| \vx)} \\
        % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
        &s.t. \;\; \pi_e(\cdot| \vx) \ge (1-\epsilon) \pi_0(\cdot| \vx), 
        % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:CMAB_IPW_single}
\end{equation}
for each context $\vx \in \mathcal{X}$ separately. 
This is due to the additive form of IPW and the worst-case safety constraint. 
% reduces to one constraint for every context.
% However, thanks to , the optimization problem can be decomposed elegantly and we can actually solve for every context $\vx \in \mathcal{X}$ separately. 
The optimization can be done similarly to \eqref{eqn:MAB_IPW_no_logged}. 
% although the optimization need to be done in real time based on the
% At first glance, it is challenging to additionally account for the stochasticity in the contexts.  
% However, when we use IPW, since there is no generalization across contexts, 
% using similar arguments, 
% we can show that a good design can be obtained by solving for every context $\vx \in \mathcal{X}$ independently (suppose we consider the worst case): \todob{This needs to be explained better. I suggest that we start with (12) and then clearly say why the optimization problem decomposes, when $L$ and $U$ are unbounded.}

\textbf{Side information.}
The scenario considered above is arguably conservative. 
For instance, one may expect to solve all contexts jointly, which allows us to violate the constraint on some contexts and remedy on the others. 
We next consider the case with side information, e.g., an existing dataset $\mD_0 = \{(\vx_i, A_i, R_i)\}$, that allows us to do so. 
% The side information relaxes us from the worst-case scenario. 

% and hence saves us from the concerns on
% to our objective
Regarding the objective function, 
by similar arguments to the MAB (Section \ref{sec:MAB_IPW}), 
$\mD_0$ only adds a $\pi_e$-independent term that can be dropped.  
However, $\mD_0$ can help us to relax the safety constraint. 
We can similarly construct a high-probability region $\mathcal{C}_\delta(\mD_0)$ such that $\vr \in \mathcal{C}_\delta(\mD_0)$ holds with probability at least $1 - \delta$. 
% We can similarly construct a set of high-probability regions $\mathcal{C}_\delta(\mD_0) = \{\mathcal{C}_\delta(\vx, \mD_0)\}_{\vx \in \mathcal{X}}$ such that the event $\{\vr(\cdot | \vx) \in \mathcal{C}_\delta(\vx, \mD_0), \forall \vx \in \mathcal{X}\}$ holds with probability at least $1 - \delta$. 
% Again, we can consider either a frequentist way to construct $\mathcal{C}_\delta(\mD_0)$ or a Bayesian way when appropriate prior is available. 
An efficient and safe policy can then be obtained from 
% which gives us 
% \scalebox{0.92}{\parbox{\linewidth}{%
\begin{equation}
    \begin{split}
        &\argmin_{\pi_e\in \Pi_{\Delta}} 
        \sum_{\vx} p(\vx)
        \sum_a \frac{\pi^2_{\Delta}(a| \vx)}{\pi_e(a | \vx)} \\
        % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
        &s.t. \sum_{\vx \in \mathcal{X}}   \Big(\pi_e(\cdot | \vx) - (1 - \epsilon) \pi_0(\cdot | \vx) \Big) \\
        &\quad\quad\quad\quad 
       \times p(\vx) \vr(\cdot | \vx)^T \ge 0, \forall \vr \in \mathcal{C}_\delta(\mD_0), %\\
        % &\quad\quad 
        % \pi_e(\cdot | \vx) \in \Pi_{\Delta}(\vx), \forall \vx \in \mathcal{X}, 
        % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
\label{eqn:CMAB_IPW_2}
\end{equation} 
% }}
where we notice that, for every fixed $\vr$, the constraint is linear in $\pi_e$. 
Therefore, similar to \eqref{eqn:MAB_IPW_w_logged}, 
we propose to solve this problem by combining convex optimization algorithms with the cutting-plane method. 
See Appendix \ref{sec:optimization_MAB} for algorithm details. 

% \todorw{This optimization is computationally daunting.}

% \textbf{Extensions.}
% In Section \ref{sec:MAB_IPW} and \ref{sec:contextual_MAB_IPW}, we focus on the IPW estimator. 
% Regarding the direct method, for MAB, it is equal to an alternative IPW-form estimator and we analyze in Appendix XX; for CMAB, discussions in the next section can be applied when we consider a linear generalization function (see Appendix \ref{sec:contextual_LB}). 
% Besides, another popular approach is the doubly robust estimator \cite{dudik2014doubly, kallus2021optimal, su2020doubly}. 
% We find discussions above can be similarly applied when we focus on minimizing the asymptotic variance, since its finite-sample variance does not have a tractable form. 
% See Appendix \ref{sec:DR} for more details. 

% , and one major difference is that 

% Here, $\mathcal{C}_\delta(\mD_0)$ is an $(1-\delta)$-confidence region on $\vr$ obtained from $\mD_0$. 
% For instance, we can construct an $(1-\delta / K)$-confidence interval for each arm separately. 



==> Safe Exploration for OPE [Camera-ready]/2_3_nonstochastic_LB_DM.tex <==
\subsection{Linear bandits with DM}\label{sec:Nonstochastic linear bandits}
% In many practical applications, the number of arms is large and efficient learning algorithms typically rely on a generalization function across arms. 
% Specifically, we focus on the linear generalization function in the section. 
Efficiency learning with a large action space typically relies on generalization functions, which also introduce interesting structures to the design of \name{SEPEC} algorithms. 
% our design problem
To shed light on this, we study linear bandits.  
% consider the following linear bandits setup: 
% \cite{kveton2019perturbed, zhu2021safe, azizi2021fixed}
At round $t$, we choose an arm $\vx_t$ 
% \todob{$x_t$ may confuse the reader because it was fixed and we conditioned on it before. Either stress the difference or use vector $a$ for actions.} 
from a set of arms $\mA$ with size $K$, and then receive a stochastic reward $R_t$. 
Each arm is represented by a $d$-dimensional vector.
Note that we overload notation and use $\vx_t$ to denote the feature vector of the pulled arm, instead of stochastic context. 
% in this section. \todob{Be specific. $x$ is a fixed feature vector associated with the pulled arm, not an uncontrolled context.}
We assume that the expected reward of arm $\vx$ is $r(\vx) = \vx^T \vthe^*$ for some unknown parameter vector $\vthe^*$. 
For design purpose, 
we assume homoscedasticity, i.e., $\var(R_t | A_t) \equiv \sigma^2$. 
% , w.l.o.g. 
% , where $\epsilon_t = R_t - \Mean(R_t | A_t)$. 
% Without loss of generality, we assume $\epsilon_t = R_t - \Mean(R_t | A_t)$ is 1-sub-Gaussian, and $||\vthe^*||_2 \le 1$. 
We use most notation introduced in the MAB. 
% A policy $\pi$ which is a distribution over these arms. 
We remark that $V_{\vthe^*}(\pi) =  (\sum_{\vx \in \mA} \pi(\vx) \vx)^T \vthe^* = \bar{\vphi}^T_{\pi} \vthe^*$, where $\bar{\vphi}_{\pi} = \sum_{\vx \in \mA} \pi(\vx) \vx$ is the mean feature direction of $\pi$. We assume that $V_{\vthe^*}(\pi_0) \ge 0$. 
% \begin{align*}
%   V(\pi) =  (\sum_{\vx \in \mA} \pi(\vx) \vx)^T \vthe = \bar{\vphi}^T_{\pi} \vthe. 
% \end{align*}
% \begin{equation*}
%     \begin{split}
%           V(\pi) =  (\sum_{\vx \in \mA} \pi(\vx) \vx)^T \vthe = \bar{\vphi}^T_{\pi} \vthe. 
%     \end{split}
% \end{equation*}

To estimate the value of a policy $\pi$, 
we consider the direct method \citep[DM, ][]{dudik2014doubly}. 
% Let $\boldsymbol{M}^+$ be the Moore–Penrose inverse of matrix $\boldsymbol{M}$. 
With a dataset $\mD = \{(\vx_i, R_i)\}$, 
DM first estimates $\vthe^*$ via least-square regression as $\hat{\vthe} = (\sum_{(\vx_i, R_i) \in \mD} \vx_i \vx_i^T)^+ (\sum_{(\vx_i, R_i) \in \mD} \vx_i R_i)$, and then 
plugs-in $\hat{\vthe}$ in the value definition to construct $\widehat{V}_{DM}(\pi; \mD)  = \sum_{\vx \in \mA} \pi(\vx) (\vx^T \hat{\vthe})= \bar{\vphi}^T_{\pi} \hat{\vthe}$. 
% \widehat{V}_{\hat{\vthe}}(\pi)
% We may sometimes write this estimator as $\widehat{V}_{DM}(\pi; \mD)$ to emphasize its dependency on $\mD$. 

% We aim to decide the set of arms $\vPhi = (\vx_1, \dots, \vx_T)^T$ that we are going to pull in the $T$ rounds, so that the value estimate after receiving the corresponding rewards has small variance. 

\textbf{Objective function.}
We pull $T$ arms $\vPhi = (\vx_1, \dots, \vx_T)^T$ to collect a  dataset $\mD_{\vPhi}$, which is stochastic and depends on $\vPhi$. 
% so that the value estimator has small variance. %high-quality
% We use $\mD_{\vPhi}$ to emphasize the dataset
In this section, we directly consider the case with side information, since it does not make a  significant difference in derivations. 
We assume we have an existing dataset $\mD_0$ and denote the corresponding feature matrix as $\vPhi_0$, which we assume is full-rank.  
Its existence simplifies our exposition. 
Alternatively, one can always use forced exploration to form a basis, or consider regularized least squares. % pull $d$ arms and
Towards the goal of variance minimization, we note that
\scalebox{0.92}{\parbox{\linewidth}{%
% {\small
\begin{align}
&\var_{\vPhi \sim \pi_e} \Big(\widehat{V}_{DM}(\pi_1; \mD_0 \cup \mD_{\vPhi}) - \widehat{V}_{DM}(\pi_0;\mD_0 \cup \mD_{\vPhi}) \Big)\nonumber\\
&= 
\Mean_{\vPhi \sim \pi_e}\Big[\var \Big(\widehat{V}_{DM}(\pi_1; \mD_0 \cup \mD_{\vPhi}) - \widehat{V}_{DM}(\pi_0; \mD_0 \cup \mD_{\vPhi}) | \vPhi \Big)
 \Big]\nonumber\\
&\;+ \var_{\vPhi \sim \pi_e}\Big[ \Mean \Big(\widehat{V}_{DM}(\pi_1; \mD_0 \cup\mD_{\vPhi}) - \widehat{V}_{DM}(\pi_0; \mD_0 \cup\mD_{\vPhi}) | \vPhi \Big)
\Big]\nonumber\\
&= 
\sigma^2
\Mean_{\vPhi \sim \pi_e}\Big[\bar{\vphi}^T_{\Delta \pi}
     (\vPhi^T\vPhi+ \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}
 \Big]\nonumber\\
&\quad\quad + \var_{\vPhi \sim \pi_e}[V(\pi_1) {-} V(\pi_0)]\nonumber\\
&= 
\sigma^2
\Mean_{\vPhi \sim \pi_e}\Big[\bar{\vphi}^T_{\Delta \pi}
     (\vPhi^T\vPhi+ \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}
 \Big] + 0. 
% = \bar{\vphi}^T_{\Delta \pi}
%      (\vPhi^T\vPhi)^{-1}
%     \bar{\vphi}_{\Delta \pi}. 
    \label{eqn:raw_LB}
\end{align}
}} 
% }
% \todob{I do not follow how we get $0$ from unbiasedness.}
The generalization function introduces interesting structures. %to our problem
For example, unlike in IPW, $\mD_0$ also enters our optimization objective, since actions are related through their features. 
Intuitively, we should spend less budget on those extensively explored directions. 
% this sentence can be removed. Not that insightful. 
Moreover, unlike IPW, the second term of \eqref{eqn:raw_LB} is zero. 
This is because, conditioned on any set of sampled arms $\vPhi$, DM estimator is always unbiased and hence its conditional expectation is independent with $\vPhi$. 

% In contrast, this does not hold for IPW, as its unbiasedness requires taking the sampling and estimation as a whole. 


% \begin{align}
% &\var \Big(\widehat{V}_{DM}(\pi_1; \mD_{\vPhi}) - \widehat{V}_{DM}(\pi_0; \mD_{\vPhi}) \mid \vPhi \Big)\nonumber\\
% &\quad = \bar{\vphi}^T_{\Delta \pi}
%     \var(\hat{\vthe} \mid \vPhi)
%     \bar{\vphi}_{\Delta \pi}
% \le \bar{\vphi}^T_{\Delta \pi}
%      (\vPhi^T\vPhi)^{-1}
%     \bar{\vphi}_{\Delta \pi}. 
%     \label{eqn:raw_LB}
% \end{align}

% Here, without additional information on the noise level related to each arm, we again relax the objective using their joint upper bound, which leads to the last inequality. 

% G-optimal allocation problem in the optimal experiment design literature \cite{shah2012theory},
The optimization of \eqref{eqn:raw_LB} is very challenging, since it involves an expectation over the inverse of a random matrix. 
We notice that this objective is related to the G-optimal experiment design problem \cite{shah2012theory}, where we aim to minimize the maximum uncertainty 
by $\argmin_{\vPhi} \max_{\Tilde{\vx} \in \mathcal{X}} \Tilde{\vx}^T (\vPhi^T\vPhi)^{-1} \Tilde{\vx}$. 
For this problem, since a direct optimization is still NP-hard, 
it is common to solve its continuous relaxation \cite{shah2012theory, zhu2021safe} 
$\argmin_{\pi_e} \max_{\Tilde{\vx} \in \mathcal{X}} \Tilde{\vx}^T  (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T)^{-1} \Tilde{\vx}$, and then apply certain randomized rounding methods to construct $\{\vx_1, \dots, \vx_T\}$ from the distribution $\pi_e$. 


% alternatively, one can go with this approach.
Motivated by the good property of this approximation \cite{shah2012theory, lattimore2020bandit}, 
we consider a similar relaxation for our problem as % continuous
\begin{align*}%\Delta_{K-1}
\argmin_{\pi_e \in \Pi'_{\Delta}}  \bar{\vphi}^T_{\Delta \pi}
     (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T + \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi},  
    % \label{eqn:raw_LB_continuous}
\end{align*} 
% \todob{Several bugs? $\max$ should be $\min$. $b$ should be $\pi_e$. Why do we need the extra $T$?}
where $\Pi'_{\Delta} = \{\pi \in \Delta_{K - 1} {:} \sum_{\vx \in \mathcal{A}} \pi(\vx) \vx \vx^T \, \text{is invertible} \}$ is a convex set by definition. 
In Section \ref{sec:analysis}, we prove that this objective is actually the \textit{asymptotic variance} of the DM estimator. 

% \begin{remark}
% By considering $K = d$ and indicator vectors as the feature vectors, we notice this problem reduces to the IPW problem. 
% This connection provides insights and show the potential generalizability of our framework. 
% \end{remark}

% Since the covariance matrices are unrestricted here, the formulation in this section also shows how to generalize Section 3.1 to arbitrary covariance matrices.

% converges to our raw objective. 
% function
% (which also implies the convergence of the solution). 
% To our knowledge, this is the first guarantee of this type. 

% By sampling from $\pi_e$ instead of rounding it to form a deterministic allocation, our discussion can be easily extended to accommodate stochastic contexts, which is a setting of sharp difference with the standard experiment design literature. 

% the other is hard to be applied to contextual
% But when need T -> inf


% % The optimization of \eqref{eqn:raw_LB} over $\vPhi$ is related to the G-optimal design in the optimal experiment design literature \cite{shah2012theory}. 
% % g/d-optimal is maximize over all, etc. none of them consider a special case as we did?
% Similar with our previous discussions for MAB, 
% % a direct optimization of \eqref{eqn:raw_LB} with respect to $\vPhi$ is knonw as NP-hard. 
% Therefore, for this kind of problem, people typically resort to its continuous relaxation \cite{shah2012theory, zhu2021safe}. 
% Specifically, we consider first solving 
% \begin{align*}
% \argmax_{b \in \Delta_{K-1}}  \bar{\vphi}^T_{\Delta \pi}
%      (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T)^{-1}
%     \bar{\vphi}_{\Delta \pi}, 
%     % \label{eqn:raw_LB_continuous}
% \end{align*}
% and then apply certain randomized rounding methods to construct $\{\vx_1, \dots, \vx_T\}$ from the distribution $\pi_e$. 
% An viable choice is to sample from the corresponding multinomial distribution. 
% Here, $T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T$ serves as a continuous approximation of $\vPhi^T \vPhi$. 

\textbf{Optimization.}
After obtaining a tractable objective function, we next study solving the exploration policy with the safety constraint. 
% and the logged dataset $\mD_0$, as considering them separately does not make much difference in this setup. 
Again, we can construct a high-probability region $\mathcal{C}_\delta(\mD_0)$ for $\vthe$ in either a frequentist way or a Bayesian way. 
With either approach, the region is typically an ellipsoid and hence convex, which we assume hereinafter.
See Appendix \ref{sec:appendix_constraint} for some examples.
The convexity allows finding the most violated constraint, for any fixed $\pi_e$, efficiently.
% \todob{It is unclear why we require convexity here. Say that this allows finding the most violated constraint, for any fixed $\pi_e$, efficiently.}
% $\mD_0$ provides information on $\vthe$ and allows us to relax the safety constraint. 
% Following similar derivations as in \eqref{eqn:raw_LB}, we propose to consider the following problem: 
The exploration policy can be obtained from
\begin{equation}
    \begin{split}
&\argmin_{\pi_e \in \Pi'_{\Delta}} \;
% \mJ(\pi_e) = 
\bar{\vphi}^T_{\Delta \pi}
    % (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T
    % + \vPhi_0^{T}\vPhi_0)^{-1} (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T) 
    (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}\\
% &s.t. \; \min_{\vthe \in \mathcal{C}_\delta(\mD_0)} \big(\pi_e - (1-\epsilon) \pi_0 \big) \mX \vthe \ge  0, 
&s.t. \; V_{\vthe}(\pi_e) \ge (1-\epsilon)V_{\vthe}(\pi_0)  , \forall \vthe \in \mathcal{C}_\delta(\mD_0). 
    \end{split}
    % \big((1-\epsilon) \pi_0 - \pi_e\big)^T \mX \vthe \le  0
\label{eqn:nonstochastic linear bandit with side info}
\end{equation} 
%  \in \mathbb{R}^{|\mA| \times p}
The constraint is equivalent to $ \big(\pi_e - (1-\epsilon) \pi_0\big)^T \mX \vthe \ge  0, \forall \vthe \in \mathcal{C}_\delta(\mD_0)$, 
where $\mX$ is the feature matrix obtained by stacking vectors in $\mA$.
% and $\mD_0$, respectively. 
% We first remark that 
Therefore, Problem \eqref{eqn:nonstochastic linear bandit with side info} is convex. 
For a finite set of constraints, we adapt the popular Frank–Wolfe (FW) algorithm \citep{frank1956algorithm}, which is a projection-free algorithm with good convergence guarantees \citep{jaggi2013revisiting}. 
To handle the infinite number of constraints, we combine the FW algorithm with the cutting-plane method. 
See Appendix \ref{sec:optimization_LB} for details.

% \textbf{Extensions.}
% In this section, we mainly focus on the linear bandits setup with a fixed set of arms and using DM as the value estimator. 
% Our discussions can be similarly extended to at least 
% (i) stochastic contextual linear bandits, where the stochastic context $\vx_t$ and the action $A_t$ together determines a feature vector $\vphi_t = \vphi_{\vx_t, A_t}$ which determines the reward linearly (see Appendix \ref{sec:contextual_LB} for details); 
% (ii) linear bandits with IPW estimator (which is usually referred to as the pseudo-inverse estimator \cite{swaminathan2016off} (see Appendix \ref{sec:PI} for details). 
% The contextual version of the pseudo-inverse estimator is particularly useful when applied to some structured problem such as slate recommendation  \cite{swaminathan2016off}, and our extensions can be applied to these cases as well. 


==> Safe Exploration for OPE [Camera-ready]/2_4_Extensions.tex <==

\subsection{Policy evaluation}\label{sec:PE}

For concreteness, we choose the policy comparison problem to present our methodology. % (estimating $V(\pi_1) - V(\pi_0)$) 
We would like to emphasize that all discussions are equally applicable to evaluating the value of a single policy, i.e., estimating $V(\pi_1)$. 
To see this, note that due to linearity, all discussions on the objective functions still hold, e.g.,  by replacing $\pi_{\Delta}$ in \eqref{eqn:raw_MAB_obj} with $\pi_1$ or $\Bar{\phi}_{\Delta \pi}$ in \eqref{eqn:raw_LB} with $\Bar{\phi}_{\pi_1}$. 
Moreover, the safety constraint is independent of the estimand. 
Therefore, the optimization problem can be formulated and solved in almost the same manner as for policy comparison. 

% to other bandit setups and value estimators

\subsection{Extensions}\label{sec:extensions}
% \todob{I like this framing. We propose a framework and showcase interesting instances throughout.} so far
As we expect and also observed, the specific solution for \name{SEPEC}  vary across different bandit setups, evaluation tasks and value estimators. 
% Although a comprehensive study is hence impossible, % [too negative? but we propose a framework? covering a lot? which is better?]
To initiate the study of this novel area, 
we considered three representative variants covering MAB, contextual problems, generalization functions, IPW and DM. 
Our discussion, derivations and algorithms can be extended to at least the following problems. 
% algorithms

First, for MAB, the DM estimator is equivalent to an alternative IPW-form estimator, which we analyze in Appendix \ref{sec:MAB_DM}. 
Second, for stochastic contextual linear bandits 
where the stochastic context $\vx_t$ and action $A_t$ together generate a feature vector $\vphi_{\vx_t, A_t}$ that determines the reward linearly, 
our analysis for IPW and linear bandits can be combined and extended. 
See Appendix \ref{sec:contextual_LB} for details. 
Third, 
linear bandits with IPW are usually referred to as the pseudo-inverse estimator \cite{swaminathan2016off}, and its contextual version is particularly useful on some structured problems, such as slate recommendation. %  \cite{swaminathan2016off} 
Our analysis in Section \ref{sec:Nonstochastic linear bandits} can be extended to these problems. 
See Appendix \ref{sec:PI} for details. 
Lastly, another popular value estimator is the doubly robust (DR) estimator  \cite{dudik2014doubly}, which combines IPW and DM. 
% , kallus2021optimal, su2020doubly
Discussions in Section \ref{sec:contextual_MAB_IPW} can be similarly applied to minimize the asymptotic variance when DR is used as the value estimator. 
% \todob{It is unclear how this relates to the doubly robust estimator in the previous sentence.}
See Appendix \ref{sec:DR} for details. 
% when we focus on minimizing the asymptotic variance, since its finite-sample variance does not have a tractable form. 


% \ref{sec:Nonstochastic linear bandits}


% In Section \ref{sec:MAB_IPW} and \ref{sec:contextual_MAB_IPW}, we focus on the IPW estimator. 
% Regarding the direct method, for MAB, it is equal to an alternative IPW-form estimator and we analyze in Appendix \ref{sec:MAB_DM}; for CMAB, discussions in the next section can be applied when we consider a linear generalization function (see Appendix \ref{sec:contextual_LB}). 
% Besides, another popular approach is the doubly robust estimator \cite{dudik2014doubly, kallus2021optimal, su2020doubly}. 
% We find discussions above can be similarly applied when we focus on minimizing the asymptotic variance, since its finite-sample variance does not have a tractable form. 
% See Appendix \ref{sec:DR} for more details. 


% \textbf{Extensions.}
% In this section, we mainly focus on the linear bandits setup with a fixed set of arms and using DM as the value estimator. 
% Our discussions can be similarly extended to at least 
% (i) stochastic contextual linear bandits,  (see Appendix \ref{sec:contextual_LB} for details); 
% (ii) linear bandits with IPW estimator (which is usually referred to as the pseudo-inverse estimator \cite{swaminathan2016off} (see Appendix \ref{sec:PI} for details). 
% The contextual version of the pseudo-inverse estimator is particularly useful when applied to some structured problem such as slate recommendation  \cite{swaminathan2016off}, and our extensions can be applied to these cases as well. 



==> Safe Exploration for OPE [Camera-ready]/3_Theory.tex <==

\section{Theoretical Analysis}\label{sec:analysis}
In this section, we provide theoretical analysis for \name{SEPEC}. 
Since our optimization problems can all be solved \textit{exactly}, the safety constraint can be satisfied as promised. % and hence
Therefore, we will focus on the efficiency maximization problem in Section \ref{sec:Efficiency}. 
All proofs are deferred to Appendix \ref{sec:proofs}. 
The connection between our objective and the testing power is discussed in Section 
\ref{sec:testing}. 

\subsection{Efficiency}\label{sec:Efficiency}
% considering the case without constraints, which is itself a novel task. 
% Therefore, we choose to focus on the efficiency maximization problem by 
% considering the case without constraints, which is itself a novel task. 
We first study MAB with IPW. 
The same conclusions can be established for CMAB under similar conditions. 
To provide insights, we first consider the case without side information and safety constraints to derive an explicit form of the overall variance. 
 %  (equivalently, the mean squared error)
Denote $\var(\widehat{V}_{IPW}(\pi_1;\mD_e) - \widehat{V}_{IPW}(\pi_0; \mD_e))$ as $\nu(\pi_e; \vr, \{\sigma_a\})$ when the true parameters are $\vr$ and $\{\sigma_a\}$. 
Denote the solution of \eqref{eqn:0_MAB_objective_no_constraint} as $\pi_e^*$. 
% \todob{$L$ is not a good letter for variance. It seems like a lower confidence bound. I know that $V$ is taken.}
% \todorw{I tried to mean Loss. Maybe $J()$? or $\nu(()$? $\upsilon()$? cost or criteria $c()$? Seems $\nu(()$ is a good choice.} 
% upper bound of
\begin{lemma}\label{lemma:ipw_explicit_form}
% Following $\pi_e^*$ to collect a dataset $\mD_{\pi_e^*}$ and then estiamte the value difference via IPW, 
% Suppose we collect dataset $\mD_{\pi_e^*}$ following $\pi_e^*$ and then estimate the value difference  using IPW. 
% Suppose we collect a size-$T$ dataset $\mD_{\pi_e^*}$ following $\pi_e^*$ and then estimate the value difference using IPW. 
The overall variance $\nu(\pi_e^*; \vr, \{\sigma_a\})$ is 
% The overall variance of the whole exploration and estimation procedure is $\nu(\pi_e^*; \vr, \{\sigma_a\})$ is 
% of $\widehat{V}_{IPW}(\pi_1;\mD_{\pi_e^*}) - \widehat{V}_{IPW}(\pi_0; \mD_{\pi_e^*})$ is 
\scalebox{0.9}{\parbox{\linewidth}{%
\begin{align*}
% \nu(\pi_e^*; \vr, \{\sigma_a\})
% &=  
\frac{1}{T} \big[
\sum_{a \in [K]} |\pi_{\Delta}(a)| {\times}
\sum_{a \in [K]} |\pi_{\Delta}(a)| (\sigma^2_a + r^2_a)
- \big(V(\pi_1) - V(\pi_0)\big)^2
\big]. 
\end{align*}
}}
\end{lemma} 
% \todob{Point to the proof. Is this obvious?}
As expected, the variance decays at rate $T^{-1}$. 
The result is intuitive as it depends on how different the two policies are (i.e., $\sum_a |\pi_{\Delta}(a)|$) and if the difference is more significant on those more important arms (with larger $\sigma^2_a$ or $r^2_a$). 

Next we study the efficiency.
As mentioned in Section \ref{sec:MAB_IPW}, the objective involves unknown parameters and 
there is no policy that always dominates (see Appendix \ref{sec:Counter-example} for proof). % so it is impossible to have
Therefore, to provide insights, we study the minimax performance and the average performance. 
For the former, we consider the set of instance $\mathcal{I} = \{(\vr, \{\sigma_a\}): \vzero \le \vr \le \vone, 0 \le \sigma_a \le \sigma, \forall a \}$. 
For the latter, we consider any instance distribution $Q$ such that 
$\Mean_Q(r_a)$, $\var_Q(r_a)$ and $\Mean_Q(\sigma^2_a)$ all have fixed values across the $K$ arms. 
% \todob{What does "all constants across arms" mean?}
% $\Mean_Q(r_a) = \Mean_Q(r_{a'})$, $\var_Q(r_a) = \var_Q(r_{a'})$ and $\Mean_Q(\sigma^2_a) = \Mean_Q(\sigma^2_a), \forall a, a' \in [K]$. 
For either Problem  \eqref{eqn:0_MAB_objective_no_constraint}, \eqref{eqn:MAB_IPW_no_logged} or \eqref{eqn:MAB_IPW_w_logged}, 
denote the solution (i.e., our policy) as $\pi_e^*$ and the set of feasible policies as $\Pi$. 
Note that $\Pi$ can be different with $\Pi_{\Delta}$, since $\Pi$ may be under safety constraints. 
% \todob{This was $\Pi_\Delta$ before.}
\name{SEPEC} enjoys the following nice properties. 
% We have the following results. 
% $\Mean_Q(r^2_a) = \Mean_Q(r^2_{a'})$
% that satisfy the same safety constraint 
% \hl{Q: should we keep the second one?}
\begin{theorem}\label{thm:mab}
The policy $\pi_e^*$ is minimax optimal, i.e., 
% $ max_{(\vr, {\sigma_a}) \in \mathcal{I}_c}  \nu(\pi_e^*; \vr, {\sigma_a}) = min_{b \in \Pi}  max_{(\vr, {\sigma_a})  \in \mathcal{I}_c} \nu(\pi_e; \vr, {\sigma_a}). $
    % &max_{(\vr, \{\sigma_a\}) \in \mathcal{I}}  \nu(\pi_e^*; \vr, \{\sigma_a\})\\
    % &= min_{\pi_e \in \Pi}  max_{(\vr, \{\sigma_a\})  \in \mathcal{I}} \nu(\pi_e; \vr, \{\sigma_a\}). 
\begin{align*}
    \pi_e^* \in \argmin_{\pi_e \in \Pi} \max_{(\vr, \{\sigma_a\})  \in \mathcal{I}} \; \nu(\pi_e; \vr, \{\sigma_a\}). 
\end{align*}
% for any instance distribution $Q$ such that $\Mean_Q(r^2_a) = \Mean_Q(r^2_{a'})$ and $\Mean_Q(\sigma^2_a) = \Mean_Q(\sigma^2_a)), \forall a, a' \in [K]$, 
The policy $\pi_e^*$ is also the most efficient on average, i.e., 
% $\Mean_{\vr, {\sigma_a} \sim Q} \nu(\pi_e^*; \vr, {\sigma_a}) 
% = min_{\pi_e \in \Pi} \Mean_{\vr, {\sigma_a} \sim Q} \nu(\pi_e; \vr, {\sigma_a}).$
\begin{align*}
\pi_e^* \in \argmin_{\pi_e \in \Pi} \Mean_{(\vr, {\{\sigma_a\}}) \sim Q} \; \nu(\pi_e; \vr, \{\sigma_a\}). 
% \Mean_{\vr, \{\sigma_a\} \sim Q} \nu(\pi_e^*; \vr, \{\sigma_a\}) 
% = min_{\pi_e \in \Pi} \Mean_{\vr, {\sigma_a} \sim Q} \nu(\pi_e; \vr, {\sigma_a}). 
% \le \Mean_{\vr, {\sigma_a} \sim Q}\nu(\pi_e_u; \vr, {\sigma_a}). 
\end{align*}
% where the equality holds if and only if $|\pi_{\Delta}(a)| \equiv c', \forall a \in [K]$, for some constant $c'$. 
\end{theorem}
Finally, we study linear bandits with DM. 
For any policy $\pi_e$, with logged data $\mD_0$, we denote the ultimate objective \eqref{eqn:raw_LB} as $\nu^*(\pi_e; \mD_0)$ 
% = T {\times} \var_{\vPhi \sim b} \big(\widehat{V}_{DM}(\pi_1; \mD_{\vPhi} \cup \mD_0) - \widehat{V}_{DM}(\pi_0; \mD_{\vPhi} \cup \mD_0) \big)
and the surrogate objective 
in \eqref{eqn:nonstochastic linear bandit with side info}
as $\nu(\pi_e;\mD_0)$. 
% $\nu(\pi_e;\mD_0) = T {\times} \bar{\vphi}^T_{\Delta \pi}
% % (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T
% % + \vPhi_0^{T}\vPhi_0)^{-1} (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T) 
% (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{-1}
% \bar{\vphi}_{\Delta \pi}$. 
We have the following promised result. 
\begin{theorem}\label{thm:LB}
% Suppose $\vPhi_0$ is invertible. 
% such that $\pi_e(\vx) \vx \vx^T$ is invertible
For any policy $\pi_e \in \Pi'_{\Delta}$, 
we have $T \times |\nu(\pi_e;\mD_0) - \nu^*(\pi_e; \mD_0)| \to 0$ as $T$ grows. 
In other words, the surrogate objective $\nu(\pi_e;\mD_0)$ is the asymptotic variance of 
$\widehat{V}_{DM}(\pi_1;\mD_0 \cup \mD_e) - \widehat{V}_{DM}(\pi_0; \mD_0 \cup \mD_e)$. 
\end{theorem}
In this sense, we regard our surrogate problem as a good proxy, which we solve \textit{exactly}. 
% our method can
% It also allows us to solve the policy efficiently. 
Moreover, notice that $\nu$ and $\nu^*$ are both continuous. 
Therefore, suppose the optimum is in a compact set where the convergence is uniform, then 
we know $T \times |\nu^*(\pi_e^*;\mD_0) - \min_{\pi_e} \nu^*(\pi_e; \mD_0)| \to 0$,  i.e., $\pi_e^*$ is \textit{asymptotically optimal}. % our policy
We leave the finite-sample analysis for future research and investigate it experimentally here. 

% $|\min_{\pi_e} \nu(\pi_e;\mD_0) - \min_{\pi_e} \nu^*(\pi_e; \mD_0)| {\to} 0$

% optimal in the asymptotic sense. 
% Besides, we can similarly derive when $\vPhi_0$ is not full-rank or $\mD_0$ is empty by considering the regularized least square. 

% uniformly

% \begin{align*}
%     S &= \sqrt{T}\Big( \widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)\\
%     %  &= T^{-1} \sum_t \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t \\
%      &\overset{d}{\to} \normal\Big(V(\pi_1) - V(\pi_0), \var\big(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t\big) \Big)
% \end{align*}
% $\hat{\Delta}(\mD_{e}) =  $

\subsection{Connection with hypothesis testing}\label{sec:testing}
% \textbf{Connection with hypothesis testing.} 
In real applications, one important task is to test whether or not the target policy $\pi_1$ is significantly better than $\pi_0$, which impacts deployment of $\pi_1$. 
Thus we investigate the relationship between the power of such a test and our objective $\var\big(\widehat{V}(\pi_1; \mD_{e}) - \widehat{V}(\pi_0; \mD_{e}) \big)$. 
For simplicity, we discuss MAB with IPW and without side information. 
A similar connection can be established for other setups considered in this paper (see Appendix \ref{sec:other_testing}). 
Specifically, we consider the test
\begin{align*}
    H_0: V(\pi_1) \le V(\pi_0) \quad \text{v.s.} \quad H_1: V(\pi_1) > V(\pi_0). 
\end{align*} 
% $\sigma(\pi_e) = \sqrt{\var\big(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t\big)}$
% $\sigma(\pi_e) = \sqrt{\var(\pi_e(A_t)^{-1}\pi_{\Delta}(A_t)R_t)}$
Denote our variance objective \eqref{eqn:raw_MAB_obj} by $\sigma(\pi_e)$  and let $\hat{\sigma}(\pi_e)$ be a consistent estimator with $\mD_e$ (typically the plug-in estimator with sample variance). 
By the central-limit theorem and the Slutsky’s lemma, we have 
% \scalebox{0.9}{\parbox{\linewidth}{%
% \begin{align*}
% % \frac{\sqrt{T}}{\hat{\sigma}(\pi_e)} 
% \sqrt{T}
% \hat{\sigma}(\pi_e)^{-1}
%     \Big[
%     \big(\widehat{V}(\pi_1; \mD_{e}) 
%     - \widehat{V}(\pi_0; \mD_{e}) \big)
%     - \big(V(\pi_1) - V(\pi_0)\big)
%     \Big]
%     \overset{d}{\to} \normal(0, 1), 
% \end{align*}
% }}
% \scalebox{0.95}{\parbox{\linewidth}{%
\begin{align*}
    \hat{\sigma}(\pi_e)^{-1} \sqrt{T}
    &\Big[
    \big(\widehat{V}(\pi_1; \mD_{e}) 
    - \widehat{V}(\pi_0; \mD_{e}) \big)\\[-1ex]
    &\quad- \big(V(\pi_1) - V(\pi_0)\big)\Big]
    \overset{d}{\to} \normal(0, 1), 
\end{align*}
% }}
% $\hat{\sigma}(\pi_e)^{-1} \sqrt{T}
% \big(\widehat{V}(\pi_1; \mD_{e}) 
% - \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}$
when $T$ grows.  %  \to \infty
Therefore, a popular (asymptotically) $\alpha$-level test \cite{cai2020validation} is to reject the null when 
\begin{align*}
\sqrt{T}\hat{\sigma}(\pi_e)^{-1}
\big(\widehat{V}(\pi_1; \mD_{e}) 
- \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}, 
\end{align*}
where $z_{1-\alpha}$ is  the upper $\alpha$th quantile of the standard normal distribution. 
For any $\Delta > 0$, the (asymptotic) power under the local alternative $H_1 : V(\pi_1) - V(\pi_0) = \Delta / \sqrt{T}$ 
is hence 
$1 - \Phi\big(z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta\big)$, where $\Phi(\cdot)$ is the cumulative distribution function of standard Gaussian. 
Since the other terms are all constant, it is clear that $\sigma(\pi_e)$ determines the power. 
Therefore, with a fixed budget, one can improve the power by designing a better policy $\pi_e$ to reduce $\sigma(\pi_e)$, which corresponds to our objective. 
% The upper bound on the variance hence transforms to the lower bound on the power. 


% in similar ways
% \hl{hold for other settings?}
% both $V(\pi_1) - V(\pi_0)$ and $z_{1-\alpha}$


% $\prob\Big(Z \ge z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta \Big)$
% $Z$ is a standard normal random variable. 


% We regard this as minimal since we assume \textit{zero} information about the instance when designing $\pi_e$ in this setup. 
% (see Remark \ref{remark:alternative objective}). 

% For simplicity, we will consider the case without side information. [we did not utilize...]
% we impose no additional requirements on $Q$ except that all arms are  
% there is no much information  
% [1]
% Our exploration policy is the most efficient policy on average, under the safety constraint. 
% in this sense

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% provide performance guarantee for

==> Safe Exploration for OPE [Camera-ready]/4_Expt.tex <==
\section{Experiments}\label{sec:expt}
In this section, we compare the empirical performance of various methods. 
We focus on three metrics: 
(i) the root mean square error (RMSE) of estimation, which quantifies the  efficiency; 
(ii) the power of detecting $V(\pi_1) > V(\pi_0)$ when it holds, which quantifies the downstream impact; 
and (iii) the loss from safety violation $\max(0, T(1-\epsilon){\times}V(\pi_0) - \sum_{t=1}^T \Mean(R_t | A_t) )$, which quantifies the risk. 
% of an algorithm without safety guardrail. 
% violating the safety constraint. 
% V(\pi_0)
% $\max(0, V(\pi_e) - (1-\epsilon) T^{-1}\sum_t \Mean(R_t | A_t) )$


% , referred to as Safe Exploration for Policy Evaluation (SEPE)
% \textbf{Baselines.}
We compare our method \name{SEPEC} with several baselines. 
The first two are introduced in Section \ref{sec:objective_and_baselines}. 
To recap, the mixture policy $\pi_e = \epsilon \pi_1 + (1-\epsilon) \pi_0$ is a common way to run safe policy comparison, while the Safe Optimal Design (SafeOD) proposed in \citet{zhu2021safe} ignores task-specific structure. 
% design a safe exploration policy
% the uniform distribution
% is good at collecting data but could
Besides, we study the performance of \textit{uniform sampling}, which is a common exploration policy; and \textit{A/B test}, which allocates a half of the budget to $\pi_1$ and the rest to $\pi_0$, and is a common practice for policy comparison.  
Finally, we consider the variant of \name{SEPEC} that does not consider the safety constraint during optimization. 
% , i.e., we solve the corresponding optimization problem with no safety constraint. 
% \todob{Say what \name{SEPEC} without safety constraint is.}
% for ablation study purpose, 

% Finally, for ablation study purpose, we consider two variants of \name{SEPEC}, which do not consider the safety constraint and do not utilize the side  information in designing $\pi_e$, respectively. 

% \textit{pure offline}, which only utilizes information in $\mD_0$ and serves as a baseline

% , for all methods above we only use $\mD_0$ in the final estimation but not in the design of $\pi_e$
% D0 should always be used in the final estimator, o.w., not fair
% So it is a fair comparison. 
% Only use in designing b

\input{Fig/simu_results}

% These two baselines are good at collecting data but have no safety guardrail. 
% We can derive the skyline with the knowledge of true env. 

% We consider two setups to sample $\pi_1$ and $\pi_0$. 
% In the first, 
% to study the power, we need to make sure the alternative hypothesis is true. 
% Therefore, we sample $\Tilde{r}_a \sim \text{Uniform}(0,1)$, set $\pi_0$ as $\pi_0(a) \propto \Tilde{r}_a$, and then set $\pi_1$ as $\pi_1(a) \propto 0.5\Tilde{r}_a +  0.5 r_a$. 
% We run a test of level $5\%$ to detect $V(\pi_1) > V(\pi_0)$ and report the power. 
% In the second, to study the risk, 
% we follow similar procedures to sample $\Tilde{r}_a$, set $\pi_1(a) \propto \Tilde{r}_a$ and $\pi_0(a) \propto 0.5\Tilde{r}_a +  0.5 r_a$. 
% The corresponding results are also used to evaluate RMSE. 
% % we need to make such the alternative hypothesis is true. 
% we sample $\pi_1 \sim \text{Dirichlet}(\vone_K)$, and

% \textbf{Setting.}
For MAB, we set $K = 10$, $T=500$, $\delta = 0.05$, $\sigma_a \equiv 3$, sample $r_a \sim \text{Uniform}(0,1)$, and vary the risk tolerance $\epsilon$. 
% \todob{Why $\sigma_a \equiv 3$ and not $\sigma_a = 3$?}
% the number of data points $T$ that we are going to collect. 
% To generate instances, we sample $r_a \sim \text{Uniform}(0,1)$. 
We assume the noise is Gaussian, and construct $\mathcal{C}_\delta(\mD_0)$ from the posteriors of $\{r_a\}$, with $|\mD_0| = 100$ logged data points and the prior $\normal(r_a, 0.2^2)$ for every arm $a$. 
% To study the three metrics in one setup
To mimic the real applications where risk and opportunity coexist, we generate $\pi_0$ and $\pi_1$ in the following manner: 
we first sample from $\text{Ber}(0.5)$ to determine if the null $H_0 : V(\pi_1) \le V(\pi_0)$ is true. 
If true, we sample $\Tilde{r}_a \sim \text{Uniform}(0,1)$, set $\pi_1$ as $\pi_1(a) \propto \Tilde{r}_a$, and then set $\pi_0$ as $\pi_0(a) \propto 0.5\Tilde{r}_a +  0.5 r_a$. 
If not, we set $\pi_0(a) \propto \Tilde{r}_a$ and $\pi_1(a) \propto 0.5\Tilde{r}_a +  0.5 r_a$.
The results are used to report the RMSEs and risks. 
% \todob{This sentence sounds strange.}
We also run a test of level $5\%$ to detect $V(\pi_1) > V(\pi_0)$, and report the power when $H_1$ is true. 
% while the rejection frequency when 
% $\pi_0 \sim \text{Dirichlet}(\vone_K)$
The configurations for CMAB and linear bandits are similar. 
For CMAB, we consider $30$ contexts with  $\{p(\vx_i)\}$ sampled from $\text{Dirichlet}(\vone_{30})$. % (or every $\pi_1(\cdot | \vx)$) $T$ is adjusted as $500$. 
For linear bandits, we sample $\vthe^*$ from the standard multivariate normal and $\vx$ from the unit sphere uniformly, with $K = 100$, $d=5$, $T = 200$, and $|\mD_0| = 100$. 
A detailed description of experiments is in Appendix 
\ref{sec:more_expt_details}. 
% \todorw{please let me know if the updated setup/results/presentation make sense to you. I think this can be regarded as one unified setup which represents the real situation that we do not know whether $\pi_1$ is better or not. So the risk, efficiency, and power can be seen from one setup.}


\textbf{Results.} 
Results aggregated over $2000$ runs are reported in Figure \ref{fig:simu}. 
Overall, we observe that \name{SEPEC} consistently yields negligible loss from violating the safety constraint, and achieves lower RMSE and higher power compared with the other two safe policies (Mixture and SafeOD). 
The comparison with these two algorithms highlights the importance of carefully designing the exploration policy and utilizing task-specific structures. 
% \todob{It is hard to see the risk of \name{SEPEC} in Figure \ref{fig:simu}. The corresponding plots should be labeled as "risk" and not as "loss".}
On the other hand, the A/B test and uniform exploration have slightly higher efficiency when the risk tolerance is very low, but are fairly risky. 
Moreover, compared with these two algorithms, the variant of \name{SEPEC} without safety constraints consistently shows better efficiency, which further supports the usefulness of a carefully designed exploration policy. 
As expected, when the safety constraint is less tight, the efficiency of \name{SEPEC} increases. 
The cost of satisfying the safety constraint is notably low in linear bandits, which is due to the generalization function.

% In general, we observe that \name{SEPEC} performs similarly to this variant when it is easy to satisfy the safety constraint, as expected. 
% In all cases, RMSEs have positive correlation with the testing power.


To investigate the robustness of the findings, we repeat the experiment under a wide range of parameters in Appendix \ref{sec:more_expt}. 
% , and the findings are similar. 
In addition, to study the performance on real datasets, 
we conduct experiments using the MNIST dataset \cite{deng2012mnist} and present the results in Figure \ref{fig:real}, with more details given in Appendix \ref{sec:MNIST}. 
The findings are consistent. 
% to study the performance on real data. 


% closely follow \citet{zhu2021safe} to


\begin{figure}[!t]
%   \centering
\hspace{-1cm}
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.2cm]{Fig/01201337CMAB_real.pdf}
  \caption{CMAB with IPW.}\label{fig:real_CMAB}
\end{subfigure}%
\hspace{.1cm}
% \hspace{-1cm}
\begin{subfigure}{0.48\textwidth}
  \centering
%   \hspace{-1cm}
  \includegraphics[width=\linewidth, height = 3.2cm]{Fig/01201337LB_real.pdf}
  \caption{Linear bandits with DM.}\label{fig:real_LB}
\end{subfigure}%
\caption{Experiment results on the MNIST dataset. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
For methods that consider the safety constraint, the losses from safety violation are around zero and hence may overlap.}\label{fig:real}
\vspace{-0.4cm}
\end{figure}




% The corresponding results are used to evaluate the power. 
% if V(pi_1) > V(pi_0), then we can observe the power, but NS-EPE will seldomly violate the safety constraint

% T = 200


% \begin{figure}[!t]
% \centering
% % \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
% \begin{subfigure}{.5\textwidth}
%   \centering
%     \vspace{.2cm}
%   \includegraphics[width=\linewidth]{Fig/Linear_diff.png}
%   \vspace{-.15cm}
%   \caption{
%   RMSE
%   }
% \end{subfigure}%
% % \hspace{.3cm}
% % \begin{subfigure}{.7\textwidth}
% %   \vspace{.2cm}
% %   \centering
% %   \includegraphics[width=\linewidth]{Fig/MAB_unsafe_freq.png}
% %   \vspace{-.15cm}
% %   \caption{Safety Constraint
% %   }
% % \end{subfigure}%
% \caption{Linear bandits: Value difference.}\label{fig:linear_bandit_DM}
% \end{figure}


==> Safe Exploration for OPE [Camera-ready]/5_Related_Work.tex <==

\section{Related Work}

\textbf{Off-policy evaluation.}
The OPE literature can be roughly classified as 
% three major approaches: 
the DM \cite{dudik2014doubly}, 
IPW \cite{horvitz1952generalization, li2015toward}, 
and doubly robust estimators \cite{dudik2014doubly, kallus2021optimal, su2020doubly}.
Few of the existing papers pay attention to data quality. 
\citet{oosterhuis2020taking} studies the exploration problem in a very specific ranking task, 
and only IPW is considered with no theoretical guarantee provided. 
\citet{tucker2022variance} is a parallel work that also studies data collection for OPE of bandit policies. 
The paper focuses on CMAB with IPW (and studies several extensions such as evaluating multiple policies), while we provide a more comprehensive study of various bandit setups and value estimators. 
Moreover, neither of the two papers studies the safety issue, which is practically important and introduces non-trivial challenges. 

% Moreover, none of them (except for paper 5 in a very specific problem) studies policy comparison (and its relationship with the testing power), which is of great interest. % power of A/B tests


% For a given OPE task and an estimator, we demonstrate how to analyze and utilize its statistical property to design the exploration policy. 
% For off-policy optimization, 
% \citet{tran2021combining} proposes several online algorithms to collect data to ensure the positivity assumption for IPW. 
% % mitigate. % focuses on the deficient support issue in IPW and
% In contrast, we focus on the statistical efficiency of evaluation,  study a wide variety of bandit setups and value estimators, and consider the safety constraint. 
% % regard statistical efficiency as our goal


% \hl{R2. More related works: (remove that OPO paper?) } 
% We did not include them in the current version because the first three are for an MDP (given the page limit), the fourth is an OPE estimator instead of an exploration policy, the fifth studies a very specific ranking problem and was omitted in the literature search, and the last is posted this February. 
% % However, they are certainly related and we will discuss all of them in the final version. 
% They are related and we will discuss them using the extra page of the final version. 



% Finally, besides these two points, other specific differences include: % with each paper
% (i)  Papers 1-3 study data collection for OPE in RL. 
% In contrast, the bandit setup, albeit simpler in formulation, has nicer structural properties that allow us to address the problem in a more systematic and rigorous way. % , comprehensive
% For example, paper 1 studies sample mean-based estimator and only provides empirical results; 
%     % aims to collect data to construct an efficient
%     paper 2 only studies IPW and fails to consider the existing dataset; 
%     paper 3 is on estimating the risk instead of the value. 
% (iii) Paper 5 studies data collection in a very specific ranking problem. 



% khezeli2020safe, 
\textbf{Conservative bandits.}
Safety constraints have been considered in the conservative bandits literature \cite{wu2016conservative, amani2019linear, moradipari2020stage}, where the key idea is to follow the baseline policy when the next taken action could be risky. 
%  (typically via lower confidence bounds)
This shares similar spirits with the mixture policy. 
% suggested by a bandit algorithm
% def is different
% line of research
Our objective of designing an exploration policy for OPE is orthogonal to this area which aims to minimize the cumulative regret. 
% \todob{We may want to mention that these guys have something to learn from us, because our policies are smarter about being safe.}
% via an adaptive policy. 

% bubeck2011pure, 
\textbf{Pure exploration.}
Similar to our work, the pure exploration literature  \cite{xu2018fully, degenne2019non, azizi2021fixed} aims to maximize the information gain, with the objective of  learning a good policy. 
% Besides cumulative regret minimization, some bandit algorithms target maximizing the information gain or identifying the best arm, which can be classified as the pure exploration problem \cite{bubeck2011pure, xu2018fully, degenne2019non, azizi2021fixed}. 
Our work has a different objective in many aspects: 
we focus on the efficiency of policy evaluation, study non-adaptive policies, and further consider safety constraints. 


\textbf{Optimal experiment design.}
% our problem also belongs to 
Our problem is related to optimal experiment design \cite{allen2017near, baird2018optimal,  fontaine2021online}, where the goal is also to design a high-quality data collection rule for statistical inference. 
% to improve the statistical efficiency for a given inference task. 
% See \citet{pukelsheim2006optimal} for a comprehensive introduction. 
Only a few of these works consider the bandit problem and none of them study OPE. 
We also consider the safety constraint, which is of great practical importance and makes the problem more challenging. 
% regression or treatment effect estimation. 
% contextual setup does not allow us to allocate the T data points fully \textit{a priori}. 




% \textbf{Off-policy evaluation.}
% Our problem is firmly related to the OPE literature. 
% Existing methods can be roughly classified as 
% % three major approaches: 
% the DM \cite{dudik2014doubly}, 
% IPW \cite{horvitz1952generalization, li2015toward}, 
% and doubly robust estimators \cite{dudik2014doubly, kallus2021optimal}. % su2020doubly
% Few of the existing papers pay attention to improving the quality of data. 
% % For a given OPE task and an estimator, we demonstrate how to analyze and utilize its statistical property to design the exploration policy. 
% In the off-policy optimization areas, 
% \citet{tran2021combining} proposes several online algorithms to collect data to ensure the positivity assumption for IPW. 
% % mitigate. % focuses on the deficient support issue in IPW and
% In contrast, we focus on the evaluation task, study a wide variety of bandit setups and value estimators, regard statistical efficiency as our goal, aim to design a non-adaptive exploration policy, and also consider the safety constraint. 
% % Multi-armed bandit problems with history
% % Combining offline learning and online learning


==> Safe Exploration for OPE [Camera-ready]/6_Discussion.tex <==
\vspace{-.1cm}
\section{Conclusions} 
% \todob{Conclusions?}
% \todorw{Hi Brano. Here is a placeholder. Waiting for you :)}
This paper initiates the study of efficient exploration for bandit policy evaluation and additionally considers safety. 
We call this problem \name{SEPEC} and study several of its representative variants. 
At a high level, our work contributes to disentangling exploration and evaluation/optimization in bandits. 
We believe that this direction is of huge practical importance, 
as our exploration strategy is easy to deploy, safe, and enables better statistical inference.
Extensions to the Bayesian setup, sequential design, and reinforcement learning are all interesting next steps. 

In Section \ref{sec:contextual_MAB_IPW}, we assumed a finite context set for simplicity. 
A closer look at the derivations shows that, if there is no side information or we do not plan to use it (e.g., when we want worst-case safety guarantee), then this assumption is not required: 
every time when a new context is observed, 
we can just solve \eqref{eqn:CMAB_IPW_single} once. 
All nice properties are retained. 
In fact, we empirically observed that the efficiency loss is minimal, unless the risk budget is very low.  
The same argument applies when one does not need the safety constraint. 
The action set can be context-dependent as well. 
If one would like to use side information to guarantee high-probability safety with infinite contexts, then $\pi_e(a|\vx)$ must be parameterized (e.g., as a neural network). 
% Given the convexity of our formulation, the problem is still solvable.
% \todob{I am not sure about this. When the policy is parameterized, we would need convexity in its parameters.}
% differentiable & needs to handle the constraint [lagrange; ADMM; [parameterize]
As a trade-off, additional assumptions on the policy class are needed. 
We leave differentiable policies for future research. 
Finally, considering a finite context set covers  applications where the context variables are discrete (e.g., day of the week, gender, age group, etc.). 
% is not rare in the literature and it

% Besides, , all discussions above also apply when $\mathcal{X}$ is infinite, where we can solve  once when a new stochastic context is observed. 


We also assumed in Section \ref{sec:contextual_MAB_IPW} that the context distribution is known. 
This is a common assumption \citep{wu2015algorithms, zhu2021safe} that simplifies theory. 
It is usually reasonable because we typically have a large set of historical contexts. 
If not, one can either
(i) optimize for every context independently as in \eqref{eqn:CMAB_IPW_single}, since possibly there is also not much side information; 
(ii) or replace $p(x)$ in the objective of \eqref{eqn:CMAB_IPW_2} by an upper bound and that in the constraint by a convex confidence region, for which we can similarly solve with a high-probability safety guarantee and worst-case efficiency guarantee.


% \todob{If the work is so important, maybe we can mention some future directions? How about RL or adaptive policies? It does not have to be long.}

% given the challenge of online algorithms to infrastructure, safety, statistical inference, etc. \citep{zhu2021safe}.  

% In many real applications, 
%  is of great importance




% There are a few extensions and future steps of the proposed methodology. 
% First, for concreteness, we focus on estimating $V(\pi_1) - V(\pi_0)$ in derivations. 
% It is easy to check that, thanks to additivity, all discussions can be easily extended to estimating $V(\pi_1)$ or even minimizing 
% $\sum_{j=1}^M w_j \var\big(\widehat{V}(\pi_j; \mD_0 \cup \mD_e)\big)$ (i.e., we would like to evaluate $M$ target policies and their weights are $\{w_j\}$). 
% Besides, additional linear  constraints can be similarly added. 


% \todob{Adaptive policies for data collection? Do we envision any value in the adaptivity?}

% \todorw{Two reasons: 1. the unknown parameters can be inferred better and we can have a different design objective; 
% 2. stochastic context: e.g., by chance, some directions appear more, then we need to adjust.}


% \todob{How is the prior used? We did not do anything Bayesian in this paper.}


% \todob{Explain why this complicated setup. Do we simply want to guarantee that $\pi_1$ beats $\pi_0$ in exactly a half of the cases? I suggest that we simplify the generation of the policies.} 
% \todob{How is this applied to the linear model?}


% \todob{\eqref{eqn:0_MAB_objective_no_constraint} This nicely shows how we differ from SafeOD. Sum over $a$ instead of min. Scaling factor $\pi^2_{\Delta}(a)$. We may want to point this out, to make the difference crystal clear, even in the simplest problem instance.}


%  \todob{I realized that you sometimes use colons in front of math and sometimes not. Choose one style and stick to it. I do not use colons, because I view display math as a continuation of text.}

% \todob{It is strange that policy $\pi_b$ collects dataset $D_0$. On the other hand, $\pi_0$ has nothing to do with $D_0$. Fix this inconsistency.}


% \todob{Why is this a remark and not a part of the text? Also too many details for how simple the message should be.}

%  \todob{Again, as before (reference), the total variance decomposition allows us to simplify the optimized objective.}

% or convex
% versatility

% Most of our discussions directly apply to other estimands such as $V(\pi_1)$, as long as the convexity of the objective function is preserved. 

% \todorw{This graph can save some space? Does it look good to you?}


% \input{Fig/illustration_one_graph}

% Second, for IPW, recall that the raw objective \eqref{eqn:0_MAB_objective_1} is related with $\sigma_a$ and $r(a)$. 
% We choose to relax using the upper bounds to improve the efficiency uniformly for all instances. 
% With side information, it is possible to consider a different surrogate objective function. 
% In that case, one may consider a Bayesian \cite{chaloner1995bayesian} or high-probability statement. 
% % protect against the worst case. 
% % experimental design
% We believe this is an interesting direction and leave it as a future step. 
% % The cost is that we should use high-probability statements when referring to our optimization objective. 
% % such as logged dataset or prior distribution


% \begin{remark}[Confounders]
% Another vital assumption for IPW is the no unmeasured confounders assumption \cite{tsiatis2007semiparametric}, which requires the action assignment mechanism in $\mD$ (i.e. $\pi_e$) is well modelled. 
% This is one main reason why people have concerns about deploying a policy without evaluating using experiment data \cite{sohoney2018handling}. 
% Our proposal actively collects experiment data in an efficient and safe manner. 
% % and makes sure this assumption is valid. 
% \end{remark}


==> Safe Exploration for OPE [Camera-ready]/9_DR.tex <==
\subsection{Doubly robust estimator for MAB and CMAB}\label{sec:DR}
% \begin{align}
% &T \times var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)\nonumber\\
% &= 
% \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
% + var_{A_t \sim \pi_e}\Big[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)\Big]\\
% %  \label{eqn:0_MAB_objective_0}\\
%  &= 
% \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
% + \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2(a)
% - c, 
% %  \label{eqn:0_MAB_objective_1}
% \end{align}

%%%%%%%%
Besides IPW and DM, the doubly robust (DR) estimator is another popular OPE estimator, both in bandits \citep{dudik2014doubly} and in reinforcement learning \citep{shi2021deeply}. % , kallus2021optimal, su2020doubly
We analyze the DR estimator in the MAB setup, and the CMAB case is similar. 
Let $\widehat{V}_{DM}$ be a consistent DM-type estimator. 
The DR value estimator \cite{tsiatis2007semiparametric} is define as 
\begin{align*}
    \widehat{V}_{DR}(\pi_1; \mD_{e}) = \sum_t \frac{\pi_{1}(A_t)}{\pi_e(A_t)} (R_t - \widehat{V}_{DM}(\pi_1; \mD_{e})) + \widehat{V}_{DM}(\pi_1; \mD_{e}). 
\end{align*}
Due to the complex structure, it is well-known that its finite-sample variance does not yield a tractable form as IPW and DM do, and therefore people commonly focus on its asymptotic variance \cite{tsiatis2007semiparametric} 
% in the 2nd equation, the 2nd term tends to have smaller magnitude compared with IPW
% but hard to optimize?
\begin{align*}
&T \times \text{AsmypVar}\Big(\widehat{V}_{DR}(\pi_1; \mD_{e})) \Big)\nonumber\\
% &= 
&= 
\sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} \sigma^2_a 
+ \var_{A_t \sim \pi_e}\Big[\frac{\pi_{1}(A_t)}{\pi_e(A_t)}\big(r_{A_t} - V(\pi_1) \big)\Big]\\
%  \label{eqn:0_MAB_objective_0}\\
 &= 
\sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} \big(r_a - V(\pi_1)\big)^2
- 0. 
% \\
%  &= 
% \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} \sigma^2_a 
% + \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} r^2(a)
% + \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} V(\pi_1)^2
% - \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)} 2r_aV(\pi_1)
%  \label{eqn:0_MAB_objective_1}
\end{align*}
%  in \eqref{eqn:0_MAB_objective_1}
Compared with the form of IPW, one can find that the only difference is that the $r_a^2$ in the second term is replaced by $\big(r_a - V(\pi_1)\big)^2$, which is also related with the unknown parameters. 
Therefore, a tractable optimization objective can be formed by considering the upper bounds as 
\begin{align*}
    \argmin_{\pi_e}  \sum_{a \in [K]} \frac{\pi^2_{1}(a)}{\pi_e(a)}. 
\end{align*}
The other discussions on the safety constraint and the optimization for IPW can then be directly applied here. 
Similar results can be established for $V(\pi_1) - V(\pi_0)$, by noting the additivity. 
% linearity. 

% \hl{Q: work for $V(\pi_1) - V(\pi_0)$? The linearity does not hold for finite sample, and may require some additional analysis.}

==> Safe Exploration for OPE [Camera-ready]/9_IPW_alterantive_objective.tex <==
\subsection{Alternative objective function with side information for IPW}\label{sec:obj_side_IPW}
For MAB with IPW (similar arguments below apply for CMAB), recall that we derived the following form for the overall variance: 
\begin{align*}
T \times \var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)
= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- \big(V(\pi_1) - V(\pi_0) \big)^2, 
\end{align*}
Since either $\sigma_a$, $r_a$, or $V(\pi_1) - V(\pi_0)$ is known, this objective is intractable to directly optimize. 
From the worst-case point of view, we relax them using the upper bounds and optimize the  surrogate objective 
\begin{align*}
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)}. 
\end{align*}
The advantage of this surrogate objective is that, for any instances, we can provide decent performance guarantee. 
However, the downside is such an objective might be conservative. 
In particular, even with side information (dataset $\mD_0$ or posterior distribution $Q$ over instance) available, our utilization of this information is limited (since the corresponding guarantee would be high-probability or Bayesian). 

We discuss alternative surrogate optimization objectives in this section. 
With the posterior distribution $Q$, 
it is easy to see that the objective, which is known as the Bayes risk \citep{brown1990information}, can be formulated as
\begin{align*}
&\Mean_Q \Big\{
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- \big(V(\pi_1) - V(\pi_0) \big)^2
\Big\}\\
&= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \Mean_Q\sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \Mean_Qr^2_a
- \Mean_Q\big(V(\pi_1) - V(\pi_0) \big)^2
\\
&= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} (\Mean_Q\sigma^2_a +\Mean_Qr^2_a)
- \Mean_Q\big(V(\pi_1) - V(\pi_0) \big)^2, 
\end{align*}
which shares similar form with the one in the main text. 
Therefore, all discussions can be extended. 

Regarding the frequentist way, we can utilize $\mD_0$ to construct upper confidence bounds for the unknown terms, and the final performance guarantee would be a high-probability statement. 

==> Safe Exploration for OPE [Camera-ready]/9_MAB_DM.tex <==
\subsection{MAB with DM}\label{sec:MAB_DM}
An alternative estimator for MAB is the direct method (DM). 
In MAB, DM essentially plugs-in the estimated mean of every arm as 
$\widehat{V}(\pi; \mD) = \sum_a \Big[\pi(a) \frac{\sum_{(A_t, R_t) \in \mD} R_t \I(A_t = a)}{\sum_{(A_t, R_t) \in \mD} \I(A_t = a)} \Big]$. 
We note this estimator is actually equivalent to 
$|\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \frac{\pi(A_i)}{\hat{\pi}_e^*(A_i)}R_i$, where $\hat{\pi}_e^*(a) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \I(A_t = a)$, i.e., the IPW-form estimator with the estimated propensity $\hat{\pi}_e^*(a)$. 
A well-known but perhaps counter-intuitive result \cite{brumback2009note} is that, even if $\mD$ is collected by following $\pi_e$ and $\pi_e$ is known, $\widehat{V}_{IPW}(\pi; \mD)$ is still more efficient than plugging-in the known function $\pi_e$. 

The following result is standard \cite{li2015toward} and we just recap here for completeness: 
\begin{align*}
    &\widehat{V}(\pi; \mD) - V(\pi)\\
    &=\sum_a \Big[\pi(a) \frac{\sum_{(A_t, R_t) \in \mD} R_t \I(A_t = a)}{\sum_{(A_t, R_t) \in \mD} \I(A_t = a)} \Big]
    - V(\pi)\\
   &=\sum_a \Big[\pi(a) \big( \frac{\sum_{(A_t, R_t) \in \mD} R_t \I(A_t = a)}{\sum_{(A_t, R_t) \in \mD} \I(A_t = a)}
   - r_a \big)
   \Big]\\
   &=\sum_a \Big[\pi(a) \big( \frac{\sum_{(A_t, R_t) \in \mD} (R_t- r_a) \I(A_t = a)}{\sum_{(A_t, R_t) \in \mD} \I(A_t = a)}
    \big)
   \Big]\\
   &=\sum_a \Big[\pi(a) \big( \frac{ |\mD|^{-1} \sum_{(A_t, R_t) \in \mD} (R_t- r_a) \I(A_t = a)}{|\mD|^{-1} \sum_{(A_t, R_t) \in \mD} \I(A_t = a)}
    \big)
   \Big]\\
   &\convergeD \normal\Big(0, \sum_a \frac{\pi^2(a)}{\pi_e(a)}\sigma_a^2 \Big). 
\end{align*}
By the additivity, we can see this relationship holds for the value difference $V(\pi_1)-V(\pi_0)$ as well. 
All of our discussions on the safety constraints and optimization algorithms can be directly extended to this case. 
Finally, similar extensions can be constructed for CMAB as well. 



% \subsection{Multi-armed bandits  with inverse probability weighting}\label{sec:MAB_IPW_alt}
% We start our discussion with estimating the value of a $K$-armed bandit  policy using the popular inverse probability weighting (IPW) estimator \cite{dudik2014doubly}. 
% For any dataset $\mD = \{(A_i, R_i)\}$, 
% the IPW estimator is defined as 
% $\widehat{V}_{IPW}(\pi; \mD) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \frac{\pi(A_i)}{\hat{\pi}_e^*(A_i)}R_i$, where $\hat{\pi}_e^*(a) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \I(A_t = a)$. 
% Note that here we use the estimated propensity $\hat{\pi}_e^*(a)$. 

% We aim to design the optimal way to collect the new dataset of size $T$, which is equivalent to allocating the $T$ budgets to the $K$ arms. 
% Let $N_a$ be the number of data points assigned to the $a$th arm, 
% set $\pi_e(a) = N_a / T, \forall a \in [K]$, 
% and denote the resulting dataset by $\mD_e$. 

% We first consider the case where there is no logged dataset $\mD_0$. 
% Our objective can then be written as
% \begin{align*}
%             &\argmin_{\pi_e \in \Delta_{K - 1}} var\big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \big)\\
%         &s.t. \;\; V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K. 
% \end{align*}
% This problem is particularly challenging due to (i) the dependency of the objective on $\pi_e$ is complex, 
% and (ii) the safety constraint involves the unknown function $V$ and hence not easy to guarantee. 

% % \textbf{Objective function. }
% We aim to first transform the objective into a tractable form. 
% Let $\pi_{\Delta} = \pi_1 - \pi_0$ and $\sigma^2_a = var(R_t \mid A_t = a), \forall a \in [K]$. 
% We have 
% \begin{align}
% &T \times var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)\nonumber\\
% &= 
% \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
%  \label{eqn:MAB_objective_alt}
% \end{align}
% Without safety constraints, 
% the optimal allocation rule is similar with the Neyman allocation in statistics \cite{neyman1992two}, i.e., $\pi_e(a) \propto \sigma_a |\pi_{\Delta}(a)|$. 
% Besides, perhaps surprisingly, following similar arguments, we can show that the on-policy strategy (i.e., by setting $b = \pi_1$) is not even optimal in minimizing $var\big(\widehat{V}(\pi_1; \mD_{e}))$, 
% when $\sigma_a$'s are different. 

% % $\{A_t\}_{t=1}^T \sim \text{Multinomial}(T, \pi_e)$, 
% %  = T \times \pi_e(a)
% The first challenge to solving \eqref{eqn:MAB_objective} is that, it is hard to guarantee that $N_a$'s are all integers for the minimizer $\pi_e$. 
% However, various randomized rounding techniques \hl{[cite]} can be applied to obtain a set of integers $\{N_a\}$ that is close to the continuous solution, and the variance inflation is guaranteed to be negligible when $K$ is small compared with $T$. % enough

% % derivations in \eqref{eqn:MAB_objective}  may not hold any longer. That is why I introduced a new IPW
% % " " does not make sense any longer
% The second challenge is that $\sigma_a$ is typically not known \textit{a priori}. 
% Without additional information and given the fact the second moment is typically more difficult to estimate than the first moment, 
% we consider an upper bound of the objective, by replacing every $\sigma_a$ with their joint upper bound. 
% With this relaxation, our objective reduces to 
% \begin{equation*}
%     \begin{split}
%     \argmin_{\pi_e  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)}
%     \end{split}
% \end{equation*}
% Without safety constraints, 
% the optimal allocation rule is similar with the proportional allocation in statistics \cite{fuller2011sampling}, i.e., $\pi_e(a) \propto |\pi_{\Delta}(a)|$. 
% % Again, the exact integer allocations can be solved via randomized rounding. 
% % This exactly corresponds to the on-policy strategy. 

% % \textbf{Safety constraint. }
% With a tractable and appropriate surrogate objective, we are now ready to consider the safety constraint $V_{\vr}(\pi_e) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K$. 
% The first observation is that, the constraint is equivalent to $\pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]$. 
% This is mainly due to that there is no any information on $\vr$ and we need to ensure the safety constraint under the worst case. 
% Specifically, 
% when there exists at least one arm $a$ such that $\pi_e(a) < (1-\epsilon) \pi_0$, we can always construct a instance to violate the constraint, where $r(a) = 1$ and $r(a') = 0, \forall a' \neq a$. 

% \textbf{Optimization without side information. }
% Therefore, we finally achieve a desired optimization objective, by solving which we can obtain an efficient and safe continuous design for our OPE task: 
% \begin{equation}
%     \begin{split}
%         &\argmin_{\pi_e  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\
%         % var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
%         &s.t. \;\; \pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K] . 
%         % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
%     \end{split}
%     \label{eqn:MAB_IPW_no_logged_alt}
% \end{equation}
% This problem is convex and hence can be efficiently solved by many convex optimization algorithms \cite{boyd2004convex}. 
% % For general values of $\{\sigma_a\}$, though this solution will not be globally optimal,  we can provide upper bounds instead. 


% % \begin{figure}
% %     \centering
% %     \includegraphics[width = 10cm]{Fig/MAB.png}
% %     \caption{MAB: $V(\pi_1)$}
% %     % \caption{Caption}
% %     % \label{fig:my_label}
% % \end{figure}

% \textbf{Utilization of side information. }
% \hl{update here.!}
% Next, we consider there is side information that allows us to improve on \eqref{eqn:MAB_IPW_no_logged}. 
% We assume we have a logged dataset $\mD_0$ generated by a historical behaviour policy $b_0$. 
% We assume $b_0$ is known for simplicity, and otherwise it can be estimated via methods standard in the OPE literature. 
% We expect the information in $\mD_0$ will have impact on both our objective and safety constraint. 
% Specifically, the original problem can be written as 
% \begin{equation}
%     \begin{split}
%         &\argmin_{\pi_e \in \Delta_{K - 1}} 
%         % (N+T)^{-2}
%         var \Big(
%         \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)} R_t
%         + \sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
%         \Big)\\
%         % var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
%         &s.t. \;\; min_{\vr \in \mathcal{C}_\delta(\mD_0)} \vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0. 
%         % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
%     \end{split}
%     \label{eqn:MAB_IPW_w_logged_raw_alt}
% \end{equation}  
% Here, $\mathcal{C}_\delta(\mD_0)$ is an $(1-\delta)$-confidence region on $\vr$ obtained from $\mD_0$. 
% For instance, we can construct an $(1-\delta / K)$-confidence interval for each arm separately. 
% Alternatively, one may consider a Bayesian setup where there is a prior on $\vr$, and $\mathcal{C}_\delta(\mD_0)$ is the credible intervals derived from the corresponding posteriors. 

% % [\vL(\delta, \mD_0), \vU(\delta, \mD_0)]


% Perhaps surprisingly, thanks to the independence between $\mD_e$ and $\mD_0$, the objective of     \eqref{eqn:MAB_IPW_w_logged_raw} is equal to
% $
% var \Big(
% \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)} R_t \Big)
% + var\Big(\sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
% \Big)$, 
% where the second term does not depend on $\pi_e$ can hence can be dropped in the objective. 
% In other words, the additional dataset $\mD_0$ does not affect the optimization objective. 
% The main reason is that in IPW, every data point contributes independently to the estimator. 
% This may not be the case for some other OPE estimators, as will be shown later. 

% \textbf{Optimization with side information. }
% Therefore, by similar arguments with \eqref{eqn:MAB_IPW_no_logged}, we can consider the following optimization problem
% \begin{equation}
%     \begin{split}
%         &\argmin_{\pi_e \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\
%         % var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
%         &s.t. \;\;  \vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \mathcal{C}_\delta(\mD_0). 
%         % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
%     \end{split}
%     \label{eqn:MAB_IPW_w_logged_alt}
% \end{equation}
% We note this problem is particularly challenging as the constraint implicitly contains a \textit{infinite} number of constraints. 
% With the observation that, for any finite set $\Theta \subset \Delta_{k-1}$, 
% $min_{\vr \in \Theta} \vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0$ is a system of linear constraints. 
% Therefore, we propose to solve \eqref{eqn:MAB_IPW_w_logged} by combining convex optimization with the cutting-plane method \cite{bertsimas1997introduction}. 
% Specifically, the cutting-plane method iteratively refines a finite set of constraints to approximate the infinite set of constraints through adding then one by one, until no constraint in the infinite set is violated. 
% We present the algorithm details in Appendix \ref{sec:optimization_MAB}. 

% % The underlying principle is to approximate the feasible region of a nonlinear (convex) program by a finite set of closed half spaces and to solve a sequence of approximating linear programs.

% \hl{[explain the allocation more clearly]}

% % We note that, with IPW as the value estimator, the objective does not change when we also utilize the logged dataset $\mD_0$ in the objective in addition to in the safety constraint. 
% % This is because the additive structure of IPW. 
% % This may not be the case when we consider other estimators. 
% % although it looks like we only utilize the side information (which typically comes from a ) in the safety constraint but not in the objective, 
% % and when we only utilize (?) it in the safety constraint




==> Safe Exploration for OPE [Camera-ready]/9_Method_Details.tex <==
\section{Additional Details of the Proposed Methods}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Safety constraint with side information}\label{sec:appendix_constraint}
In this section, we give a few examples on how to construct the high-probability confidence (or credible) region $\mathcal{C}_\delta(\mD_0)$ and show why it is convex in these cases. 
For any vector $\vv$ and matrix $V$, we denote $||\vv||_V = \vv^T V^{-1} \vv$. 
% Most of the derivations are standard and included for completeness. 

For MAB, we can construct a confidence region by using an $(1-\delta / K)$-confidence interval for each arm separately. 
For example, suppose the noise is sub-Gaussian and there is at least one data point for each arm. 
We have $\prob \big[ |\hat{r}_a - r_a| / \sigma_a \ge \sqrt{2/n_a log(2/\delta)} \big] \le \delta$, 
where $n_a$ and $\hat{r}_a$ are the count and sample mean for arm $a$, respectively. 
Therefore, 
\begin{align*}
    \mathcal{C}_\delta(\mD_0) = \{\vr: max(\hat{r}_a - \sigma_a\sqrt{2/n_a log(2K/\delta)}, 0) \le r_a \le min(\hat{r}_a + \sigma_a\sqrt{2/n_a log(2K/\delta)}, 1), \forall a \in [K] \} 
\end{align*}
is a valid confidence region, based on the Bonferroni correction. 
We remark that, other choice is also possible than splitting the $\delta$ equally over arms. 

Alternatively, we can consider the Bayesian perspective. 
We additionally assume the existence of a prior over $r_a$ as $\normal(\mu_{a,0}, \sigma_{a,0}^2)$ for every arm $a$ independently. 
By assuming that the reward from arm $a$ follows $\normal(0, \sigma^2_a)$, 
we can derive $r_a | \mD_0 \sim \normal \big(
\hat{r}'_a, \hat{\sigma}^2_a\big)$, where $\hat{\sigma}^2_a = (1/\sigma_{a,0}^2 + n_a /\sigma^2_a)^{-1}$ and $\hat{r}'_a = \hat{\sigma}^2_a(\mu_{a,0} / \sigma_{a,0}^2 + n_a\hat{r}_a/\sigma^2_a)$. 
Therefore, one valid credible region is 
\begin{align*}
    \mathcal{C}_\delta(\mD_0) = \{\vr: max(\hat{r}'_a - z_{\delta/2K} \hat{\sigma}_{a}, 0) \le r_a \le min(\hat{r}'_a + z_{\delta/2K}\hat{\sigma}_{a}, 1), \forall a \in [K] \}, 
\end{align*}
where we construct an interval for each arm separately. 
Alternatively, utilizing the fact that these Gaussian variables are independent, we can construct a joint region. 

Notably, all examples above give us a convex set. 
The high-probability region in the CMAB case can be similarly derived. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For linear bandits, based on $\mD_0$, with a given regularization parameter $\lambda$, we can construct a covariance matrix $\widehat{V}_0 = \sum_{(\vx_i, R_i) \in \mD_0} \vx_i \vx_i^T + \lambda \mathbf{I}$, an initial estimate $\hat{\vthe}_0 = \widehat{V}_0^-1 (\sum_{(\vx_i, R_i) \in \mD_0} \vx_i R_i)$, 
and a corresponding high-confidence region for $\vthe^*$ as $\mathcal{C}_\delta(\mD_0) = \{\vthe : ||\vthe - \hat{\vthe}_0||_{\widehat{V}_0} \le S_{\delta}\}$. 
By carefully choosing $S_{\delta}$ as given in Theorem 2 of \citet{abbasi2011improved}, we can guarantee that $\prob\big(\vthe^* \in \mathcal{C}_\delta(\mD_0)\big) \ge 1-\delta$. 
% with probability at least $1-\delta$. 
% where $\hat{\vthe}_0$ and $\widehat{V}_0$ are the (regularized) least square estimate and sample covariance matrix obtained in $\mD_0$. 

For the Bayesian perspective, we additionally assume the existence of a prior over $\vthe$ as 
$\normal\big(\vmu_{\vthe}, \Sigma_{\vthe}\big)$, which can be learned either from domain knowledge or via meta-learning \cite{kveton2021meta, wan2021metadata}. 
Assume that the noise follows $\normal(0, \sigma^2)$. 
The standard Bayesian results on Gaussian linear regression tell us that 
\begin{align*}
    \vthe | \mD_0 \sim \normal\Big( \widehat{\Sigma} \big(\Sigma_{\vthe}^{-1}\vmu_{\vthe}  + \sum_{(\vx_i, R_i) \in \mD_0} \vx_i R_i / \sigma^2 \big) , \widehat{\Sigma}  \Big), 
    \widehat{\Sigma} = \big(\Sigma_{\vthe}^{-1} + \sum_{(\vx_i, R_i) \in \mD_0} \vx_i \vx_i^T / \sigma^2 \big)^{-1}
\end{align*}
Let $\hat{\vthe} =  \widehat{\Sigma} \big(\Sigma_{\vthe}^{-1}\vmu_{\vthe}  + \sum_{(\vx_i, R_i) \in \mD_0} \vx_i R_i / \sigma^2 \big)$. 
We can then define  the ellipsoid as 
$\mathcal{C}_\delta(\mD_0) = \{\vthe : ||\vthe - \hat{\vthe}||_{\widehat{V}} \le \chi^2_{d}(1-\delta)\}$. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Connections with hypothesis testing}\label{sec:other_testing}
% under other settings
For linear bandits, the problem reduces to the random design analysis of linear models   \cite{hsu2011analysis}. 
We assume homoscedasticity, i.e., $\var(\epsilon_t) \equiv \sigma^2$. 
We focus on that $\mD_{0}$ is empty for simplicity, and it is straightforward to extend to the case with $\mD_{0}$. 
By the central limit theorem and the Slutsky’s lemma, 
we can establish that 
\begin{align*}
    \sqrt{T}(\hat{\vbeta} - \vbeta) 
     &\overset{d}{\to} \normal\Big(\vzero,  
     \sigma^2
     \big(
     \sum_\vx \pi_e(\vx) \vx \vx^T
     \big)^{-1}
     \Big), 
     T \to \infty. 
\end{align*}
which implies 
\begin{align*}
    \sqrt{T}
    \Big[
    \big(\widehat{V}_{DM}(\pi_1; \mD) - \widehat{V}_{DM}(\pi_0; \mD) \big)
    - \big(V(\pi_1; \mD) - V(\pi_0; \mD) \big)
    \Big]
     &\overset{d}{\to} \normal\Big(\vzero, 
     \sigma^2 
    \bar{\vphi}^T_{\Delta \pi}  \big(\sum_\vx \pi_e(\vx) \vx \vx^T\big)^{-1} \bar{\vphi}_{\Delta \pi}
     \Big), 
     T \to \infty. 
\end{align*}
Therefore, by similar derivations as in the MAB case, we can design a valid testing procedure and identify that the testing power is determined by $\bar{\vphi}^T_{\Delta \pi} \big( \sum_\vx \pi_e(\vx) \vx \vx^T\big)^{-1} \bar{\vphi}_{\Delta \pi}$, i.e., our optimization objective. 

% Regarding the contextual version of MAB and linear bandits, 
Regarding CMAB with IPW, note the fact the the estimator, as in the MAB case, is also an U-statistic (i.e., the average of i.i.d samples). 
Therefore, we can similar derive its asymptotic distribution and relate the asymptotic variance (and hence the power) with our optimization objective. 
For example, 
let $\sigma(\pi_e) {=} \sqrt{\var(\pi_e(A_t|\vx_t)^{-1}\pi_{\Delta}(A_t|\vx_t)R_t)}$ and $\hat{\sigma}(\pi_e)$ be a consistent estimator (typically the plug-in estimator with sample variance). 
By the central-limit theorem and the Slutsky’s lemma, we again have  
\begin{align*}
\frac{\sqrt{T}}{\hat{\sigma}(\pi_e)}
    \Big[
    \big(\widehat{V}(\pi_1; \mD_{e}) 
    {-} \widehat{V}(\pi_0; \mD_{e}) \big)
    {-} \big(V(\pi_1) {-} V(\pi_0)\big)\Big]
    \overset{d}{\to} \normal(0, 1), 
\end{align*}
when $T$ grows.  %  \to \infty
The remaining discussions are exactly the same with the MAB case. 


\subsection{Optimization algorithm for MAB and CMAB with IPW}\label{sec:optimization_MAB}
As we mentioned in the main text, at the first glance, it is challenging to solve 
\eqref{eqn:MAB_IPW_w_logged} as it involves infinite number of linear constraints. 
Fortunately, both the objective and the feasible set are convex, and so we can adapt the cutting-plane method \cite{boyd2007localization} to solve. 


As an iterative algorithm, there are two main steps in the cutting-plane method. 
At every iteration, we need to 
(i) proposed a \textit{query point} $\pi_e^{(i)}$, and then 
(ii) check with an oracle on whether or not $\pi_e^{(i)}$ is in a target convex set (the feasible set in our case): 
if true, then we can terminate; otherwise, we find a plane to separate $\pi_e^{(i)}$ and the target convex set (i.e., the cutting plane). 



The choices of $\pi_e^{(i)}$ and the cutting plane are both central to the computational efficiency. 
Following  \cite{zhu2021safe}, we design the algorithm as in Algorithm \ref{alg:CP_MAB}, where both are obtained by a solving a simple subproblem. 
Specifically, the one for $\pi_e^{(i)}$ has a convex objective function and a set of linear constraints, and the one for $\vr^{(i)}$ is a linear programming problem. 
The optimization algorithm for the CMAB case can be designed similarly. 
The convergence analysis is provided in \citet{boyd2007localization}. 


\input{Alg/alg_CP_MAB}

% \begin{equation*}
%     \begin{split}
% \frac{\partial \mJ(\pi_e)}{\partial \pi_e(a|\vx)}
% &= 
% -p(\vx)\frac{\pi_{\Delta}^2(a|\vx)}{\pi_e^2(a|\vx)}
%     \end{split}
% \end{equation*}


\subsection{Optimization algorithm for linear bandits with DM}\label{sec:optimization_LB}
% Frank-Wolfe with a Cutting Plane Method
% FW algorithm for safe linear bandits exploration with the cutting-plane method
We first introduce how to solve for a finite set of constraints $\Theta$: 
\begin{equation*}
    \begin{split}
&\argmin_{\pi_e \in \Delta_{K-1}} \;
\mJ(\pi_e) = 
\bar{\vphi}^T_{\Delta \pi}
    % (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T
    % + \vPhi_0^{T}\vPhi_0)^{-1} (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T) 
    (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{+}
    \bar{\vphi}_{\Delta \pi}\\
% &s.t. \; \min_{\vthe \in \mathcal{C}_\delta(\mD_0)} \big(\pi_e - (1-\epsilon) \pi_0 \big) \mX \vthe \ge  0, 
&s.t. \; \max_{\vthe \in \Theta} \big((1-\epsilon) \pi_0 - \pi_e\big)^T \mX \vthe \le  0. 
    \end{split}
\end{equation*}
We propose to adapt the Frank–Wolfe (FW) algorithm \citep{frank1956algorithm}, which is a projection-free algorithm for convex optimization and it enjoys nice convergence property  \citep{frank1956algorithm, lattimore2020bandit, jaggi2013revisiting}. 
We summarize in Algorithm \ref{alg:FW}. 
% We next derive the key steps. 
For Step 1, we note that 
the partial derivative can be derived as
\begin{equation*}
    \begin{split}
\frac{\partial \mJ(\pi_e)}{\partial \pi_e(\vx_i)}
&= 
-T
\Big\{
\bar{\vphi}^T_{\Delta \pi}
(T\vG(\pi_e) + \vG_0)^{-1} \vx_i \Big\}^2
    \end{split}
\end{equation*}
where $\vG_0 = \vPhi_0^T \vPhi_0$ and $\vG(\pi_e) = \sum_\vx \pi_e(\vx) \vx \vx^T$. 
For Step 2, we notice that it is a linear programming problem. 

 
% \hl{TBD}
% In Algorithm \ref{alg:FW_CP}, 
% to find $\vthe \in C_\delta$ on which the constraint is maximally violated by the current policy $\pi^{(i)}$, we need to maximize a linear function on an ellipsoid. 
% Fortunately, the solution can be obtained explicitly \citep{zhu2021safe} as 





\input{Alg/main_alg_FW_CP}


Next, we integrate the cutting-plane method and the FW algorithm to solve the most challenging problem \eqref{eqn:nonstochastic linear bandit with side info}, where there exists a infinite number of constraints. 
Refer to Appendix \ref{sec:optimization_MAB} for an introduction to the cutting-plane method. 
We note that, since the cutting-plane method only requires a feasible query point in every iteration instead of running the whole FW algorithm every time, one can stop the FW after a few iterations. 
This does not affect the convergence over the whole algorithm. 
% in every inner iteration

In Algorithm \ref{alg:FW_CP}, a key step is to find a good cutting plane, or equivalently, $\vthe \in C_\delta$ on which the constraint is maximally violated by the current policy $\pi^{(i)}$.
Assume $\mathcal{C}_\delta(\mD_0) = \{\vthe : ||\vthe - \hat{\vthe}_0||_{\widehat{V}_0} \le S_{\delta}\}$ for some $\hat{\vthe}_0$ and $\widehat{V}_0$. 
Let $\vv_{\pi^{(i)}} = \Big[\big((1-\epsilon) \pi_0 - \pi^{(i)}\big)^T \mX \Big]^T$. 
We need to maximize a linear function on an ellipsoid. 
Fortunately, the solution can be obtained explicitly \citep{zhu2021safe} as 
\begin{align*}
\vthe^{(i)} = 
    \argmax_{\vthe \in \mathcal{C}_\delta(\mD_0)} 
\Big[
\big((1-\epsilon) \pi_0 - \pi^{(i)}\big)^T \mX 
\Big]
\vthe 
= 
\hat{\vthe}_0
+ 
\frac{\widehat{V}_0 \vv_{\pi^{(i)}}}{\sqrt{\vv_{\pi^{(i)}}^T \widehat{V}_0 \vv_{\pi^{(i)}} /  S_\delta}}.  
\end{align*}
% $\lambda = \sqrt{\pi_e^T \Sigma b / 2 \delta}$
% double check!
% Accordingly, 
% $\max_{\vthe \in \mathcal{C}_\delta(\mD_0)} 
% \Big[
% \big((1-\epsilon) \pi_0 - \pi^{(i)}\big)^T \mX 
% \Big]
% \vthe 
% = \vv_{\pi^{(i)}}^T \hat{\vthe}_0
% + \sqrt{S_{\delta} \vv_{\pi^{(i)}}^T
% \widehat{V}_0
% \vv_{\pi^{(i)}}}
% $ can be used to determine if all constraints have been satisfied. 

% \begin{align*}
% \vthe^{(i)} = 
%     \argmax_{\vthe \in \mathcal{C}_\delta(\mD_0)} 
% \Big[
% \big((1-\epsilon) \pi_0 - \pi^{(i)}\big)^T \mX 
% \Big]
% \vthe 
% = 
% \hat{\vthe}_0
% + 
% \frac{\widehat{V}_0 \vv_{\pi^{(i)}}}{\sqrt{2\vv_{\pi^{(i)}}^T \widehat{V}_0 \vv_{\pi^{(i)}} /  \delta}}, 
% \end{align*}


==> Safe Exploration for OPE [Camera-ready]/9_PI.tex <==
\subsection{Pseudo-inverse estimator for linear bandits and its contextual version}\label{sec:PI}
Under the linear generalization assumption, besides the DM estimator, we can also consider the Pseudo-Inverse (PI) estimator \cite{swaminathan2016off}. 
Instead of inferring $\vthe$, PI directly constructs a weighted average of the observed rewards as in IPW, but it also utilizes the linear structure. 
PI is particular useful when being applied to some structured problem such as slate recommendation  \cite{swaminathan2016off}. 
Let $\vG(\pi) = \sum_\vx \pi(\vx) \vx \vx^T$. 
We first note that 
\begin{align*}
    V(\pi; \mD) 
    = \bar{\vphi}^T_{\pi} \vthe
    = \bar{\vphi}^T_{\pi} \vG(\pi)^{-1}  \sum_{\vx} \pi(\vx) \vx (\vx^T\vthe)
\end{align*}
Motivated by this relationship, the PI estimator is constructed as 
\begin{align}
    \widehat{V}_{PI}(\pi; \mD) 
    = |\mD|^{-1} \sum_{(\vx_i, R_i) \in \mD} \bar{\vphi}^T_{\pi} \vG(\pi)^{-1} (R_i \vx_i)
    = |\mD|^{-1} \bar{\vphi}^T_{\pi} \vG(\pi)^{-1}  \sum_{(\vx_i, R_i) \in \mD}R_i \vx_i
    \label{eqn:PI_estimator}
\end{align}
Let $\vPhi$ be the feature matrix stacked over points in $\mD$. 
We first derive the finite-sample conditional variance $\var(\widehat{V}_{PI}(\pi_1; \mD) | \vPhi)$ as % conditional on $\vPhi$ 
\begin{align*}
    \var(\widehat{V}_{PI}(\pi_1; \mD) | \vPhi)
    = |\mD|^{-2}\sum_{(\vx_i, R_i) \in \mD} \Big[\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1}\vx_i \Big]^2  \var(R_i \mid \vx_i)
\end{align*}
For simplicity of notations, w.l.o.g.,  we assume the noise variance is $1$. 
By the law of total variance, we can obtain that
\begin{equation}
    \begin{split}
    &T \times \var(\widehat{V}_{PI}(\pi_1; \mD_e))\\
    &=T \times  \Mean_{\vPhi \sim \pi_e} \var(\widehat{V}_{PI}(\pi_1; \mD_e) | \vPhi)
    +T \times  \var_{\vPhi \sim \pi_e} \Mean(\widehat{V}_{PI}(\pi_1; \mD_e)|\vPhi)\\
    % \var(\widehat{V}_{PI}(\pi_1; \mD) | \vPhi)
    &= \Mean_{\vx_i \sim \pi_e}  \Big[\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1}\vx_i \Big]^2 
    + T \times \var_{\vPhi \sim \pi_e} \Big\{ T^{-1} \bar{\vphi}^T_{\pi} \vG(\pi)^{-1}  \vPhi^T \vPhi \vthe \Big\}\\
    &\to  \bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1} \vG(\pi_e) \vG(\pi_1)^{-1} \bar{\vphi}_{\pi_1}
    + \var_{\vx \sim \pi_e} \Big\{ \bar{\vphi}^T_{\pi} \vG(\pi)^{-1}  \vx \vx^T \vthe \Big\}.  
    % + \var_{\mPhi} \Big\{\sum_{(\vx_i, R_i) \in \mD} \Big[\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1}\vx_i \Big]^2  \var(R_i \mid \vx_i)\Big\}
    \end{split}
\label{eqn:raw_PI}
\end{equation}
The proof for the asymptotic variance statement (i.e., the last row) is by similar arguments as in Appendix \ref{sec:proof_LB}. 


% Therefore, by replacing $\var(R_i \mid \vx_i)$ with the uniform upper bound, 
By similar arguments as in the IPW for MAB case, 
the raw objective \eqref{eqn:raw_PI} is infeasible to solve, as it involves the unknown parameter $\vthe$. 
Therefore, we relax with the upper bound of the unknown parameters and focus on minimizing  the \textit{intrinsic uncertainty} term from the reward noise, i.e., 
$\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1} \vG(\pi_e) \vG(\pi_1)^{-1} \bar{\vphi}_{\pi_1}$. 
Notice that, under the linear generalization assumption, all discussions in Section \ref{sec:Nonstochastic linear bandits} regarding the safety constraint still apply here. 
Therefore, this problem can be similarly solved as in Section \ref{sec:Nonstochastic linear bandits}, via combining the cutting-plane method with the FW algorithm. 

% by considering the corresponding continuous relaxation
% we can form the objective as 
% \begin{align*}
% \argmin_{\vPhi \sim \pi_e} 
%  \Big[\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1} \vPhi^T \Big] \Big[\bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1} \vPhi^T \Big]^T
%  = 
%  \bar{\vphi}^T_{\pi_1} \vG(\pi_1)^{-1} \vPhi^T \vPhi \vG(\pi_1)^{-1} \bar{\vphi}_{\pi_1}. 
% \end{align*}

Besides, 
by noting that \eqref{eqn:PI_estimator} is linear in $\bar{\vphi}^T_{\pi} \vG(\pi)^{-1}$, it is straightforward to extend to studying the value difference $V(\pi_1) - V(\pi_0)$. 
Moreover, as in \citet{swaminathan2016off} and \citet{zhu2021safe}, the PI estimator and the discussions above can be extended to the contextual setup in a straightforward manner. 
% In this section, every time point, we will



% \todorw{Discussion here.}
% However, it seems non-trivial to extend this approach to the value difference $\var(\widehat{V}_{PI}(\pi_1; \mD) - \widehat{V}_{PI}(\pi_0; \mD) | \vPhi)$ due to the $\vG(\pi)^{-1}$ term. 
% , i.e., how to analyze the value difference



% DM first estimate $\vthe^*$ via least-square regression, as $\hat{\vthe} = (\sum_i \vx_i \vx_i^T)^+ (\sum_i \vx_i R_i)$.
% Next, DM  plugs-in $\hat{\vthe}$ in the value definition to construct  
% We may sometimes write this estimator as $\widehat{V}(\pi; \mD)$ to emphasize its dependency on $\mD$. 
% \todob{A good paper on IPS in linear models is "Off-Policy Evaluation for Slate Recommendation". Given what we did before, this seems more natural than the direct method.}
% $\overline{\vphi}$


==> Safe Exploration for OPE [Camera-ready]/9_Proof.tex <==
\section{Proofs}\label{sec:proofs}

\subsection{Proof of Lemma \ref{lemma:ipw_explicit_form}}
\begin{proof}
First, recall that 
\begin{align*}
T \times \nu(\pi_e; \vr, \{\sigma_a\})    
&=  T \times \var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)\\
&= \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- \Big(V(\pi_1) - V(\pi_0)\Big)^2. 
\end{align*}

Let $W = \sum_a |\pi_{\Delta}(a)|$. 
We have $\pi_e^*(a) = |\pi_{\Delta}(a)| / W$. 
Therefore
\begin{equation*}
    \begin{split}
        &T \times \nu(\pi_e^*; \vr, \{\sigma_a\})\\
&= \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{|\pi_{\Delta}(a)| / W} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{|\pi_{\Delta}(a)| / W} r^2_a
- c\\
&= \sum_{a \in [K]} |\pi_{\Delta}(a)|W (\sigma^2_a + r^2_a)
- \Big(V(\pi_1) - V(\pi_0)\Big)^2, 
    \end{split}
\end{equation*}
which implies
\begin{align*}
\nu(\pi_e^*; \vr, \{\sigma_a\})
=  
\frac{1}{T} \Big[
\sum_a |\pi_{\Delta}(a)| \times
\sum_{a \in [K]} |\pi_{\Delta}(a)| (\sigma^2_a + r^2_a)
- \big(V(\pi_1) - V(\pi_0)\big)^2
\Big]
\end{align*}

\end{proof}


\input{9_proof_MAB}

\input{9_proof_LB}
\input{9_counter_eg}



\subsection{Convexity of the objectives and constraints}\label{sec:convexity}
For the sake of completeness, we show in this section that the objectives and constraints considered in this paper are all convex. 
Regarding the objective of IPW, we note the relationship that 
\begin{align*}
     \alpha\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)}
    + (1-\alpha) \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi'_e(a)}
    \ge  \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\alpha \pi_e(a) + (1-\alpha)\pi'_e(a)}, 
\end{align*}
due to the inequality
\begin{align*}
     \alpha \frac{1}{\pi_e(a)}
    + (1-\alpha)  \frac{1}{\pi'_e(a)}
    \ge   \frac{1}{\alpha \pi_e(a) + (1-\alpha)\pi'_e(a)}, \forall a \in [K], 
\end{align*}
which stems from the convexity of $f(x) = 1/x$. 
The same arguments hold for CMAB with IPW. 

Regarding the objective of linear bandits with DM, 
\begin{align*}
\bar{\vphi}^T_{\Delta \pi}
    (T\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}, 
\end{align*}
we notice that $\sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T$  is linear in $\pi_e$ and the matrix inverse operator is a convex function. 
Therefore, their composition is still convex.

Regarding the constraint, notice that, for every single instance, the constraint is a linear one and hence convex. 
The overall feasible set is the intersection of these convex sets, and hence is convex. 



% \begin{equation}
%     \begin{split}
%     % \Delta_{K - 1}
%         &\argmin_{\pi_e  \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\
%         % \var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
%         &s.t. \;\; \pi_e(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]. 
%         % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
%     \end{split}
%     \label{eqn:MAB_IPW_no_logged}
% \end{equation}


% \subsection{Some other derivations for MAB with IPW}
% As we mentioned, since the objective $\var\big(\widehat{V}(\pi_1; \mD_0 \cup \mD_e) - \widehat{V}(\pi_0; \mD_0 \cup \mD_e)\big)$ is related with some unknown parameters (to be learned), 
% it is impossible to guarantee that one exploration policy can always dominate another. 

% When $|\pi_{\Delta}(a)|-K|\pi_{\Delta}(a)|\big)| < 0$ (i.e., the two policies differ more than average), the value of $|\pi_{\Delta}(a)|$ is higher than that when $|\pi_{\Delta}(a)|-K|\pi_{\Delta}(a)|\big)| \ge 0$. 
% Therefore, in the extreme case where $\sigma^2_a \equiv = \sigma$ and $r^2_a \equiv r$, 
% it is clear that our policy is more efficient. 
% Apparently this setup is too restrictive, but it provides insights (\hl{why? what?})

% % Although this is again a Bayesian statement? 
% % And why not incorporate as side information? 
% % Find as we do not assume any specific form of this distribution?

% How about the case with side information? Things will be different. 
% And safety constraint?

% With $V(\pi_1)$ as the objective, it is easier to talk about why it would be more efficient?

% \begin{align*}
%     \sum_{a \in [K]}
%  \Big[
%  \big(1-K\pi_1(a)\big)\pi_1(a) \big(\sigma^2_a + r^2_a\big)
%  \Big]
% \end{align*}

% positive correlation between $\pi_1(a)$ and $r_a$. 



% \textbf{Linear bandits.}
% \begin{align}
% \var \Big(\widehat{V}(\pi_1; \mD_{\vPhi}) - \widehat{V}(\pi_0; \mD_{\vPhi}) \mid \vPhi \Big)
% = \bar{\vphi}^T_{\Delta \pi}
%      (\vPhi^T\vPhi)^{-1}
%     \bar{\vphi}_{\Delta \pi}. 
% \end{align}
 
% We replace it by 
% $\Big[\bar{\vphi}^T_{\Delta \pi}
%      (\Mean_{\vPhi \sim \pi_e}\vPhi^T\vPhi)^{-1}
%     \bar{\vphi}_{\Delta \pi}
%  \Big]$

% By assuming P.S.D., we know 
% $(\Mean_{\vPhi \sim \pi_e}\vPhi^T\vPhi)^{-} \preceq  \Mean_{\vPhi \sim \pi_e}(\vPhi^T\vPhi)^{-}$: wrong direction!



==> Safe Exploration for OPE [Camera-ready]/9_counter_eg.tex <==
\subsection{Counter-example}\label{sec:Counter-example}
In this section, we argue that there does not exist a policy $\pi_e$ that dominates all other policies across all problem instances, when we use the IPW estimator. 

Suppose $\pi_1 \neq \pi_0$. 
For any policy $\pi_e$, we can always construct an instance $(\vr, \{\sigma_a\})$ and a policy $b'$, such that \begin{align*}
    \nu(\pi_e; \vr, \{\sigma_a\}) >  \nu(\pi_e'; \vr, \{\sigma_a\}). 
\end{align*}

To see this, note that 
\begin{align*}
    T \times \Big[ \nu(\pi_e; \vr, \{\sigma_a\}) -  \nu(\pi_e'; \vr, \{\sigma_a\}) \Big]
= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b'(a)} \sigma^2_a 
- \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b'(a)} r^2_a. 
\end{align*}
By setting $r_a \equiv 0$, we get 
\begin{align*}
    T \times \Big[ \nu(\pi_e; \vr, \{\sigma_a\}) -  \nu(\pi_e'; \vr, \{\sigma_a\}) \Big]
= 
\sum_{a \in [K]} 
\big(
\frac{1}{\pi_e(a)}
- \frac{1}{b'(a)}
\big)
\pi^2_{\Delta}(a) \sigma^2_a. 
\end{align*}
Since $\pi_1 \neq \pi_0$, there are at least two arms $a'$ and $a''$ where the two policies differ. 
By design, we know $\pi_e(a')$ and $\pi_e(a'')$ are both positive. 
A counter-example can hence be designed by setting $\sigma_a' = 0$, $\sigma_{a''} = 1$, $b'(a') = 0.5\pi_e(a')$,  $b'(a'') = 0.5\pi_e(a') + \pi_e(a'')$ and keeping $\pi_e(a) = b'(a)$ on the other arms. 
In other words, we move more budgets to the arm of high variance. 
More precisely, we have 
\begin{align*}
&T \times \Big[ \nu(\pi_e; \vr, \{\sigma_a\}) -  \nu(\pi_e'; \vr, \{\sigma_a\}) \Big]\\
&= 
0 + 
\big(
\frac{1}{\pi_e(a')}
- \frac{1}{b'(a')}
\big)
\pi^2_{\Delta}(a') \sigma^2_{a'}
+ 
\big(
\frac{1}{\pi_e(a'')}
- \frac{1}{b'(a'')}
\big)
\pi^2_{\Delta}(a'') \sigma^2_{a''}\\
&= 
\big(
\frac{1}{\pi_e(a'')}
- \frac{1}{0.5\pi_e(a') + \pi_e(a'')}
\big)
\pi^2_{\Delta}(a'') \sigma^2_{a''}\\
&> 0. 
\end{align*}





==> Safe Exploration for OPE [Camera-ready]/9_expt.tex <==
\section{Additional Experiment Details and Results}\label{sec:appendix_expt}


\subsection{Additional experiment details}\label{sec:more_expt_details}
In this section, we introduce more details of the experiment setup used in our simulation study. 
The configuration for CMAB is almost the same with that for MAB introduced in the main text, except for that we generate for every context independently. 
For linear bandits, we following \citet{kazerouni2016conservative} to make sure $\vx_i^T \vthe^*$ is positive for all arms when sampling the feature vectors. 
To generate the policies $\pi_0$ and $\pi_1$, we follow a similar design with MAB, except for that we first sample $\Tilde{\vthe}$  from the multivariate normal and then generate $\pi_1(a)$ (or $\pi_0(a)$) proportional to $\vx_a^T \Tilde{\vthe}$. 


% logged dataset
% prior


% \hl{TODO}

% When sampling a policy, we first sample $\Tilde{\vthe} \sim \text{Dirichlet}(\vone_d)$, and then derive the distribution proportional to $\boldsymbol{X}\Tilde{\vthe}$. 

\subsection{Additional simulation experiments}\label{sec:more_expt}
In this section, we repeat the simulation experiments in the main text under a variety of parameter combinations to study the robustness of our findings. 
See Figure \ref{fig:more_CMAB} for results on CMAB and 
Figure \ref{fig:more_LB} for results on LB. 
Overall, the main findings are consistent with those in the main text.

\input{Fig/more_settings}

\subsection{Experiments on the MNIST dataset}\label{sec:MNIST}
In this section, we conduct two experiments on the MNIST dataset \cite{deng2012mnist}. 
In this dataset, every arm is an  (vectorized) image of a digit between $0$ and $9$, 
% This experiment is a more realist variant of that in Figure 2, where the actions A and the safety ellipsoid Θ are estimated from a real-world dataset

\textbf{CMAB.}
The first experiment focuses on contextual bandits. 
As standard in the literature \cite{dudik2014doubly}, 
we adapt a classification task to a CMAB problem. 
Specifically, in every trail, we randomly pick $100$ images as our contexts, with their probability sampled from  $\text{Dirichlet}(\vone_{100})$. 
The $K = 10$ arms correspond to the $10$ digits, and only the arm corresponding to the one on the image returns reward $1$. 
All the other arms return reward $0$. 
The two policies $\pi_0$ and $\pi_1$ are two classifier trained with $1000$ randomly sampled data points, 
one using the decision tree and the other using multi-class logistic regression. 
We define the one with higher accuracy as $\pi_1$ when $H_1$ is true, and as $\pi_0$ when $H_0$ is true. 
We aim to collect $T = 1000$ data points. 

This setup aims to mimic a common application: we have two policies trained using logged data and with different functional form assumptions, so a direct comparison is unfair and may suffer from model misspecification. 
% (note that we are considering bandit feedbacks and hence we can not easily do cross-validations). 
Therefore, one typically utilizes IPW (which is guaranteed to be unbiased under minimal assumptions) to compare these two policies. 

% delta = 0.05
% n_additional_data = 100


\textbf{Linear bandits.}
In the second experiment, we closely follow \citet{zhu2021safe} to study the performance on linear bandits. 
In every trail, we randomly pick one digit as the correct answer, and 
we assign reward $1$ to the images corresponding to this correct digit. 
$K = 100$ arms are randomly chosen. 
We set $\sigma = 1$, $|\mD_0| = 100$ and $T = 100$. 
$\vthe^*$ is fitted from the whole dataset. 
% How to generate the policies?

\textbf{Results.}
Results aggregated over $2000$ random seeds are presented in Figure \ref{fig:real}. 
The superior performance of \name{SEPEC} and other findings are largely consistent with our simulation experiments. 
In particularly, for linear bandits, the cost of satisfying the safety constraint is negligible, which is consistent with the findings in \citet{zhu2021safe}. 
Besides, regarding the power under linear bandits, we observe that  \name{SEPEC} is even slightly better than its non-safe version, though the difference is not statistically  significant. 
A closer look into the intermediate results tell that this is mainly due to that the FW is an iterative algorithm and the convergence situation might slightly vary due to numerical reasons. 
% (i) the difference between the finite-sample performance


% \input{Fig/real_data_results}


==> Safe Exploration for OPE [Camera-ready]/9_proof_LB.tex <==
\subsection{Proof of Theorem \ref{thm:LB}}\label{sec:proof_LB}
\begin{proof}
Denote $\vG(\pi_e) = \sum_{\vx \in \mathcal{A}} \pi_e(\vx) \vx \vx^T. $
We first note that 
\begin{align*}
T \times    \nu\pi_e;\mD_0) 
    = T \times \bar{\vphi}^T_{\Delta \pi}
% (T\vG(\pi_e)
% + \vPhi_0^{T}\vPhi_0)^{-1} (T\vG(\pi_e)) 
(T\vG(\pi_e)+ \vPhi_0^{T}\vPhi_0)^{-1}
\bar{\vphi}_{\Delta \pi}
    = \bar{\vphi}^T_{\Delta \pi}
% (T\vG(\pi_e)
% + \vPhi_0^{T}\vPhi_0)^{-1} (T\vG(\pi_e)) 
(\vG(\pi_e)+ T^{-1}\vPhi_0^{T}\vPhi_0)^{-1}
\bar{\vphi}_{\Delta \pi}
\to \bar{\vphi}^T_{\Delta \pi}\vG(\pi_e)^{-1}\bar{\vphi}_{\Delta \pi}, 
\end{align*}
when $T$  goes to infinity. %$T \to \infty$. 
Besides, we note the following relationship
\begin{align*}
    T \times \nu^*(\pi_e; \mD_0) 
    &= T \times \var_{\vPhi \sim \pi_e} \Big(\widehat{V}_{DM}(\pi_1; \mD_{\vPhi} \cup \mD_0) - \widehat{V}_{DM}(\pi_0; \mD_{\vPhi} \cup \mD_0) \Big)\\
    &=  \Mean_{\vPhi \sim \pi_e}\Big[\bar{\vphi}^T_{\Delta \pi}
     (T^{-1}\vPhi^T\vPhi+ T^{-1}\vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}
 \Big].
\end{align*}

Since the rows of $\vPhi$ are \textit{i.i.d.}, 
 by the strong law of large numbers, 
we know $T^{-1}\vPhi^T\vPhi \overset{a.s.}{\to} \vG(\pi_e)$, 
and hence $T^{-1}\vPhi^T\vPhi + T^{-1}\vPhi_0^{T}\vPhi_0 \overset{a.s.}{\to} \vG(\pi_e)$. 
Therefore, by the continuous mapping theorem, we have $(T^{-1}\vPhi^T\vPhi + T^{-1}\vPhi_0^{T}\vPhi_0)^{-1} \overset{a.s.}{\to} \vG(\pi_e)^{-1}$ and also 
$\bar{\vphi}^T_{\Delta \pi} \big[T^{-1}\vPhi^T\vPhi + T^{-1}\vPhi_0^{T}\vPhi_0\big]^{-1} \bar{\vphi}_{\Delta \pi}
\overset{a.s.}{\to} \bar{\vphi}^T_{\Delta \pi}\vG(\pi_e)^{-1}\bar{\vphi}_{\Delta \pi}$. 
Finally, from the random matrix theory for the tail bounds on the eignevalues of random matrix with $i.i.d.$ rows  \cite{vershynin2010introduction}, we know the uniformly integrable condition can be satisfied and hence we conclude with 
\begin{align*}
    \Mean_{\vPhi \sim \pi_e} \Big[
    \bar{\vphi}^T_{\Delta \pi} \big[T^{-1}\vPhi^T\vPhi + T^{-1}\vPhi_0^{T}\vPhi_0\big]^{-1} \bar{\vphi}_{\Delta \pi}
    \Big] \to \bar{\vphi}^T_{\Delta \pi}\vG(\pi_e)^{-1}\bar{\vphi}_{\Delta \pi}
\end{align*}


% The above is for a fixed $\pi_e$. We need to show uniform. 


% and hence $\bar{\vphi}^T_{\Delta \pi}(T^{-1}\vPhi^T\vPhi)^{-1}\bar{\vphi}_{\Delta \pi} \overset{p}{\to} \bar{\vphi}^T_{\Delta \pi}\vG(\pi_e)^{-1}\bar{\vphi}_{\Delta \pi} $


% %  (Only when $p = o(T)$, it converge in probability? We can just consider a fixed $p$). 

% \hl{need $\pi_e$ such that G(\pi_e) is invertible?}

\end{proof}


==> Safe Exploration for OPE [Camera-ready]/9_proof_MAB.tex <==
\subsection{Proof of Theorem \ref{thm:mab}}
\begin{proof}
First, recall that 
\begin{align*}
T \times \nu(\pi_e; \vr, \{\sigma_a\})    
= T \times \var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \Big)
= \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- c, 
\end{align*}
where $c = \Big(V(\pi_1) - V(\pi_0) \Big)^2$ is independent with $\pi_e$. 


Denote $\Mean_Q(r^2_a) \equiv r^2_Q$ and $\Mean_Q(\sigma^2(a)) \equiv \sigma^2_Q$. 
Therefore, 
for any $\pi_e \in \Pi$, 
we have 
\begin{align*}
&T \times \Mean_{Q} \Big[ \nu(\pi_e^*; \vr, \{\sigma_a\}) - \nu(\pi_e; \vr, \{\sigma_a\})   \Big]\\
&= \Mean_{Q} \Big[ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e^*(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e^*(a)} r^2_a
- \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
- \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
\Big]\\
&= 
\Big[ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e^*(a)}
- \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)}
\Big] \times \big(\sigma^2_a + r^2_a\big)\\
&\le 0, 
\end{align*}
where the last inequality is due to that, by design, $\pi_e^*$ is the minimizer of $\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)}$ within the class of safe policies. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Minimax %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

To prove the minimax optimality, we first show that, for any policy $\pi_e$, 
$\max_{(\vr, {\sigma_a})  \in \mathcal{I}} \nu(\pi_e; \vr, {\sigma_a})$ is achieved when $\vr = \vone$ and $\sigma_a \equiv \sigma$. 
To see this, we exam
\begin{align*}
&T \times \nu(\pi_e; \vr, \{\sigma_a\}) - T \times \nu(\pi_e; \vone, \{\sigma, \dots, \sigma\}) \\
&=\Big[
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2_a 
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} r^2_a
- (V(\pi_1) - V(\pi_0))^2
\Big]\\
&\quad-
\Big[
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \sigma^2
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} 1^2
- 0^2
\Big]\\
&=\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} (\sigma^2_a - \sigma^2)
+ \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} (r^2_a-1)
- (V(\pi_1) - V(\pi_0))^2\\
&\le 0.  
\end{align*}

Therefore, we have 
\begin{align*}
T \times \max_{(\vr, {\sigma_a})  \in \mathcal{I}} \nu(\pi_e; \vr, {\sigma_a})
= \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} (\sigma^2 + 1)
\end{align*}
Notice that $\pi_e^*$, by design, is the minimizer of this objective. 
Therefore, we have that $\pi_e^*$ is minimax optimal, i.e., 
$ \max_{(\vr, {\sigma_a}) \in \mathcal{I}}  \nu(\pi_e^*; \vr, {\sigma_a}) = \min_{\pi_e \in \Pi}  \max_{(\vr, {\sigma_a})  \in \mathcal{I}} \nu(\pi_e; \vr, {\sigma_a})$. 
% \begin{align*}
%     max_{(\vr, {\sigma_a}) \in \mathcal{I}_c}  \nu(\pi_e^*; \vr, {\sigma_a}) = \min_{b \in \Pi}  max_{(\vr, {\sigma_a})  \in \mathcal{I}_c} \nu(\pi_e; \vr, {\sigma_a}). 
% \end{align*}



% \hl{TODO}
% Alternatively, we can also compare the worst-case. 
% Note that 
% $c = (V(\pi_1) - V(\pi_0))^2 = [\sum_a \pi_{\Delta}(a) r_a]^2$. 

% \begin{align*}
% \max_{\{r_a\}, \{\sigma_a\}}
% \sum_a |\pi_{\Delta}(a)| \times
% \sum_{a \in [K]} |\pi_{\Delta}(a)| (\sigma^2_a + r^2_a)
% - [\sum_a \pi_{\Delta}(a) r_a]^2
% \end{align*}

% \begin{align*}
% \sum_{a \in [K]} K\pi^2_{\Delta}(a) (\sigma^2_a + r^2_a)
% - [\sum_a \pi_{\Delta}(a) r_a]^2. 
% \end{align*}



% \textbf{can not achieve minimax optimality because the upper bound is not tight.
% To achieve that, we need to find the worst case for any fixed $\pi_e$ w.r.t. \eqref{eqn:0_MAB_objective_1} and then optimize over $\pi_e$. TBD. These complexity come from "sampling from b". 
% }
% Therefore, for any policy $\pi_e$, we have 
% \begin{align*}
% max_{(\vr, {\sigma_a}) \in \mathcal{I}_c}  \nu(\pi_e; \vr, {\sigma_a})
% = 
% \end{align*}




\end{proof}


==> Safe Exploration for OPE [Camera-ready]/9_stochastic_contextual_LB.tex <==
\subsection{Stochastic contextual linear bandits}\label{sec:contextual_LB}
Next, we consider the contextual bandits setting with a linear generalization function, i.e., the stochastic contextual linear bandits problem. 
At every round $t$, a stochastic context $\vx_t$ will be sampled i.i.d. and can not be known \textit{a priori}.  
The agent will then choose an arm $A_t$, which together with $\vx_t$ gives us the transformed feature vector $\vphi_t = \vphi_{\vx_t, A_t}$. 
Let $\bar{\vphi}_{\pi} = \Mean_{\vx \sim p(\vx), a \sim \pi(a \mid \vx) }   \vphi_{\vx,a}$. 
Assume $p(\vx)$ is known and hence $\bar{\vphi}_{\pi}$ is also known. 
Given an estimate $\hat{\vthe}$ obtained via least-square regression, 
recall our value estimator via DM is $\widehat{V}_{\hat{\vthe}}(\pi) = \Mean_{\vx \sim p(\vx), a \sim \pi(a \mid \vx)} \vphi^T_{\vx,a}  \hat{\vthe}  
= \big[ \Mean_{\vx \sim p(\vx), a \sim \pi(a \mid \vx)} \vphi^T_{\vx,a}\big]  \hat{\vthe} 
= \bar{\vphi}^T_{\pi} \hat{\vthe}$. 
Let $\bar{\vphi}_{\Delta\pi} = \bar{\vphi}_{\pi_1} - \bar{\vphi}_{\pi_0}$. 
W.l.o.g.,  we assume the noise variance is upper bounded by $1$. 
Without other information or constraints, 
by similar arguments as in Section \ref{sec:Nonstochastic linear bandits}, 
our objective can be transformed as follows
\begin{equation}
    \begin{split}
    &\var(\widehat{V}(\pi_1; \mD_{e} \cup \mD_{0}) - \widehat{V}(\pi_0; \mD_{e} \cup \mD_{0})) \\
    &= \bar{\vphi}^T_{\Delta\pi} cov(\hat{\vthe})  \bar{\vphi}_{\Delta\pi}\\
    &= 
    \bar{\vphi}^T_{\Delta\pi}
    \Big\{
    \Mean_{\vPhi \sim \pi_e, \vx} \Big[ cov(\hat{\vthe} \mid \vPhi) \Big]
    + cov_{\vPhi \sim \pi_e, \vx} \Big[ \Mean(\hat{\vthe} \mid \vPhi) \Big]
    \Big\}
    \bar{\vphi}_{\Delta\pi}\\
    &= 
    \bar{\vphi}^T_{\Delta\pi}
    \Big\{
\Mean_{\vPhi \sim \pi_e, \vx} \Big[ (\vPhi^T\vPhi + \vPhi_0^T\vPhi_0)^{-1}\Big]\Big\}
    \bar{\vphi}_{\Delta\pi}\\
    % cov(\hat{\vthe} \mid \mD_0)
    % &= \Mean_{\vPhi} \Big[ cov(\hat{\vthe} \mid \vPhi, \mD_0) \Big]
    % + cov_{\vPhi} \Big[ \Mean(\hat{\vthe} \mid \vPhi, \mD_0) \Big]\\
    % % &= \Mean_{\vPhi} \Big[\sigma^2 (\vPhi_0\vPhi)^{-1} \Big]
    % % + cov_{\vPhi} \Big[ \Mean(\hat{\vthe} \mid \vPhi) \Big]
    % &= \Mean_{\vPhi} \Big[\sigma^2 (\vPhi^T\vPhi + \vPhi_0^{T}\vPhi_0)^{-1} (\vPhi^T\vPhi) (\vPhi^T\vPhi + \vPhi^{_0T}\vPhi_0)^{-1}\Big]\\
    % &\quad + cov_{\vPhi} \Big[  (\vPhi^T\vPhi + \vPhi_0^{T}\vPhi_0)^{-1} (\vPhi_0^{T} \vR_0 +  \vPhi^T\vPhi\vthe) \Big]
    \end{split}
\end{equation}
Here, $\vPhi$ and $\vPhi_0$ is the feature matrix stacked over points in $\mD$ and $\mD_0$, respectively. 
More specifically, $\vPhi = (\vphi_{\vx_1, A_1}, \dots, \vphi_{\vx_T, A_T})^T$. 
We use $\vPhi \sim \pi_e, \vx$ to emphasize the expectation is taken over $\vPhi$, which depends on both the policy $\pi_e$ and the  stochastic context $\vx$. 



% \label{sec:Nonstochastic linear bandits}

% The logged dataset $\mD_0$ may make some directions less (marginally) informative. 
Besides, the safety constraint also needs to be satisfied. 
Therefore, our problem can be written as 
\begin{equation}
    \begin{split}
    &\argmin_{\pi_e}
    \bar{\vphi}^T_{\Delta\pi}
    \Big\{
\Mean_{\vPhi \sim \pi_e, \vx} \Big[ (\vPhi^T\vPhi + \vPhi_0^T\vPhi_0)^{-1}\Big]\Big\}
    \bar{\vphi}_{\Delta\pi}\\
    % &s.t. \;  \min_{\vthe \in \mathcal{C}_\delta(\mD_0)} \quad 
    % \Big\{
    % \Mean_{\vPhi \sim \pi_e, \vx} \big(\vone^T \vPhi\vthe\big)  
    % - (1-\epsilon) 
    %  \Mean_{\vPhi \sim \pi_0} \big(\vone^T \vPhi\vthe\big) \Big\}
    % \ge 0\\
    % The next is stronger and eaiser to solve?
    &s.t. \; 
    \big[
    \bar{\vphi}_{\pi_e^*}^T - (1-\epsilon) \bar{\vphi}_{\pi_0}^T
    \big]\vthe
    \ge 0, \forall \vthe \in \mathcal{C}_\delta(\mD_0), \\
    &\quad \; 
    \pi_e(\cdot \mid \vx) \in \Delta_{K - 1}, \forall \vx \in \mathcal{X}
    \end{split}
\end{equation}
The challenges on optimization include that (i) both the objective and $\bar{\vphi}_{\pi_e}$ in the constraint can have complex dependency on $\pi_e$, 
(ii) the constraint implicitly includes infinite linear constraints, 
and (iii) the stochasticity in the context is hard to handle, unlike in Section \ref{sec:Nonstochastic linear bandits}. 

When there is a finite number of contexts, 
following similar arguments as in Section \ref{sec:Nonstochastic linear bandits}, 
we can consider the following surrogate objective instead, which can be similarly proved as the asymptotic variance of our procedure: 
\begin{equation}
    \begin{split}
            &\argmin_{\pi_e} 
    \bar{\vphi}^T_{\Delta\pi}
    \Big\{ 
    \Big[ (
    T \sum_{\vx, a} p(\vx) \pi_e(a | \vx) \vphi_{\vx, a} \vphi^T_{\vx, a}
     + \vPhi_0^T\vPhi_0)^{-1}\Big]\Big\}
    \bar{\vphi}_{\Delta\pi}\\
    &s.t. \; \min_{\vthe \in \mathcal{C}_\delta(\mD_0)} \quad 
    \big[
    %\bar{\vphi}_{\pi_e^*} 
    \sum_{\vx, a} p(\vx) \pi_e(a | \vx) \vphi_{\vx, a}
    - (1-\epsilon) \bar{\vphi}_{\pi_0}
    \big]^T\vthe
    \ge 0. 
    %,\\
    % &\quad \; 
    % \pi_e(\cdot \mid \vx) \in \Delta_{K - 1}, \forall \vx \in \mathcal{X}. 
%   &\begin{aligned}
%   \end{aligned}\\
    \end{split}
\end{equation}
The problem can be solved similarly as in \eqref{eqn:nonstochastic linear bandit with side info} by utilizing the convexity. 
See Appendix  \ref{sec:optimization_LB} for details. 




% Besides, if we need a fixed exploration policy, things might become more complicated when we consider the stochastic context setup (i.o. a fixed set of arms).
% Q: why it has nothing to do with the policy forms?


% $\prob{(\widehat{V}(\pi_1) - \widehat{V}(\pi_0)) (V(\pi_1) - V(\pi_0)) > 0}$


% Functional form
% Various Objectives
% Heteroscedasticity




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






% Suppose we choose an arm $\vx_t$ in each round from a \textit{fixed} and \textit{finite} set of arms $\mA_t$. 
% Let $\bar{\vx}^T_{\pi_1} = \Mean_{\vx_t \sim \pi_1} \vx_t$. 
% We assume $r(\vx_t) = \vx_t \vthe^*$ and consider the DM value estimator $V(\pi) = \sum_{\vx} \pi(\vx) (\vx \hat{\vthe}) = 
% (\sum_{\vx} \pi(\vx) \vx) \hat{\vthe} = \bar{\vphi}^T_{\pi} \hat{\vthe}$, where $\bar{\vphi}_{\pi} = \sum_{\vx} \pi(\vx) \vx$. 
% $\overline{\vphi}$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \textbf{Optimization for Problem \ref{eqn:linear bandit with side info}.} 
% We first note that this is still a convex problem. 
% The derivative can be shown to be 
% \begin{equation}
%     \begin{split}
% \frac{\partial \mJ(\pi_e)}{\partial \pi_e(\vx_i)}
% &= 
% T  
% \bar{\vphi}^T_{\Delta \pi}
% \Big\{
% - (TG(\pi_e) + G_0)^{-1} (\vx_i \vx_i^T) (TG(\pi_e) + G_0)^{-1}\\
% &\quad + 2 (TG(\pi_e) + G_0)^{-1} (\vx_i \vx_i^T) (TG(\pi_e) + G_0)^{-1} G_0 (TG(\pi_e) + G_0)^{-1}
% \Big\}
% \bar{\vphi}_{\Delta \pi}\\
% &= 
% T  
% \bar{\vphi}^T_{\Delta \pi}
% (TG(\pi_e) + G_0)^{-1}
% \Big\{
% -  (\vx_i \vx_i^T)  + 2  (\vx_i \vx_i^T) (TG(\pi_e) + G_0)^{-1} G_0 
% \Big\}
% (TG(\pi_e) + G_0)^{-1}
% \bar{\vphi}_{\Delta \pi}, 
%     \end{split}
% \end{equation}
% where $G_0 = \vPhi_0^T \vPhi_0$ and $G(\pi_e) = \sum_\vx \pi_e(\vx) \vx \vx^T$. 

% \begin{equation}
%     \begin{split}
% &\argmin_{\vPhi} \;
%  
% \bar{\vphi}^T_{\Delta \pi}
%     (\vPhi^T\vPhi + \vPhi_0^{T}\vPhi_0)^{-1} (\vPhi^T\vPhi) (\vPhi^T\vPhi + \vPhi_0^{T}\vPhi_0)^{-1}
%     \bar{\vphi}_{\Delta \pi}\\
% &s.t. \; \min_{\vthe \in \mathcal{C}_\delta(\mD_0)} \big(\pi_1 - (1-\epsilon) \pi_0 \big) \mX \vthe \ge  0, 
%     \end{split}
% \end{equation}


% more info than adaptive 
% \subsection{Baselines}
% \begin{itemize}
%     \item Uniform 
%     \item On-policy with safety constraint
% \end{itemize}
% We start with estimating $V(\pi_1)$. 


==> Safe Exploration for OPE [Camera-ready]/Alg/alg_CP_MAB.tex <==
\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
$\pi_0$, $\pi_1$
, $\mathcal{C}_\delta(\mD_0)$
, $\epsilon$
% , $\mX$
% , $\vPhi_0$
% , $\bar{\vphi}_{\Delta \pi}$
}


Set $i = 0$, $\pi_e^{(0)} = \pi_0$ and $\Theta = \varnothing$. 

\While{Not converge}{
    i = i + 1
    
    Apply convex optimization algorithms to obtain $\pi_e^{(i)}$ by solving
    \begin{equation*}
        \begin{split}
            &\argmin_{\pi_e \in \Pi_{\Delta}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{\pi_e(a)} \\
            % var_{A_t \sim \pi_e}[\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}r(A_t)]\\
            &s.t. \;\;  \vr^T(\pi_e - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \Theta. 
            % \mathcal{C}_\delta(\mD_0). 
            % V(\pi_e) \ge (1-\epsilon) V(\pi_0). 
        \end{split}
    \end{equation*}
    
    \uIf{$min_{\vr \in\mathcal{C}_\delta(\mD_0)} \vr^T(\pi_e^{(i)} - (1-\epsilon) \pi_0) \ge  0$}{
    Terminate the iteration
    }
    \Else{
    Solve $\vr^{(i)} = \argmin_{\vr \in\mathcal{C}_\delta(\mD_0)} \vr^T(\pi_e^{(i)} - (1-\epsilon) \pi_0)$  \tcp*{Constraint is maximally violated}
    
    Update $\Theta = \Theta \cup \{\vr^{(i)}\}$
  }
}

\textbf{Output:} $\pi_e = \pi_e^{(i)}$

 \caption{Safe MAB exploration with the cutting-plane method}\label{alg:CP_MAB}
\end{algorithm}


==> Safe Exploration for OPE [Camera-ready]/Alg/main_alg_FW_CP.tex <==
\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
$\pi_0$
, $\mathcal{C}_\delta(\mD_0)$
, $\epsilon$
, $\mX$
, $\vPhi_0$
, $\bar{\vphi}_{\Delta \pi}$
}

Set $i = 0$, $\pi_e^{(0)} = \pi_0$ and $\Theta = \varnothing$. 

\While{TRUE}{
    i = i + 1
    
    1. Compute the gradient $d^{(i)} = \partial \mJ(\pi_e)/\partial \pi_e|_{\pi_e=\pi_e^{(i)}}$
    
    2. Compute a feasible direction as $\Delta \pi_e$ by solving 
    \begin{equation*}
    \begin{split}
    &\argmin_{w \in \Delta_{K-1}} \;
    d^{(i)} w\\
    &s.t. \; \max_{\vthe \in \Theta} \big((1-\epsilon) \pi_0 - w\big)^T \mX \vthe \le  0. 
    \end{split}
    \end{equation*}
    
    3. Run line search to find the optimal step size $\lambda^{(i)}$ by solving
    $
    \argmin_{\lambda \in [0,1]} \mJ\Big(\pi_e^{(i)} + \lambda (\Delta \pi_e - \pi_e^{(i)}) \Big)
    $

    4. Update $\pi_e^{(i+1)} = \pi_e^{(i)} + \lambda^{(i)} (\Delta \pi_e - \pi_e^{(i)}) $
}
\textbf{Output:} $\pi_e = \pi_e^{(i)}$
 \caption{Optimization for linear bandits with the FW algorithm}\label{alg:FW}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%
% for i in range(self.num_iters_FW):
%     self.compute_gradient()
%     self.compute_direction()
%     self.compute_step_size_and_new_b()
%     self.b = self.new_b
%     if self.last_obj - self.best_obj < self.tol:
%         break
%     self.last_obj = self.best_obj
% return self.b

%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[!h]
\SetAlgoLined
\KwData{
$\pi_0$
, $\mathcal{C}_\delta(\mD_0)$
, $\epsilon$
, $\mX$
, $\vPhi_0$
, $\bar{\vphi}_{\Delta \pi}$
}

Set $i = 0$, $\pi_e^{(0)} = \pi_0$ and $\Theta = \varnothing$. 

\While{TRUE}{
    i = i + 1

    Run the FW algorithm to obtain $\pi_e^{(i)}$ by solving
    \begin{align*}
&\argmin_{\pi_e \in \Delta_{K-1}} \;
\mJ(\pi_e) = 
\bar{\vphi}^T_{\Delta \pi}
    % (T\sum_\vx \pi_e(\vx) \vx \vx^T
    % + \vPhi_0^{T}\vPhi_0)^{-1} (T\sum_\vx \pi_e(\vx) \vx \vx^T) 
    (T\sum_\vx \pi_e(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{-1}
    \bar{\vphi}_{\Delta \pi}\\
% &s.t. \; \min_{\vthe \in \mathcal{C}_\delta} \big(\pi_e - (1-\epsilon) \pi_0 \big) \mX \vthe \ge  0, 
&s.t. \;  \big((1-\epsilon) \pi_0 - \pi_e\big)^T \mX \vthe \le  0, \forall \vthe \in \Theta
    \end{align*}
    
    \uIf{$max_{\vthe \in C_{\delta}} \big((1-\epsilon) \pi_0 - \pi_e^{(i)}\big)^T \mX \vthe \le  0$}{
    Terminate the iteration
    }
    \Else{
    Solve $\vthe^{(i)} = \argmax_{\vthe \in C_{\delta}} \big((1-\epsilon) \pi_0 - \pi_e^{(i)} \big)^T \mX \vthe$  \tcp*{Constraint is maximally violated}
    
    Update $\Theta = \Theta \cup \{\vthe^{(i)}\}$
  }
    % \For{j = 1, \dots, M}{
    
    % }
    % Solve the linear programming () to find the direction 
    
    % Do linear search to find the optimal step size
}

% \For{i = 1, \dots, N}{
% }
\textbf{Output:} $\pi_e = \pi_e^{(i)}$

 \caption{Safe linear bandits exploration with the FW algorithm and the cutting-plane method}\label{alg:FW_CP}
\end{algorithm}


% \begin{algorithm}[!h]
% \SetAlgoLined
% \KwData{
% $\pi_0$
% , $C_{\delta}$
% , $\epsilon$
% , $\mX$
% , $\vPhi_0$
% , $\bar{\vphi}_{\Delta \pi}$
% }

% Set $i = 0$, $pi^{(0)} = \pi_0$ and $\Theta = \varnothing$. 

% \While{TRUE}{
%     i = i + 1

%     Run the FW algorithm to obtain $\pi^{(i)}$ by solving
%     \begin{align*}
% &\argmin_{b \in \Delta_{K-1}} \;
% \mJ(b) = 
% \bar{\vphi}^T_{\Delta \pi}
%     % (T\sum_\vx b(\vx) \vx \vx^T
%     % + \vPhi_0^{T}\vPhi_0)^{-1} (T\sum_\vx b(\vx) \vx \vx^T) 
%     (T\sum_\vx b(\vx) \vx \vx^T+ \vPhi_0^{T}\vPhi_0)^{-1}
%     \bar{\vphi}_{\Delta \pi}\\
% % &s.t. \; \min_{\vthe \in \mathcal{C}_\delta} \big(b - (1-\epsilon) \pi_0 \big) \mX \vthe \ge  0, 
% &s.t. \; \max_{\vthe \in \Theta} \big((1-\epsilon) \pi_0 - b\big)^T \mX \vthe \le  0, 
%     \end{align*}
    
%     \uIf{$max_{\vthe \in C_{\delta}} \big((1-\epsilon) \pi_0 - b\big)^T \mX \vthe \le  0$}{
%     Terminate the iteration
%     }
%     \Else{
%     Solve $\vthe^{(i)} = \argmax_{\vthe \in C_{\delta}} \big((1-\epsilon) \pi_0 - \pi^{(i)} \big)^T \mX \vthe$  \tcp*{Constraint is maximally violated}
    
%     Update $\Theta = \Theta \cup \{\vthe^{(i)}\}$
%   }
%     % \For{j = 1, \dots, M}{
    
%     % }
%     % Solve the linear programming () to find the direction 
    
%     % Do linear search to find the optimal step size
% }

% % \For{i = 1, \dots, N}{
% % }

%  \caption{FW algorithm for safe linear bandit exploration with the cutting-plane method}\label{alg:FW_CP}
% \end{algorithm}


==> Safe Exploration for OPE [Camera-ready]/Archive/8_discussion_points.tex <==
\section{Discussion Points}



% \todob{Restructure the above paragraph to better motivate what we do. In off-policy optimization, we estimate $\widehat{V}(\pi_1; \mD)$ for some known $\pi_1$ and from known $\mD$. This is typically used to test if $V_r(\pi_1) > V_r(\pi_0)$. How $\mD$ arises is never questioned. We study the problem of collecting $\mD$ to decide $V_r(\pi_1) > V_r(\pi_0)$ as efficiently as possible.}
% \todorw{Let's discuss should we discuss more in the introduction and keep this setup section concise?}


\todorw{Let's discuss the space issue as well. Some details/derivations/contents need to be moved to the appendix anyway. ICML format instruction requires name+year citation. }



==> Safe Exploration for OPE [Camera-ready]/Archive/9_Differentiable_Policy.tex <==
\subsection{Differentiable Policy}

==> Safe Exploration for OPE [Camera-ready]/Archive/9_Discussions.tex <==
\section{Discussion points to be resolved}
% Note that
% \begin{equation}
%     \begin{split}
%         var_{A_t \sim b}[\frac{\pi(A_t)}{b(A_t)}r(A_t)] 
%         = \sum_a \frac{\pi^2(a) r^2(a)}{b(a)}
%     \end{split}
% \end{equation}
% but this may not hold for \pi_{\Delta}
\begin{itemize}
    % \item The main goal of the discussion above is to motivate why we can ignore the second term in solving an efficient allocation. Alternatively, we can direct start our discussions with an exact design, and then relax to the continuous design case, which might be more natural. Though we need to introduce design instead of policy earlier. 
% Any other suggestions?
% from our observe in estimating $L$ and $U$ from the logged data 
\end{itemize}

% The second term can be dropped when we consider a fixed design where $N_a = \sum_t \I(A_t = a) \propto b(a)$.  \todob{I do not understand why the second term can be dropped. It does not seem to be zero. Specifically, even for a fixed design, when $A_t \sim b$, the term is not zero.}

% Although such a design probably can be obtained exactly, it can be our motivation to consider optimizing $b$ with this first term as the objective (where $b$ is used to compute the allocation proportions), and in implementation we may still need randomized rounding would be needed. 
% % Ignoring the second term for now (as in SafeOD)
% In this case, we consider the value estimator to be IPW with estimated assignment probability, i.e., the plug-in estimator with sample mean $\widehat{V}(\pi) = \sum_{a \in [K]} \frac{\sum_t \I(A_t = a) R_t}{\sum_t \I(A_t = a)}$. 
% \todob{Why do we need this plug-in estimator? I thought that we do inverse propensity scores. A: the main reason is, with a deterministic allocation rule, the standard IPW is not well defined.}


==> Safe Exploration for OPE [Camera-ready]/Archive/9_MAB_IPW_estiamted_propensity.tex <==
\subsection{Multi-armed bandits  with inverse probability weighting}\label{sec:MAB_IPW_alt}
We start our discussion with estimating the value of a $K$-armed bandit  policy using the popular inverse probability weighting (IPW) estimator \cite{dudik2014doubly}. 
For any dataset $\mD = \{(A_i, R_i)\}$, 
the IPW estimator is defined as 
$\widehat{V}_{IPW}(\pi; \mD) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \frac{\pi(A_i)}{\hat{b}(A_i)}R_i$, where $\hat{b}(a) = |\mD|^{-1}\sum_{(A_i, R_i) \in \mD} \I(A_t = a)$. 
Note that here we use the estimated propensity $\hat{b}(a)$. 
A well-known but perhaps counter-intuitive result \cite{brumback2009note} says that, even if $\mD$ is collected by following $b$ and $b$ is known, $\widehat{V}_{IPW}(\pi; \mD)$ is more efficient than plugging-in $b$. 

We aim to design the optimal way to collect the new dataset of size $T$, which is equivalent to allocating the $T$ budgets to the $K$ arms. 
Let $N_a$ be the number of data points assigned to the $a$th arm, 
set $b(a) = N_a / T, \forall a \in [K]$, 
and denote the resulting dataset by $\mD_b$. 

We first consider the case where there is no logged dataset $\mD_0$. 
Our objective can then be written as
\begin{align*}
            &\argmin_{b \in \Delta_{K - 1}} var\big(\widehat{V}_{IPW}(\pi_1; \mD_{b}) - \widehat{V}_{IPW}(\pi_0; \mD_{b}) \big)\\
        &s.t. \;\; V_{\vr}(b) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K. 
\end{align*}
This problem is particularly challenging due to (i) the dependency of the objective on $b$ is complex, 
and (ii) the safety constraint involves the unknown function $V$ and hence not easy to guarantee. 

% \textbf{Objective function. }
We aim to first transform the objective into a tractable form. 
Let $\pi_{\Delta} = \pi_1 - \pi_0$ and $\sigma^2_a = var(R_t \mid A_t = a), \forall a \in [K]$. 
We have 
\begin{align}
&T \times var\Big(\widehat{V}_{IPW}(\pi_1; \mD_{b}) - \widehat{V}_{IPW}(\pi_0; \mD_{b}) \Big)\nonumber\\
&= 
\sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \sigma^2_a 
 \label{eqn:MAB_objective_alt}
\end{align}
Without safety constraints, 
the optimal allocation rule is similar with the Neyman allocation in statistics \cite{neyman1992two}, i.e., $b(a) \propto \sigma_a |\pi_{\Delta}(a)|$. 
Besides, perhaps surprisingly, following similar arguments, we can show that the on-policy strategy (i.e., by setting $b = \pi_1$) is not even optimal in minimizing $var\big(\widehat{V}(\pi_1; \mD_{b}))$, 
when $\sigma_a$'s are different. 

% $\{A_t\}_{t=1}^T \sim \text{Multinomial}(T, b)$, 
%  = T \times b(a)
The first challenge to solving \eqref{eqn:MAB_objective} is that, it is hard to guarantee that $N_a$'s are all integers for the minimizer $b$. 
However, various randomized rounding techniques \hl{[cite]} can be applied to obtain a set of integers $\{N_a\}$ that is close to the continuous solution, and the variance inflation is guaranteed to be negligible when $K$ is small compared with $T$. % enough

% derivations in \eqref{eqn:MAB_objective}  may not hold any longer. That is why I introduced a new IPW
% " " does not make sense any longer
The second challenge is that $\sigma_a$ is typically not known \textit{a priori}. 
Without additional information and given the fact the second moment is typically more difficult to estimate than the first moment, 
we consider an upper bound of the objective, by replacing every $\sigma_a$ with their joint upper bound. 
With this relaxation, our objective reduces to 
\begin{equation*}
    \begin{split}
    \argmin_{b  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)}
    \end{split}
\end{equation*}
Without safety constraints, 
the optimal allocation rule is similar with the proportional allocation in statistics \cite{fuller2011sampling}, i.e., $b(a) \propto |\pi_{\Delta}(a)|$. 
% Again, the exact integer allocations can be solved via randomized rounding. 
% This exactly corresponds to the on-policy strategy. 

% \textbf{Safety constraint. }
With a tractable and appropriate surrogate objective, we are now ready to consider the safety constraint $V_{\vr}(b) \ge (1-\epsilon) V_{\vr}(\pi_0), \forall \vr \in [0,1]^K$. 
The first observation is that, the constraint is equivalent to $b(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K]$. 
This is mainly due to that there is no any information on $\vr$ and we need to ensure the safety constraint under the worst case. 
Specifically, 
when there exists at least one arm $a$ such that $b(a) < (1-\epsilon) \pi_0$, we can always construct a instance to violate the constraint, where $r(a) = 1$ and $r(a') = 0, \forall a' \neq a$. 

\textbf{Optimization without side information. }
Therefore, we finally achieve a desired optimization objective, by solving which we can obtain an efficient and safe continuous design for our OPE task: 
\begin{equation}
    \begin{split}
        &\argmin_{b  \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\; b(a) \ge (1-\epsilon) \pi_0(a), \forall a \in [K] . 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_no_logged_alt}
\end{equation}
This problem is convex and hence can be efficiently solved by many convex optimization algorithms \cite{boyd2004convex}. 
% For general values of $\{\sigma_a\}$, though this solution will not be globally optimal,  we can provide upper bounds instead. 


% \begin{figure}
%     \centering
%     \includegraphics[width = 10cm]{Fig/MAB.png}
%     \caption{MAB: $V(\pi_1)$}
%     % \caption{Caption}
%     % \label{fig:my_label}
% \end{figure}

\textbf{Utilization of side information. }
\hl{update here.!}
Next, we consider there is side information that allows us to improve on \eqref{eqn:MAB_IPW_no_logged}. 
We assume we have a logged dataset $\mD_0$ generated by a historical behaviour policy $b_0$. 
We assume $b_0$ is known for simplicity, and otherwise it can be estimated via methods standard in the OPE literature. 
We expect the information in $\mD_0$ will have impact on both our objective and safety constraint. 
Specifically, the original problem can be written as 
\begin{equation}
    \begin{split}
        &\argmin_{b \in \Delta_{K - 1}} 
        % (N+T)^{-2}
        var \Big(
        \sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{b(A_t)} R_t
        + \sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
        \Big)\\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\; min_{\vr \in \mathcal{C}_\delta(\mD_0)} \vr^T(b - (1-\epsilon) \pi_0) \ge 0. 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_w_logged_raw_alt}
\end{equation}  
Here, $\mathcal{C}_\delta(\mD_0)$ is an $(1-\delta)$-confidence region on $\vr$ obtained from $\mD_0$. 
For instance, we can construct an $(1-\delta / K)$-confidence interval for each arm separately. 
Alternatively, one may consider a Bayesian setup where there is a prior on $\vr$, and $\mathcal{C}_\delta(\mD_0)$ is the credible intervals derived from the corresponding posteriors. 

% [\vL(\delta, \mD_0), \vU(\delta, \mD_0)]


Perhaps surprisingly, thanks to the independence between $\mD_b$ and $\mD_0$, the objective of     \eqref{eqn:MAB_IPW_w_logged_raw} is equal to
$
var \Big(
\sum_{t=1}^T \frac{\pi_{\Delta}(A_t)}{b(A_t)} R_t \Big)
+ var\Big(\sum_{(A_i, R_i) \in \mD_0} \frac{\pi_{\Delta}(A_i)}{b_0(A_i)} R_i
\Big)$, 
where the second term does not depend on $b$ can hence can be dropped in the objective. 
In other words, the additional dataset $\mD_0$ does not affect the optimization objective. 
The main reason is that in IPW, every data point contributes independently to the estimator. 
This may not be the case for some other OPE estimators, as will be shown later. 

\textbf{Optimization with side information. }
Therefore, by similar arguments with \eqref{eqn:MAB_IPW_no_logged}, we can consider the following optimization problem
\begin{equation}
    \begin{split}
        &\argmin_{b \in \Delta_{K - 1}} \sum_{a \in [K]} \frac{\pi^2_{\Delta}(a)}{b(a)} \\
        % var_{A_t \sim b}[\frac{\pi_{\Delta}(A_t)}{b(A_t)}r(A_t)]\\
        &s.t. \;\;  \vr^T(b - (1-\epsilon) \pi_0) \ge 0, \forall \vr \in \mathcal{C}_\delta(\mD_0). 
        % V(b) \ge (1-\epsilon) V(\pi_0). 
    \end{split}
    \label{eqn:MAB_IPW_w_logged_alt}
\end{equation}
We note this problem is particularly challenging as the constraint implicitly contains a \textit{infinite} number of constraints. 
With the observation that, for any finite set $\Theta \subset \Delta_{k-1}$, 
$min_{\vr \in \Theta} \vr^T(b - (1-\epsilon) \pi_0) \ge 0$ is a system of linear constraints. 
Therefore, we propose to solve \eqref{eqn:MAB_IPW_w_logged} by combining convex optimization with the cutting-plane method \cite{bertsimas1997introduction}. 
Specifically, the cutting-plane method iteratively refines a finite set of constraints to approximate the infinite set of constraints through adding then one by one, until no constraint in the infinite set is violated. 
We present the algorithm details in Appendix \ref{sec:optimization_MAB}. 

% The underlying principle is to approximate the feasible region of a nonlinear (convex) program by a finite set of closed half spaces and to solve a sequence of approximating linear programs.

\hl{[explain the allocation more clearly]}

% We note that, with IPW as the value estimator, the objective does not change when we also utilize the logged dataset $\mD_0$ in the objective in addition to in the safety constraint. 
% This is because the additive structure of IPW. 
% This may not be the case when we consider other estimators. 
% although it looks like we only utilize the side information (which typically comes from a ) in the safety constraint but not in the objective, 
% and when we only utilize (?) it in the safety constraint




==> Safe Exploration for OPE [Camera-ready]/Archive/9_Setup.tex <==


% \section{Setup}


% \begin{align*}
%     r(\vx_t, a) &= \vx_t^T \vthe_a, \forall a \in \mathcal{A} \; \text{(disjoint, finite arm)} \\ % including two-arm (A learning?)
%     r(\vx,a) &= \vphi^T_{\vx,a} \vthe \; \text{(transformed feature)}\\ % \Mean(R_t|\vx_t = \vx, A_t = a) = 
%     % , \forall a \in \mathcal{A} \\ % including two-arm (A learning?)
%     r(\mX,a) &= \vx^T_{a,t} \vthe \; \text{(one context per arm)}\\ 
%     r(\vx_t) &=  \vx_t^T \vthe  \;\; \text{(x is just arm; can be a fixed set, or infinite)}     % linear regression 
% \end{align*}

% \textbf{Setup.} 
% \begin{equation}
%     \begin{split}
%     r(\vx,a) &= \vphi^T_{\vx,a} \vthe^*\\ % \Mean(R_t|\vx_t = \vx, A_t = a) = 
%     V(\pi) &= \Mean_{\vx \sim p(\vx), a \sim \pi(a \mid \vx) }  \; r(\vx, a)
%     % V(\pi) &= \ \Mean_{\vx \sim p(\vx)}  \sum_{a \in \mathcal{A}} \pi(a \mid x) r(x, a)\\
%     % , \forall a \in \mathcal{A} \\ % including two-arm (A learning?)
%     \end{split}
% \end{equation}



% \item : i.i.d. sampled following a behaviour policy $b_0$, which could be the same with $\pi_0$
% \item the context distribution $p(\vx)$ or possibly a large context dataset $\mD'_{\vx}$
% \item a function to construct the transformed feature  $\vphi_{\vx, a}$


% Suppose we have access to (some are optional):
% \begin{itemize}
    % or adaptively collected
    % \item an off-policy optimization algorithm $\mathcal{O}$ which maps a dataset to a policy
%     \item budget $T$ and risk tolerance $\epsilon \in (0,1)$ % safety threshold
% \end{itemize}


% \textbf{Goal. }
% % We would like to design a  (or an adaptive one?) to collect a new dataset $\mD = \{(\vx_t, A_t, R_t)\}_{t=1}^T$ where $A_t \sim b(\cdot|\vx_t)$, 
% so that 
% % (i) during the $T$ interactions, we satisfy the safety constraint that $\sum_t\Mean_{\vx_t \sim p(\vx), A_t \sim b(\cdot \mid \vx_t)}R_t \ge (1-\epsilon) \sum_t\Mean_{\vx_t \sim p(\vx), A_t \sim \pi_0(\cdot \mid \vx_t)} R_t$ for any problem instance (or with probability at least $\delta$ evaluated using logged dataset? expectation over x?), 
% % (could be a stage-wise as well) 
% and (ii) after the $T$ interactions, we achieve one of the following goals: 
% % \begin{itemize}
% %     \item \textbf{Evaluation}: we can consider several goals, of (potentially) increasing difficulty
%     \begin{itemize}
%         \item minimize $var(\widehat{V}(\pi_1))$: suppose we have enough data following  $\pi_0$ and hence its value can be well estimated, which is a common starting point. (We also need to assume the linear reward function is correctly specified, and hence the DM estimator is unbiased, and hence we only need to minimize the variance. )
%         \item maximize $\prob( \widehat{V}(\pi_1) - \widehat{V}(\pi_0) \ge 0  \mid V(\pi_1) - V(\pi_0) \ge \delta)$
%         % \item maximize $\prob{(\widehat{V}(\pi_1) - \widehat{V}(\pi_0)) (V(\pi_1) - V(\pi_0)) > 0}$
%         \item maximize $\prob(reject \;\; \{V(\pi_1) - V(\pi_0) \le 0 \} \mid V(\pi_1) - V(\pi_0) \ge \delta)$
%         % \item continuously monitor the test to allow early stop
%     \end{itemize}
    % our new policy $\pi' = \mathcal{O}\Big(\mD \bigcup \mD'\Big)$ yields high value in expectation (or high-probability bound?), i.e., we aim to maximize $\Mean(V(\pi'))$ where the expectation is taken over $\mD'$ and hence $\pi'$.
    % \item \textbf{Optimization}: our new policy $\pi' = \mathcal{O}\Big(\mD \bigcup \mD_0\Big)$ yields high value in expectation (or high-probability bound?), i.e., we aim to maximize $\Mean(V(\pi'))$, where the expectation is taken over $\mD$ and hence $b$.
% \end{itemize}

% There are several moving parts: 
% \begin{enumerate}
%     % \item Objective
%     \item Safety constraint: there are a few ways to define
%     \item Logged dataset: should enter (provide information for) both the objective and the safety constraint
%     \item Value estimator can be different (IPW, DM, DR)
%     \item Bandit problem setup: MAB, nonstochastic linear bandits, 
%     contextual MAB, stochastic contextual linear bandits, etc. 
%     % linear generalization, contextual MAB, etc. 
% \end{enumerate}

% Distributional G-optimal design?
% back to linear regression? so simple?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% functional form of pi and pi_0 matter? [let us start with linear]

% \subsection{Related work and comparison}


==> Safe Exploration for OPE [Camera-ready]/Archive/9_allocation_rule.tex <==
\subsection{From exploration policy to allocation rule}
In the previous discussion, we aim to solve an efficient exploration policy $b$, which is a (conditional) distribution over arms. 

For tractability, NP-hard.

In this section, we discuss how to utilize $b$ to collect the dataset $\mD_b$ of size $T$. 


\hl{Read more. }

==> Safe Exploration for OPE [Camera-ready]/Archive/9_derivations_IPW.tex <==
\subsection{Inverse IPW}
\begin{equation}
    \begin{split}
   V_{\pi_1}  &= \Mean  \sum_a Y(a) \pi_1(a \mid \vx) = \Mean \frac{R_t \pi_1(A_t \mid \vx_t)}{b(A_t \mid \vx_t)}\\
   \widehat{V}_{\pi}  &= N^{-1} \sum_t\frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} 
    \end{split}
\end{equation}

Positivity assumption: $\forall (\vx, a)$, if $P(\vx) > 0$ and  $\pi_1(a \mid \vx ) > 0$, then $b(a \mid \vx ) > 0$. 

\begin{equation}
    \begin{split}
\argmin_b \;\;
&var \Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
+ 
var_{\vx_t} \Mean_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
+ 
var_{\vx_t} \Mean_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]\\
&= 
\Mean_{\vx_t} var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{R_t  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \mid \vx_t \Big]
% + 
% var_{\vx_t} \Mean_{A_t \sim \pi_1(a \mid \vx_t)}\Big[R_t \mid \vx_t \Big]
+ const\\
&= 
\Mean_{\vx_t} 
\Big\{
\Mean_{A_t \sim b(a \mid \vx_t)}\Big[ var(R_t \mid A_t, \vx_t) \frac{ \pi^2_1(A_t \mid \vx_t) }{b^2(A_t \mid \vx_t)}  \Big]
+
var_{A_t \sim b(a \mid \vx_t)}\Big[ \frac{\Mean(R_t \mid A_t, \vx_t)  \pi_1(A_t \mid \vx_t) }{b(A_t \mid \vx_t)} \Big]
\Big\}
+ const\\
&= 
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}
+ const
    \end{split}
\end{equation}
Without the safety constraint and ignoring the logged dataset, and suppose we know  $\Mean[R^2_t \mid \vx_t, A_t] $, the optimal design should be the Neyman allocation, i.e., 
\begin{equation}
    \begin{split}
    b(a \mid \vx) \propto \sqrt{var(R_t \mid A_t = a, \vx_t = \vx)} \times  \pi_1(a \mid \vx), \forall \vx
    \end{split}
\end{equation}

There are several issues we need to address:
\begin{enumerate}
    \item $var(R_t \mid A_t = a, \vx_t = \vx)$ is unknown: The unknown variance can be replaced with the plug-in estimator, or we can consider some less optimal ones? 
% Since 
    \item The safety constraint
    \item The existing offline dataset: The existing offline dataset can be accommodated via results from stratified sampling, as in \cite{kallus2021optimal}. 
\end{enumerate}
% adaptively collected
% support deficiency



The safety constraint needs a lower bound for IPW-based value estiamtor (under potential support deficiency?) 
Based on the asymptotic distribution 

\begin{align*}
          \sqrt{n}(\widehat{V}_{b} - V_{b})
    %   \sim  
    &\convergeD
      \mathcal{N}(\vzero, \sigma_1^2), 
      \quad  
      \sigma_1^2 
      = 
    \Mean_{b_0}\Big(\frac{R_t  b(A_t \mid \vx_t)}{b_0(A_t \mid \vx_t)}  - V_{b} \Big)^2, 
    %   \Mean\Big(\frac{(Y_i - V_{\delta})^2}{\prob_{\delta(\vx_t)}} \Big)
\end{align*}
where $b_0$ is the behaviour policy for $\mD_0$. 
A lower bound on $V_b$ is then $\widehat{V}_{b} - z_{\alpha} n^{-1/2} \sigma_1$. 
Hence, we may need to solve the problem above, under a constraint similar with (too conservative?)
$  \widehat{V}_{b} = |\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i)   \ge (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1$. 
% Given any $\vx$, we would like to solve
% \begin{align*}
%     \argmin_{b} \; 
%     \sum_a 
%     \frac{\Mean[R^2_t \mid \vx, a]  \pi^2_1(a \mid \vx)}{b(a \mid \vx)} 
% \end{align*}

% suppose the variance level is the same. 
% stratified sampling

\begin{equation}
    \begin{split}
    &\argmin_b    
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}\\
&s.t. \;
|\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i)   \ge (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1  
    \end{split}
\end{equation}

We can parameterize $b$ as a differentiable policy and solve the Lagrange via stochastic gradient descent-ascent? 
\begin{equation}
    \begin{split}
min_b \max_{\lambda \ge 0}    L(b, \lambda)
    = \Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\} 
+ \lambda 
\Big\{
l_0 - |\mD_0|^{-1} \sum_i\frac{R_i}{b_0(A_i \mid \vx_i)} b(A_i \mid \vx_i) 
\Big\}, 
    \end{split}
\end{equation}
where $l_0 = (1-\epsilon) V_{\pi_0} + z_{\alpha} n^{-1/2} \hat{\sigma}_1$. 


 
 
Alternatively, we can consider
\begin{equation}
    \begin{split}
&\argmin_b    
\Mean_{\vx_t} 
\Big\{
\sum_a
\frac{var(R_t \mid A_t = a, \vx_t)  \pi^2_1(a \mid \vx_t) }{b(a \mid \vx_t)}  
\Big\}\\
&s.t. \;  b(a\mid\vx) \ge (1-\epsilon) \pi_0(a\mid\vx), \forall a, \vx, 
    \end{split}
\end{equation}
which can probably be solved via constrained optimization. 
Alternatively, we can consider the policy mixture approach in \cite{zanette2021design}, that is, do \textit{pseudo} online learning with the offline dataset from $t = 0$, and at each time point, we choose the direction that minimize the variance under the constraint, and finally apply a mixture policy. 

% Assuming a linear value function?:
% \begin{align*}
%     \min_{\vthe \in \mathcal{C}_\delta} \quad \Mean_{\vPhi \sim b} \big(\vone^T \vPhi\vthe\big)  
%     \ge (1-\epsilon) \max_{\vthe \in \mathcal{C}_\delta}  \Mean_{\vPhi \sim \pi_0} \big(\vone^T \vPhi\vthe\big)  
% \end{align*}

% Try to further simplify the form. 

% \begin{align*}
%     \argmin_{b} \; &\Mean_{\vx_t \sim p(\vx), A_t \sim b(a \mid \vx_t) }\Big(\frac{R_t  \pi_1(A_t \mid \vx_t)}{b(A_t \mid \vx_t)}  - V_\pi \Big)^2\\
%     % s.t. \quad 
%     s.t. \; &\min_{\vthe \in \mathcal{C}_\delta} \quad \Mean_{\vPhi \sim b} \big(\vone^T \vPhi\vthe\big)  
%     \ge (1-\epsilon) \max_{\vthe \in \mathcal{C}_\delta}  \Mean_{\vPhi \sim \pi_0} \big(\vone^T \vPhi\vthe\big)  
%     % &XX1
% \end{align*}

\subsection{Adaptive exploration policy}
maximize the least confident direction + check the lower bound to make sure no violation

\subsection{Fixed exploration policy}
Achieve that idea in an offline fashion [by simulation] [because of the fixed] [a simulation based procedure]


==> Safe Exploration for OPE [Camera-ready]/Archive/main_draft.tex <==
% \input{FRONT}
\input{Style}
\title{Safe Exploration for Efficient Off-policy Evaluation}
\date{\today}
\author{}
% Efficient
% Optimization

\begin{document}
\maketitle
\linenumbers
% \pagestyle{fancy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \input{1_Setup}
\input{1_Intro}

\input{2_Method}

\input{3_Theory}

\input{4_Expt}



\bibliographystyle{aaai2021.bst}
\bibliography{bib}

\appendix
\newpage


\input{9_Appendix_other_settings}


\end{document}


==> Safe Exploration for OPE [Camera-ready]/Archive/testing.tex <==

\subsection{Connection with hypothesis testing}
% \textbf{Connection with hypothesis testing.} 
In real applications, one important task is to test whether or not the target policy $\pi_1$ is significantly better than $\pi_0$, which impacts the decision-making of deploying $\pi_1$. 
We next present the relationship between the power of such a test and our ultimate optimization objective $var\big(\widehat{V}_{IPW}(\pi_1; \mD_{e}) - \widehat{V}_{IPW}(\pi_0; \mD_{e}) \big)$. 
We focus on the case without side information for simplicity, and it is straightforward to accommodate $\mD_{0}$. 
% extend to the case with
Specifically, we consider the test
\begin{align*}
    H_0: V(\pi_1) \le V(\pi_0) \quad \text{v.s.} \quad H_1: V(\pi_1) > V(\pi_0). 
\end{align*} 
% $\sigma(\pi_e) {=} \sqrt{var\big(\frac{\pi_{\Delta}(A_t)}{\pi_e(A_t)}R_t\big)}$
% $\sigma(\pi_e) {=} \sqrt{var(\pi_e(A_t)^{-1}\pi_{\Delta}(A_t)R_t)}$
Denote our raw objective \eqref{eqn:raw_MAB_obj} by $\sigma(\pi_e)$  and let $\hat{\sigma}(\pi_e)$ be a consistent estimator with $\mD_e$ (typically the plug-in estimator with sample variance). 
By the central-limit theorem and the Slutsky’s lemma, we have 
\scalebox{0.92}{\parbox{\linewidth}{%
\begin{align*}
\frac{\sqrt{T}}{\hat{\sigma}(\pi_e)}
    \Big[
    \big(\widehat{V}(\pi_1; \mD_{e}) 
    {-} \widehat{V}(\pi_0; \mD_{e}) \big)
    {-} \big(V(\pi_1) {-} V(\pi_0)\big)\Big]
    \overset{d}{\to} \normal(0, 1), 
\end{align*}
}}
% \begin{align*}
%     \hat{\sigma}(\pi_e)^{-1} \sqrt{T}
%     &\Big[
%     \big(\widehat{V}(\pi_1; \mD_{e}) 
%     - \widehat{V}(\pi_0; \mD_{e}) \big)\\
%     &\quad- \big(V(\pi_1) - V(\pi_0)\big)\Big]
%     \overset{d}{\to} \normal(0, 1), 
% \end{align*}
% $\hat{\sigma}(\pi_e)^{-1} \sqrt{T}
% \big(\widehat{V}(\pi_1; \mD_{e}) 
% {-} \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}$
when $T$ grows.  %  \to \infty
Therefore, an (asymptotically) $\alpha$-level test is to reject the null when 
\begin{align*}
    \hat{\sigma}(\pi_e)^{-1} \sqrt{T}
\big(\widehat{V}(\pi_1; \mD_{e}) 
{-} \widehat{V}(\pi_0; \mD_{e}) \big) \ge z_{1-\alpha}, 
\end{align*}
where $z_{1-\alpha}$ is  the upper $\alpha$th quantile of the standard normal distribution. 
For any $\Delta > 0$, the (asymptotic) power under the local alternative $H_1 : V(\pi_1) - V(\pi_0) {=} \Delta / \sqrt{T}$ 
is hence 
$1 - \Phi\big(z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta\big)$, where $\Phi(\cdot)$ is the cumulative distribution function of standard Gaussian. 
Since the other terms are all constant, it is clear that $\sigma(\pi_e)$ determines the power. 
Therefore, with a fixed budget, one can improve the power by designing a better policy $\pi_e$ to reduce $\sigma(\pi_e)$, which corresponds to our objective. 
Such a connection can be built similarly for the other setups considered in this paper (see Appendix \ref{sec:other_testing} for details). 
\todob{Do we want to have something more finite-sample?} 
\todorw{Let's discuss more. Not sure how. In Stats and Econ, the value tests I am aware of are all asymptotic. (besides boostrapping-based)}
\todob{We do not really do policy evaluation. That would be estimate $V(\pi_1)$. We do lift evaluation. This is what $V(\pi_\Delta)$ means. The problems are algebraically equivalent though. We can claim that we can do both. We focus on $V(\pi_\Delta)$ because it is more practical.}
% in similar ways
% \hl{hold for other settings?}
% both $V(\pi_1) - V(\pi_0)$ and $z_{1-\alpha}$


% $\prob\Big(Z \ge z_{1-\alpha} - \sigma(\pi_e)^{-1} \Delta \Big)$
% $Z$ is a standard normal random variable. 

==> Safe Exploration for OPE [Camera-ready]/Fig/illustration.tex <==
\begin{figure*}[!t]
\centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\begin{subfigure}{.3\textwidth}
  \centering
    % \vspace{.2cm}
  \includegraphics[width=\linewidth]{Fig/safeOD_OPE-OPE.pdf}
  \vspace{-0.5cm}
  \caption{
  Standard OPE. 
  }
\end{subfigure}%
% \hspace{.3cm}
\begin{subfigure}{.55\textwidth}
  \vspace{-.2cm}
  \centering
  \includegraphics[width=\linewidth]{Fig/safeOD_OPE-Ours.pdf}
  \vspace{-1.1cm}
  \caption{SEPEC: designing a safe and efficient exploration policy to collect high-quality data for a given OPE task. 
  }
\end{subfigure}%
\vspace{-.3cm}
\caption{Comparisons between the standard OPE setting and our proposal.}\label{fig:illustration}
\vspace{-0.3cm}
% safe design of experiments
\end{figure*}


==> Safe Exploration for OPE [Camera-ready]/Fig/illustration_one_graph.tex <==
\begin{figure}[!t]
\hspace{-.5cm}
\begin{subfigure}{.55\textwidth}
%   \vspace{-.2cm}
  \centering
  \includegraphics[width=\linewidth]{Fig/safeOD_OPE-one-graph.pdf}
%   \vspace{-1.1cm}
\end{subfigure}%
% \vspace{-.3cm}
\caption{SEPEC: designing a safe and efficient exploration policy to collect high-quality data for a given evaluation task. 
}
\label{fig:illustration}
% \vspace{-0.3cm}
% safe design of experiments
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Fig/more_setting_results.tex <==
\renewcommand{\sharedwidthSubFig}{0.9}
\renewcommand{\sharedwidth}{0.52}
\renewcommand{\sharedheight}{3cm}
\renewcommand{\hbetween}{0.1cm}
\renewcommand{\vbetween}{-0.5cm}

\begin{figure}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/MAB.pdf}
    \vspace{\vbetween}
  \caption{
  MAB with IPW. 
  }
\end{subfigure}%

% \hspace{\hbetween}
\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/CMAB.pdf}
    \vspace{\vbetween}
  \caption{CMAB with IPW.}
\end{subfigure}%

\hspace{-0.5cm}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/LB.pdf}
  \vspace{\vbetween}
  \caption{Linear bandits with DM.}
\end{subfigure}%
\vspace{-0.2cm}
\caption{Experiment results. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
For methods that consider the safety constraint, the losses from safety violation are around zero and hence may overlap.}\label{fig:more_setting_CMAB}
% safe design of experiments
\vspace{-0.5cm}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Fig/more_settings.tex <==
\begin{figure}[!t]
  \centering
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337CMAB_T2000K5sigma3.pdf}
  \caption{$T = 2000, K = 5, \sigma = 3$.}
\end{subfigure}%
\hspace{.5cm}
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337CMAB_T200K20sigma2.pdf}
  \caption{$T = 200, K = 20, \sigma = 2$.}
\end{subfigure}%
\caption{Experiment results for CMAB under other combinations of setting parameters.}\label{fig:more_CMAB}
\end{figure}


\begin{figure}[!t]
  \centering
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337LB_T100K100sigma2d10.pdf}
  \caption{$T = 100, K = 100, \sigma = 2, d= 10$.}
\end{subfigure}%
\hspace{.5cm}
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337LB_T200K100sigma2d3.pdf}
  \caption{$T = 200, K = 100, \sigma = 2, d = 3$.}
\end{subfigure}%
\caption{Experiment results for LB under other combinations of setting parameters.}\label{fig:more_LB}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Fig/real_data_results.tex <==
\begin{figure}[!t]
  \centering
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337CMAB_real.pdf}
  \caption{CMAB with IPW.}\label{fig:real_CMAB}
\end{subfigure}%
\hspace{.5cm}
\begin{subfigure}{0.48\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = 3.5cm]{Fig/01201337LB_real.pdf}
  \caption{Linear bandits with DM.}\label{fig:real_LB}
\end{subfigure}%
\caption{Experiment results on the MNIST dataset. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
For methods that consider the safety constraint, the losses from safety violation are around zero and hence may overlap.}\label{fig:real}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Fig/simu_res_old.tex <==
% \newcommand{\sharedwidthSubFig}{0.85}
\newcommand{\sharedwidth}{0.5}
\newcommand{\sharedheight}{3cm}
\newcommand{\hbetween}{0.1cm}
\newcommand{\vbetween}{-0.6cm}
\newcommand{\hleft}{-0.3cm}

\begin{figure}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/MAB.pdf}
    \vspace{\vbetween}
  \caption{
  MAB with IPW. 
  }
\end{subfigure}%

% \hspace{\hbetween}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/CMAB.pdf}
    \vspace{\vbetween}
  \caption{CMAB with IPW.}
\end{subfigure}%

\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/LB.pdf}
  \vspace{\vbetween}
  \caption{Linear bandits with DM.}
\end{subfigure}%
\vspace{-0.2cm}
\caption{Experiment results. 
The errorbars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
% For methods that consider the safety constraint, 
The losses from safety violation for safe methods are all around zero and hence overlap.}\label{fig:simu}
% safe design of experiments
\vspace{-0.5cm}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Fig/simu_results.tex <==
% \newcommand{\sharedwidthSubFig}{0.85}
\newcommand{\sharedwidth}{0.5}
\newcommand{\sharedheight}{3.2cm}
% \newcommand{\sharedheight}{3.5cm}
\newcommand{\hbetween}{0.1cm}
% \newcommand{\vbetween}{-0.6cm}
\newcommand{\vbetween}{-0.5cm}
\newcommand{\hleft}{-0.3cm}

\begin{figure}[!t]
% \centering
% \includegraphics[width=.8\textwidth]{figures/diag_with_cost.png}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/01201337RMSE.pdf}
    \vspace{\vbetween}
  \caption{
  Estimation efficiency measured by RMSE. 
  }
\end{subfigure}%

% \hspace{\hbetween}
\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/01201337risk.pdf}
    \vspace{\vbetween}
  \caption{Risk from safety violation.}
\end{subfigure}%

\hspace{\hleft}
\begin{subfigure}{\sharedwidth\textwidth}
%   \vspace{.2cm}
  \centering
  \includegraphics[width=\linewidth, height = \sharedheight]{Fig/01201337power.pdf}
  \vspace{\vbetween}
  \caption{Power of detecting $V(\pi_1) > V(\pi_0)$.}
%   , when $H_1$ is true
\end{subfigure}%
% \vspace{-0.2cm}
\caption{Experiment results. 
The error bars indicate the standard errors of the averages.   
% averaged over $500$ random seeds
% For methods that consider the safety constraint, 
% The losses from safety violation for safe methods are all around zero and hence overlap.
}\label{fig:simu}
% safe design of experiments
\vspace{-0.5cm}
\end{figure}


==> Safe Exploration for OPE [Camera-ready]/Mis/new_commands.tex <==
\newcommand{\loss}{\nu}
\newcommand{\lam}{\lambda}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vz}{\mathbf{z}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vbeta}{\boldsymbol{\beta}}
\newcommand{\vlam}{\boldsymbol{\lam}}
\newcommand{\vrho}{\boldsymbol{\rho}}
\newcommand{\vM}{\boldsymbol{M}}
\newcommand{\vG}{\boldsymbol{G}}
%%%%%%%%%%%%%%%%%%%%
\newcommand{\vy}{\boldsymbol{y}}
\newcommand{\vY}{\boldsymbol{Y}}
\newcommand{\vL}{\boldsymbol{L}}
\newcommand{\vU}{\boldsymbol{U}}

\newcommand{\valpha}{\boldsymbol{\alpha}}
\newcommand{\vgamma}{\boldsymbol{\gamma}}

\newcommand{\tod}{\overset{d}{\to}}
\newcommand{\convergeD}{\xrightarrow[]{d}}

\newcommand{\hRI}{\widehat{RI}}
\newcommand{\vthe}{\boldsymbol{\theta}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mJ}{\mathcal{J}}

\newcommand{\TO}{\tilde{O}}

\newcommand{\indep}{\perp \!\!\! \perp}
% \newcommand{\Y}[1]{Y^*(#1)}
\newcommand{\Yz}{Y^*(0)}
\newcommand{\Yzi}{Y_i^*(0)}

\newcommand{\Yo}{Y^*(1)}
\newcommand{\Yoi}{Y_i^*(1)}

\newcommand{\mC}{\mathcal{C}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mE}{\mathbb{E}} 
\newcommand{\vxi}{\mathbf{x}_i} 
\newcommand{\vxj}{\mathbf{x}_j} 
\newcommand{\vc}{\mathbf{c}}
\newcommand{\veps}{\mathbf{\epsilon}}
\newcommand{\vdelta}{\boldsymbol{\delta}}


\newcommand{\dopt}{d^{opt}} 

\newcommand{\vA}{\boldsymbol{A}}
\newcommand{\vJ}{\boldsymbol{J}}


\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\neigh}{\mathcal{N}}

\newcommand{\name}[1]{\texttt{#1}}
\newcommand{\vS}{\boldsymbol{S}}
\usepackage{soul}
\usepackage{xcolor}
\newcommand{\tH}{\tilde{H}}
\newcommand{\Mean}{{\mathbb{E}}}
\newcommand{\Var}{{\mathbb{VAR}}}
% \newcommand{\Cov}{{\mathbb{COV}}}
\newcommand{\Cov}{\boldsymbol{\Sigma}}

\newcommand{\prob}{\mathbb{P}}

\newcommand{\vphi}{\boldsymbol{\phi}}
\newcommand{\vPhi}{\boldsymbol{\Phi}}
\newcommand{\vR}{\boldsymbol{R}}
\newcommand{\vr}{\boldsymbol{r}}
\newcommand{\vpi}{\boldsymbol{\pi}}
\newcommand{\vone}{\boldsymbol{1}}
\newcommand{\vzero}{\boldsymbol{0}}
\newcommand{\vI}{\boldsymbol{I}}
\newcommand{\vmu}{\boldsymbol{\mu}}

\newcommand{\mX}{\boldsymbol{X}}
\newcommand{\mK}{\boldsymbol{K}}
\newcommand{\mZ}{\boldsymbol{Z}}
\newcommand{\mU}{\boldsymbol{U}}
\newcommand{\mW}{\boldsymbol{W}}
\newcommand{\mV}{\boldsymbol{V}}

\newcommand{\normal}{\mathcal{N}}

\usepackage{amsthm}
\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{asmp}{Assumption}
% \newtheorem*{remark}{Remark}
\newtheorem{remark}{Remark}

%%%%%%%%%%%%

\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\green}[1]{{\textcolor{green}{#1}}}


\newcommand{\vage}{\boldsymbol{age}}
\newcommand{\vh}{\boldsymbol{h}}
\newcommand{\vw}{\boldsymbol{w}}
\newcommand{\vu}{\boldsymbol{u}}
\newcommand{\vliq}{\boldsymbol{liq}}


==> Safe Exploration for OPE [Camera-ready]/Mis/packages.tex <==
\usepackage[utf8]{inputenc}
% \usepackage[left=1.02in, right=1.02in, top=1.1in, bottom=1.05in]{geometry}
\usepackage{array}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{setspace}
\usepackage{textcomp}
\usepackage{enumitem}
\usepackage{datetime2}
\usepackage{multirow}
\usepackage[font=small,labelfont=bf]{caption}
% \doublespacing
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\usepackage{subcaption}
\usepackage{mathtools}
\usepackage{dirtytalk}

% \usepackage[usenames,dvipsnames]{xcolor}
\usepackage[backgroundcolor=white]{todonotes}
\newcommand{\todob}[2][]{\todo[color=red!20,size=\tiny,inline,#1]{B: #2}}
\newcommand{\todorw}[2][]{\todo[color=blue!20,size=\tiny,inline,#1]{RW: #2}}

% from cjhebrew.sty (with scaling added)
\DeclareFontFamily{U}{cjheb}{}
\DeclareFontShape{U}{cjheb}{m}{n}{%
  <-11> s*[1.2] cjhblsm
  <11-> s*[1.2] cjhbltx
}{}
\newcommand{\cjhebfamily}{\fontencoding{U}\fontfamily{cjheb}\selectfont}
\DeclareTextFontCommand{\textcjheb}{\cjhebfamily}

% provide the commands in case amssymb is not loaded
\providecommand{\beth}{}
\providecommand{\gimel}{}
\providecommand{\daleth}{}
% renew the commands
\newcommand{\mathhebrew}[1]{\text{\cjhebfamily#1}}
\renewcommand{\aleph}{\mathhebrew{\char'047}}
\renewcommand{\beth}{\mathhebrew{\char'142}}
\renewcommand{\gimel}{\mathhebrew{\char'147}}
\renewcommand{\daleth}{\mathhebrew{\char'144}}

% \usepackage{unicode-math}
% \usepackage{libertine}
% \setmathfont[range={\beth,\gimel,\daleth,\aleph}]{Linux Libertine O}   

